The Wreaths of KHAN: Uniform Graph Feature Selection with False Discovery Rate Control

Graphical models find numerous applications in biology, chemistry, sociology, neuroscience, etc. While substantial progress has been made in graph estimation, it remains largely unexplored how to select significant graph signals with uncertainty assessment, especially those graph features related to topological structures including cycles (i.e., wreaths), cliques, hubs, etc. These features play a vital role in protein substructure analysis, drug molecular design, and brain network connectivity analysis. To fill the gap, we propose a novel inferential framework for general high dimensional graphical models to select graph features with false discovery rate controlled. Our method is based on the maximum of $p$-values from single edges that comprise the topological feature of interest, thus is able to detect weak signals. Moreover, we introduce the $K$-dimensional persistent Homology Adaptive selectioN (KHAN) algorithm to select all the homological features within $K$ dimensions with the uniform control of the false discovery rate over continuous filtration levels. The KHAN method applies a novel discrete Gram-Schmidt algorithm to select statistically significant generators from the homology group. We apply the structural screening method to identify the important residues of the SARS-CoV-2 spike protein during the binding process to the ACE2 receptors. We score the residues for all domains in the spike protein by the $p$-value weighted filtration level in the network persistent homology for the closed, partially open, and open states and identify the residues crucial for protein conformational changes and thus being potential targets for inhibition.

==> Intro_May2023.tex <==
% !TEX root = main.tex


% {\darkblue

% Hessian matrix is defined as 
% $$
% \boldsymbol{H}_{i j}=\frac{\gamma \boldsymbol{\Gamma}_{i j}}{\left(R_{i j}^0\right)^2}\left[\begin{array}{lll}
% X_{i j} X_{i j} & X_{i j} Y_{i j} & X_{i j} Z_{i j} \\
% Y_{i j} X_{i j} & Y_{i j} Y_{i j} & Y_{i j} Z_{i j} \\
% Z_{i j} X_{i j} & Z_{i j} Y_{i j} & Z_{i j} Z_{i j}
% \end{array}\right],
% $$
% where ${R}_{i j}^0$ is the equilibrium distances between nodes $i$ and $j$, 
%  $X_{i j}, Y_{i j}$ and $Z_{i j}$ are the components of the distance vector ${R}_{i j}^0$. $\boldsymbol{\Gamma}_{i j}$ is equal to 1 if nodes $i$ and $j$ are within an
% interaction cutoff distance $r_c$, zero otherwise. $\gamma$ is a constant.


% The diagonal super elements of $\boldsymbol{H}$ are $3 \times 3$ submatrices
% $$
% \boldsymbol{H}_{i i}=-\sum_{j \mid j \neq i} \boldsymbol{H}_{i j} .
% $$


% $\,\,$The cross-correlation between the equilibrium fluctuations of residues $i$ and $j$ is expressed in terms of the trace (tr) of these submatrices as
% $$
% \boldsymbol{C}_{i j} =\frac{\operatorname{tr}\left(\boldsymbol{H}_{i j}^{-1}\right)}{\sqrt{\operatorname{tr}\left(\boldsymbol{H}_{i i}^{-1}\right) \operatorname{tr}\left(\boldsymbol{H}_{j j}^{-1}\right)}}
% $$
% where $\boldsymbol{H}^{-1}$ is the pseudo-inverse. 
% }


\section{Introduction}\label{sec:intro}
% {  
% \begin{itemize}
%     \item edit the parts pointed out in jiajun pdf sent in Wechat
%     \item change the red parts
%     \item delete ising high temperature
%     \item M can be at order $d$. change expression for $\tbinom{d}{M}$.
%     \item (PH)in persistent homology, the graph of ising is $W^*=E[XuXv]$ not $W^*=E[XuXv]-\tanh \theta$ that used in subgraph selection
%     \item change $\sqrt{n}\hat{W}_e$ to $\sqrt{n}\hat{W}_e/\hat{\sigma}_e$ - done
%     \item find a proper definition of $\sigma_e$
%     \item (PH)edit S set and H tilde set by incorparting normalization.
%     \item (PH)edit remark 5.2 - done
%     \item (PH)read persistent homology algorithms and edit the explanation for algorithms
%     \item (PH)simplify the discussion of theory parts.
% \end{itemize}
% }

% Graphical models are widely used to model the relationships among variables. They have vast applications in a variety of fields, including social networks \citep{newman2002random}, genetics \citep{luscombe2004genomic, yuan2017co} and neuroscience \citep{rubinov2010complex, van2013network}.   
% Most existing literature focuses on the estimation and inference of edges \citep{cai2013optimal, liu2013gaussian, cai2013two, gu2015local, jankova2017honest, li2021ggm}.
% Graphical models are widely used to model the relationships among random variables based on observations of these random variables, and find many applications, including social networks \citep{newman2002random}, genetics \citep{luscombe2004genomic, yuan2017co} and neuroscience \citep{rubinov2010complex, van2013network}.   
% Most existing literature focuses on the estimation and inference of edges \citep{cai2013optimal, liu2013gaussian, cai2013two, gu2015local, jankova2017honest, li2021ggm}.



%Jan 30
Graphical models are a prevalent tool for modeling relationships between variables. They are widely used in various fields where the structure of graphs between  variables is of great interest. 
In biology, proteins are vital to life and their practical function is highly influenced by their unique structure, which is determined by the combination of amino acids. Understanding and identifying protein structures is therefore crucial. 
For example, the Y-shape of an antibody enables it to bind to antigens like bacteria and viruses with one end and to other immune-system proteins with the other end \citep{janeway2001structure}. Similarly, the donut-like shape of the DNA polymerase III holoenzyme facilitates the efficient formation of a ring around DNA, enabling fast DNA synthesis \citep{kelman1995dna, 2013v}. 
Alphabet/Google is developing AlphaFold to predict the structures of proteins with  artificial intelligence (AI) \citep{jumper2021highly, evans2021protein}.   
In chemistry, a critical task is modeling molecular structures, which determine their pharmacological and ADME/T properties (absorption, distribution, metabolism, excretion, and toxicity). For instance, the stable loop structure of the benzene ring prevents it from breaking apart easily \citep{armstrong1890structure}; the presence of the cyanide group (CN) makes hydrogen cyanide (HCN) highly toxic, leading to potential death within minutes\citep{national2002acute}. 
In neuroscience, cliques within the brain network are vital as they are neurologically strongly associated with efficient support of behavior \citep{bassett2017network, wang2021learning}.
In sociology, plays an important role in understanding behavior among individuals or organizations and making social recommendations or marketing strategies. For instance, the presence of a "star" structure in the social network indicates that the central user is active and influential, as they are connected to many other users. Therefore, the advertising industry often targets these individuals with free samples to increase their reputation, rather than selecting people at random \citep{ ilyas2011distributed, li2018influence,lee2019discovering}.


% Graph selection is also of great importance in many fields because structures of graphs matter in practice.
% % 
% In biology, proteins are essential to life, and the practical function of a protein highly depends on its unique structure, or the combination of different amino acids. So it is crucial to understand and identify  protein structures. % and protein-protein interaction. 
% For example, an antibody is Y-shaped so each tip of ``Y'' binds with antigens such as bacteria and viruses, and another end binds to other immune-system proteins \citep{janeway2001structure}. DNA polymerase III holoenzyme is donut-shaped, which helps it form a ring around DNA as it copies genetic information so it can synthesize DNA with high speed \citep{kelman1995dna, 2013v}. 
% Alphabet/Google is developing AlphaFold to predict the structures of proteins with  artificial intelligence (AI) \citep{jumper2021highly, evans2021protein}.
% % AlphaFold has been used to predict protein structures of SARS-CoV-2, the causative agent of COVID-19 (CITE).
% % \yue{For instance, \cite{kramer2009regularized} applied Gaussian Graphical Models to construct a large-scale network of gene-gene interactions.}    
% Also, in chemistry, one essential task is to model molecular structure, which decides its pharmacological and ADME/T (absorption, distribution, metabolism, excretion, and toxicity) property. For example, the unique loop structure of the benzene ring makes it stable and does not break apart easily \citep{armstrong1890structure}. The existence of the cyanide group (CN) makes hydrogen cyanide (HCN) highly toxic, which can cause death within minutes \citep{national2002acute}. 
% In addition, in neuroscience, cliques in the brain network are essential because they have neurological meanings that they should be strongly related to support a behavior most efficiently \citep{bassett2017network, wang2021learning}.
% %Selecting protein loops and RNA internal loops are also important in chemistry and biology {   (Protein loop selection using orientation-dependent force fields derived by parameter optimization) ( Small Molecule Microarray Platform To Select RNA Internal Loop-Ligand Interactions)(Optimal sequence and structure of iron-responsive elements. Selection of RNA stem loops with high affinity for iron regulatory factor)}. 
% In sociology, the structure of the social network is also important for understanding behavior between individuals or organizations and social recommendation or marketing. For example, a ``star'' structure in the social network means the hub user is active and influential as they connect to many other users. So the advertising industry tends to give free samples to them instead of random people to increase reputation \citep{ ilyas2011distributed, li2018influence,lee2019discovering}.



% \yue{xxx paper said yyyy structure is important
% }

%   For example, \cite{mahmood2021masked} use graphical model to learn conditional distributions over nodes (atoms) for drug discovery and materials design. \cite{olsson2019dynamic} use Ising model to model molecular dynamics based on observed states. % of subsystems.





Motivated by the vast applications of the structure of graphical models mentioned above, this paper focuses on selecting subgraphs of interest in general graphical models.
Let $G^* = (V, E^*)$ represents the true undirected graph, where $V=\{1,2 \cdots, d\}$ is the collection of nodes and $E^*$ is the edge set of the graph.
Let $\bX=\bigl(X_{1}, \cdots, X_{d}\bigr)^\top \in \mathbb{R}^{d}$ be a random vector indexed by the nodes of $G^* = (V, E^*)$, i.e., node $j$ of the graph corresponds to random variable $X_j$. $\bX$ can be either continuous (e.g., Gaussian graphical model) or discrete (e.g., Ising model).
The edge set $E^*$ consists of pairs of distinct nodes.  In general, we denote the true edge weights as $W^*:=\{W^*_e\}_{e \in V\times V}$.
% {  examples to show what F is? and what the Fsubset F mean? I recall these are formally defined later...But it seems without those definitions it may be hard to understand these concepts here.}
Suppose $\cF=\{F_1,F_2,\ldots,F_J\}$ is the set consisting of all subgraphs of interest in $G^*$ that we aim to select. We denote the cardinality  of $\cF $ as $J:=|\cF |$.  Some of them may exist in $G^*$, some may not. To select them simultaneously,  we consider a multiple testing problem, which involves testing whether each subgraph  $F_j\in {\cal F}$ can be embedded into the true graph $G^*$, i.e., 
\begin{equation}\label{eqn:hypo}
H_{0j}: F_j \not\subseteq  G^* \quad \mbox{v.s.}\quad H_{1j}: F_j \subseteq G^*,\quad 1\leq j\leq J.    
\end{equation}   
When selecting the subgraphs, we aim to have statistical control over the false discovery proportion (FDP) and the false discovery rate (FDR), which are defined as:
\begin{equation}\label{eq:classicalFDPFDR}
    \mathrm{FDP}:=\frac{\sum_{j \in \cH_{0}} \psi_{j}}{\max \Bigl\{1, \sum_{j=1}^{J} \psi_{j}\Bigr\}}, \qquad \mathrm{FDR}:=\mathbb{E}[\mathrm{FDP}].
\end{equation}
Here $\mathcal{H}_{0}$ is the set of all true null hypothesis, i.e., $\cH_0=\bigl\{1\leq j \leq J \biggiven  F_j \not\subseteq G^* \bigr\}$. Also, $\psi_{j}$ is defined as the result of the $j$-th test in \eqref{eqn:hypo} where $\psi_{j}=1$ if we reject $H_{0j}$ and $\psi_{j}=0$ otherwise.
    


Our goal is to select subgraphs of interest from $G^*$ simultaneously
with controlling false discovery 
We propose a novel inferential framework. Our approach is applied to two widely-used graphical models: the Gaussian graphical model and the Ising model.

The core of our method is estimating the $p$-value for each subgraph. We then employ the well-established Benjamini and Hochberg (BHq) procedure \citep{benjamini1995controlling} to determine the rejection set based on these $p$-values. To determine a credible $p$-value for each subgraph, we first compute the $p$-value for each individual edge.
Interestingly, we show that a valid way to assign the $p$-value for a subgraph is by taking the maximum $p$-value among all edges within the subgraph. This is because making a type I error in a single subgraph test implies that we must have made a type I error in at least one of the edges involved in that subgraph.  Thus, as long as the $p$-value for each edge is valid, our defined $p$-value for each subgraph is reliable. . This approach differs significantly from previous methods in combinatorial inference, e.g., \cite{zhang2021startrek,shen2020combinatorial, liu2022lagrangian}. % {  one more citation?}  
Our proposed method is designed to be computationally efficient and does not rely on the use of the maximum statistic or Gaussian multiplier bootstrap for quantile estimation. As a result, our approach offers a more straightforward and efficient solution compared to existing methods in the literature.

The previous method provides a solution  for detection of linearly dependent structure on a graph, which could be algebraically redundant in some vector spaces. Further, we provide solutions to select linearly independent subgraph features. We also aim to evaluate the persistence of the   subgraphs features in addition to just selecting them.  Intuitively, the persistence of subgraphs is related to the signal strength, which can vary across different subgraphs. During the filtration process of the graph, subgraphs with weak signal strength may disappear quickly, while those with strong signal strength may persist.
 In particular, we utilize the framework of persistent homology, which is a powerful tool for analyzing and measuring the persistence of specific subgraph features, such as loops and tetrahedrons. The concept of topological features will be formally introduced in Section \ref{sec:ph:pre}.

 To analyze the persistence of  subgraph features, we  select  cycle group at a specific filtration level, and further obtain the lifespan of each subgraph feature (the birth and death time). 
% Basically, {   $k$-th cycle  group is a set of cycles which are $k$ chains with empty boundary.}
% topological invariant features, which formalizes the idea of the number of ``holes'' in the graph.  $0$-th group is the group of connected components,  $1$-th group is the group of loops, $2$-th group is the group of voids. We consider selecting all the $k$-th homology groups for $k\in \cD$.
It is not a simple variable selection problem, as we actually aim to select linearly independent bases in each group. Denote $\bar J$ as the dimension of the cycle group of interest. 
% Intuitively starting from a null group, as we add edges in our group, the dimension of this group will increase once we add some ``critical'' edges. So we have $\bar J_k$ ``critical'' edges for the $k$-th homology group, and there is a homology group associated with
% each $j$-th critical edge of the  $k$-th homology group, denoted as $\bar{\mathrm{H}}_k^j$. 
The problem can be framed as the following multiple testing pairs in terms of $j$:
\begin{equation}\label{eqn:3}
\begin{aligned}
& H_{0j}(\mu):\text{the $j$-th basis of the  {cycle} group} \nsubseteq G^*(\mu),\\
     \text{v.s.}  \ 
     & 
     H_{1j}(\mu):\text{the $j$-th basis of the  cycle group} \subseteq G^*(\mu),%, 
     %\quad j \in \bar J.
\end{aligned}
\end{equation}
where $\mu$ is the filtration level of the graph, and $G^*(\mu)$ is the filtered graph at level $\mu$ formally defined in Section \ref{sec:ph:pre}.


 We propose Algorithm \ref{alg:ph:basis} to select the linearly independent bases at any given filtration level $\mu \in (\mu_0,\mu_1)$ for some self-determined $\mu_0, \mu_1$. Basically at each iteration, we select the basis with the smallest $p$-value and is linearly independent of the currently selected bases.
%
However, running Algorithm \ref{alg:ph:basis} infinitely is not feasible for obtaining complete persistent barcodes of subgraph features. Instead, we propose Algorithm \ref{alg:ph:barcode}, which efficiently identifies the change points in the filtration level where the cycle group changes. This algorithm utilizes the discrete structure of the graph and adaptively determines the next filtration levels at which the set of selected bases changes.


Moreover, when selecting the cycle group along the filtration of the graph, we would like to uniformly control FDP and FDR over a continuous filtration interval $(\mu_0,\mu_1)$.
In this paper, we propose the uniform False Discovery Proportion (uFDP) and the uniform False Discovery Rate (uFDR), which are   the supremum of the standard FDP and FDR over the interval $(\mu_0,\mu_1)$.  Theoretically, we prove that the defined uFDP and uFDR in \eqref{eq:ph:FDPFDR} can be controlled asymptotically with our algorithms. 

In summary, we list the following three novelties in the second part of our paper: selecting linearly independent subgraph  features and cycle group, adaptively detecting the change points by our proposed algorithm, and developing  uniform false discovery control. 


% Motivated by various applications, in this paper, we aim to  select general subgraphs of interest from high dimensional graphical model. Suppose we are interested in a specific subgraph $F$,
% and our goal is to select all subgraphs with the same structure as $F$ (i.e., isomorphic  to $F$. The formal definition of isomorphic can be found in Definition \ref{def:isomorphic})  with FDR control.   
% We also apply our method to two widely-used graphical
% models: the Gaussian graphical model and the Ising model. 




% Despite the aforementioned significant progress of graph inference, 

Finally, we point out several essential differences between our paper and \cite{zhang2021startrek}.
First, the Startrek procedure in \cite{zhang2021startrek} is primarily designed for selecting   hub nodes, while our goal is to select general subgraphs of interest in our paper (which can also give hub nodes once we select the ``star'' pattern). Our problem is much more  complicated and challenging, and has broader applications.
Second, the Startrek procedure in \cite{zhang2021startrek} involves the use of the maximal statistic for uniform control over edges and Gaussian multiplier bootstrap for quantile estimation, which is complex, statistically conservative and computationally intensive. In contrast, our proposed method does not require the use of either the maximum statistic or Gaussian multiplier bootstrap, making it simpler and more efficient.
% 
Third, our method can be applied to study the persistence of subgraph features in the framework of persistent homology and has stronger false discovery control over continuous scales. 
In summary, our proposed method is simpler and faster, while our problem is harder and more complicated with broader applications compared to the problem in \cite{zhang2021startrek}.

\color{black}


\subsection{Related work}

Learning  graph structures  has been widely studied in the existing literature. There have been many significant progress on recovering the underlying graph by estimation.
For the Gaussian graphical model, many works estimate the
graph through estimating the inverse covariance matrix $\Theta^*$ where $\Theta^*_{uv}=0$  if and only if the edge $(j, k) \in E^*$
\citep{meinshausen2006high, friedman2008sparse, lam2009sparsistency, peng2009partial, ravikumar2011high, cai2011constrained, shen2012likelihood}.
For the Ising model, which consists of discrete variables ($+1$ or $-1$), \cite{ravikumar2010high} estimate the parameters by penalized logistic regression, \cite{bhattacharya2018inference} study parameter estimation and inference using  maximum pseudolikelihood estimate.


Beyond estimation, inferential methods are also proposed to quantify the uncertainty in graph. % Here we focus on multiple testing problem in graphical model \citep{xxxxx}.
%
However, most literature focus on continuous quantities and local properties of graph (e.g., presence of edges) \citep{cai2013optimal,jankova2015confidence,ren2015asymptotic, cai2016inference,  chen2016asymptotically, neykov2018unified}. For example, \cite{cai2013optimal}
construct hypothesis tests for covariance matrix, \cite{ren2015asymptotic} test the presence of edges in the Gaussian graphical model, \cite{cai2016inference} consider estimation and testing of high-dimensional differential correlation matrices. 
For multiple tests in graphical models, 
\cite{10.2307/23566754} focus on selecting edges with FDR control using Benjamini-Hochberg method \citep{benjamini1995controlling}, \cite{li2021ggm} learn the structure of Gaussian graphical models with FDR control based on the knockoff framework.
%



All previously mentioned methods focus mainly on  the local properties of a graph. For combinatorial structure and global properties of graph, \cite{lu2017adaptive} propose to test monotone properties in the Gaussian graphical model, e.g., connectivity, the maximum degree, cycle presence.  \cite{neykov2019property, jin2020computational} aim to test graph properties in  the Ising model. 
However, their methods are designed to conduct single tests only. 
For simultaneously multiple testing problem, \cite{zhang2021startrek} propose the Startrek algorithm to select hub nodes with degree larger than a pre-specified threshold in graphs. 


% There is also a line of works developing combinatorial inferential methods in graph. For example,
% \cite{lu2017adaptive, neykov2019combinatorial} propose a
% general inferential framework for testing combinatorial properties of graph, such as size of the largest clique,
% the maximum degree, connectivity.  \cite{neykov2019property, jin2020computational}  aim to test graph properties  in Ising models. 
% \cite{zhang2021startrek} propose Startrek algorithm to select hub nodes with degree larger than a pre-specified threshold in graphs. 

    


\vspace{10pt}



% However, the problem of selecting general subgraphs of interest remains largely unexplored, which is of crucial importance in practice. For example, {   clique in brain network, have neurological meanings that they should be strongly related to support a behavior most efficiently.
% (Learning Clique Subgraphs in Structural Brain Network Classification with Application to Crystallized Cognition)}
%     Also,  selecting protein loops  in chemistry or RNA internal loops {   xxxxxxxx (Protein loop selection using orientation-dependent force fields derived by parameter optimization) ( Small Molecule Microarray Platform To Select RNA Internal Loop-Ligand Interactions)(Optimal sequence and structure of iron-responsive elements. Selection of RNA stem-loops with high affinity for iron regulatory factor)}.
    
% {   REPLACE (Paper) by reference}

% {   benzene in chem?}

% {   ADD other motivating examples}



\subsection{Contribution}
For ordinary subgraph selection,   we develop a novel
inferential framework to select general subgraphs in graphical models. In general, the subgraphs of interest  can be loops, cliques, and stars, among others.
Additionally, our method is significantly simpler and faster than previous combinatorial inference methods  since it does not involve maximum statistic and Gaussian multiplier bootstrap for quantile estimation. In theory, the proposed framework is guarantee to achieve FDR control and be powerful theoretically under reasonable sparsity and dependence conditions. 
It is shown to be valid for many different graphical models. We provide two applications for continuous and discrete observations in graphs: the Gaussian graphical model and the Ising model.

%The first part provides a solution  for detection of linearly dependent structure on a graph, which could be algebraically redundant in some vector spaces. 
Moreover, we propose a new algorithm that utilizes persistent homology to efficiently select the underlying linearly independent bases of subgraph features and evaluate their persistence along filtration.  
We introduce a new and stronger definition to quantify uniform  false discovery on continuous scales (namely uFDP and uFDR). We  show that the empowered procedure could satisfy guarantee of statistical control of  uFDP and uFDR on a whole interval. %Surprisingly, we also discover that statistically and computationally the task of selecting linearly independent structure could be much easier to the corresponding task of selecting linearly dependent structure. We can still do feature selection with strong power and control on false discoveries guarantee even if we cannot observe the empirical rejection results of multiple testing.



\subsection{Notations}
 
We denote set $A \times B=\{(a,b): a \in A, b \in B\}$ and define $E=V\times V$ to be the complete edge set. 
We define $E(\cdot)$ to be a  function where   $E(G)$ gives the  edge set of graph $G$, and we define $V(G)$  be the vertex set  of graph $G$. We say $G \subseteq G'$ if and only if $V(G)\subseteq V(G')$ and $E(G)\subseteq E(G')$.   
Let $G^*$ be a true graph with vertex set $V$ and edge set $E^*$, and let $G$ be an arbitrary graph that may differ in different instances. We use  $[n]:=\{1,2,\ldots,n\}$ and $|A|$ to denote the cardinality of a set $A$.
For a vector $\bX = \bigl(X_{1}, \cdots, X_{d}\bigr)^\top$, we define $\bX_{-\cI}:=\bX_{[d] \backslash \cI}$ on a set ${\cal I}$.
 $\Phi(\cdot)$ is the cumulative distribution  function of standard Gaussian.



 % \yue{$\hat{\Theta}^d:\mbox{any estimate for } \Theta^{\star}$, $\widetilde{\Theta}:\mbox{any estimate for } \Theta^{\star}$, $\widetilde{\Theta}^d:\mbox{any debiased estimate for } \Theta^{\star}$.} 	
 
 
 
% { ques Change section title to `subgraph selection'}

\section{Method}\label{sec:method}
%In this paper, we first describe the general subgraph selection problem from graphical models.
In this section, we first provide some preliminaries on the concept of graphical model and the subgraph selection problem. Then, we provide our methodology.



\subsection{Problem Setup}\label{sec:setup}

Undirected graphical model is widely used to represent the conditional dependence structure between random variables.     
Let $G^* = (V, E^*)$ be the true undirected graph, where $V=\{1,2 \cdots, d\}$ is the node set and $E^*$ is the edge set of the graph.
Let $\bX=\bigl(X_{1}, \cdots, X_{d}\bigr)^\top \in \mathbb{R}^{d}$ be a random vector indexed by the nodes of $G^* = (V, E^*)$, i.e. node $j$ of the graph corresponds to random variable $X_j$. 
The edge set $E^*$ consists of pairs of distinct nodes. 
In general, we denote the true edge weights as $W^*:=\{W^*_e\}_{e \in E^*}$. The following two examples are widely used in practical applications.

\begin{example}[Gaussian Graphical Model]\label{ex:GGM}
In the Gaussian graphical model, $\bX$ follows a multivariate Gaussian distribution $N_d(\bm{0},\Sigma^*)$
with mean vector $\bm{0}$ and covariance matrix $\Sigma^*$. 
Let the precision matrix $\Theta^* = {\Sigma^*}^{-1}$, which indicates the conditional independence between the random variables.
We have $\Theta^*_{uv}=0$ if and only if $(u,v) \notin E^*$ (i.e., $X_u \indep X_v \given \bX_{-\{u,v\}}$).
In this example, we can take the edge weight as $ W^*_{uv}=\Theta^*_{uv}$  for any $(u,v)\in E$. 
\end{example}

\begin{example}[Ferromagentic Ising Model]\label{ex:ising}
In the Ising model,  $\bX \in \{1,-1\}^{d}$ for each node has distribution
\begin{equation}\label{eqn:Ising}
\mathbb{P}(\bX = \mathbf{x}) = \frac{1}{Z(\mathbf{w}^*)} \exp \Big( \sum_{(u, v) \in E} w^*_{u v} x_{u} x_{v}\Big),
\end{equation} 
where $\mathbf{x} = (x_{1}, \cdots, x_{d})^\top$ is an observation of $\bX$, $\mathbf{w}^* = \{w^*_{u v}\}_{(u, v) \in E}$ is the weights on the edges, and $$Z(\mathbf{w}^*) = \sum_{\mathbf{x} \in \{1,-1\}^{d}} \exp \Big( \sum_{(u, v) \in E} w^*_{u v} x_{u} x_{v}\Big)$$ is the partition function (i.e., the normalizing constant), which ensures the distribution in \eqref{eqn:Ising} sums to $1$. We have $w^*_e > 0$ if and only if $e \in E^*$, $w^*_e=0$ for $e \notin E^*$. Similar to \cite{neykov2019property}, we assume there is a known lower bound $\theta$ for $w^*_e, e\in E^*$.
% 
In practice, estimating the weight $w^*_{uv}$ in the Ising model \eqref{eqn:Ising} is not easy. 
% 
However, Lemma 3.1 in\cite{neykov2019property} shows that  the correlation between variables can be used to characterize the edge weight. Specifically,  $\E[X_uX_v]- \tanh \theta >0$ if and only if $w^*_{uv} >0$. Moreover,  correlation $\E[X_uX_v]$ is easier to estimate than $w^*_{uv}$.
 So we focus on studying  the weight  $W^*_{uv}=\mathbb{E}[X_uX_v]-\tanh(\theta)$  in Sections \ref{sec:thm} and  \ref{sec:example:Ising}. 
% {  Jiajun: the weight problem, its for subgraph not for ph}

\end{example}



%{ ques Are they 0 for the diagonal of $W^*$?}
% {   $M$ denotes $\max_j|V(F_j)|$}

% In addition, we assume Gaussian graphical model throughout this paper, i.e., the random vector $\bX$ follows a multivariate Gaussian distribution $N_d(\bm{0},\Sigma^*)$
% with mean vector $\bm{0}$ and covariance matrix $\Sigma^*$.
% % 
% Let the precision matrix $\Theta^* = {\Sigma^*}^{-1}$. We have $\Theta^*_{ij}=0$ if and only if $(i, j) \notin E^*$ (i.e., $X_i \indep X_j \given \bX_{-\{i,j\}}$). So we can write edge set as $E^*=\big\{(i, j) \in E \biggiven i \neq j, \Theta^*_{i j} \neq 0\big\}$.

% {   
% We consider the following parameter space for precision matrices
% $$
% \mathcal{U}(s)=\left\{\Theta \in \mathbb{R}^{d \times d} \mid 1/\rho \leq \Theta \leq \rho, \max _{j \in[d]}\left\|\Theta^*_{\cdot j}\right\|_{0} \leq s,\|\Theta\|_{1} \leq M, \Theta = \Theta^\top \right\},
% $$ which requires $\Theta$ having less than $s$ non-zero entries for each column. Thus, $\Theta$ is $s$-sparse under this condition, and the induced graphs have maximum degree of less than or equal to $s$.
% %
% Also, we assume $1/\rho \leq \Theta \leq \rho$ meaning that $\lambda_{\min }(\Theta) \geq 1 / \rho$ and $\lambda_{\max }(\Theta) \leq \rho$, i.e., the minimum and maximum eigenvalues of $\Theta$ are  bounded by $1/\rho$ and $\rho$.
% 
% So the parameter space $\mathcal{U}(s)$
% restricts our precision matrix $\Theta$ to well-conditioned symmetric matrices.

% }

Given the above setup, assuming we have $n$ i.i.d. observations $\bX_1,\ldots, \bX_n$ follow the distribution of $\bX$, our goal is to select general subgraphs  $\cF:=\{F_j\}_j$  from the underlying true graph $G^*$ with the false discovery rate (FDR) control.  The subgraphs $F_j$ can be any type of subgraph such as a triangle or a clique, and some of them may exist in $G^*$ while others may not. To select them simultaneously,  we consider  the  multiple testing problem defined in \eqref{eqn:hypo} and 
aim to control the false discovery proportion (FDP) and the false discovery rate (FDR), which is defined in \eqref{eq:classicalFDPFDR}.
In this paper, we propose a general multiple testing procedure to select subgraphs while  the  tail probability of  FDP and the FDR can be controlled below a given level $0<q<1$.

      
% % \begin{definition}
% % We say $H=(V_H,E_H)$ can be embedded into $G = (V, )$ (denoted by $H \subseteq G$) if $|V_H| = |V|$ and there exists a map  $\sigma\in P$ such that $\Big\{(\sigma(i),\sigma(j)):(i,j)\in E_H\Big\}\subseteq E$, where $P=\{\sigma:V_H \mapsto V\}$ be the set of all permutations from node set  $V_H$ to $V$. 
% % \end{definition}

% % For example, $H=\big(\{4,5,6\}, \{(4,5),(4,6)\}\big)$ can be embedded into $G=\big(\{1,2,3\}, \{(1,2),(1,3),(2,3)\}\big)$. % See Figure \ref{fig:sub}.

% % \vspace{-20pt}
 
% % \begin{figure}[h!]
% % 	\begin{center}
% % 		\begin{tabular}{cc}	
% % 	\includegraphics[width=.25\textwidth,angle=0]{./figure/sub} \\
% % 			[-37pt]
% % 		\end{tabular}
% % 	\end{center}
% % 	\caption{Illustration of the definition for subgraphs. $G_0=\big(\{2,3\}, \{(2,3)\}\big)$ (as highlighted in blue) is a subgraph of $G=\big(\{1,2,3\}, \{(1,2),(1,3),(2,3)\}\big)$.}
% % 	\label{fig:sub}
% % \end{figure}
% {
% \color{gray}
% In general, the subgraphs we are interested in selecting (i.e., $H$) can be a loop, a clique, or a star. Several concrete examples are provided below. 

% \begin{example}[Triangle]\label{eg:triangle}
% A triangle is a structure involving three nodes, where every two distinct nodes are connected. See Figure \ref{fig:subgraph} (A).
% \end{example}

% \begin{example}[Cycle]\label{eg:cycle}
% A cycle is a structure that forms a path such that the first node of the path corresponds to the last node. See Figure \ref{fig:subgraph} (B).
% \end{example}

% \begin{example}[Clique]\label{eg:clique}
% A clique is a structure where every two distinct nodes are connected. See Figure \ref{fig:subgraph} (C).
% \end{example}

% \begin{example}[Star]\label{eg:star}
% A star is a structure where one central node is connected
% to several other nodes. This structure is widely analyzed in the social network. See Figure \ref{fig:subgraph} (D).
% \end{example}


% \begin{figure}[h!]
% 	\begin{center}
% 		\begin{tabular}{cc}	
% 		&{\ (A) Triangle \quad\quad  (B) Cycle \quad\quad  (C) Cilque \quad\quad\quad\ \  (D) Star \quad\quad\quad\ } \\
% 		&\includegraphics[width=.7\textwidth,angle=0]{./figure/triangle} \\
% 			[-10pt]
% 		\end{tabular}
% 	\end{center}
% 	\caption{Examples of subgraphs of interest.}
% 	\label{fig:subgraph}
% \end{figure}

% }

% \begin{definition}
% Let $\cV$ be  the set of all $m$-elements subsets of $V$ and $|\cV|=\binom{d}{m}$. 
% For $1\leq j\leq \binom{d}{m}$, we define $G_j^*:=(V_j,E^*_j)$ where $V_j^*$ is the $j$-th element  of $\cV$, and $E^*_j=\big\{e \in V_j^* \times V_j^* \biggiven e \in E^*  \big\}$.
% \end{definition}
  
  


% {\color{pink}

% \begin{definition}
% Let $\cV$ be  the set of all $m$-elements subsets of $V$ and $|\cV|=\binom{d}{m}$, where $m=|V_H|$. Let $V_i^*$ be the $i$-th element  of $\cV$.
% For $1\leq i\leq \binom{d}{m}$, 
% assume $H$ can be embedded into the complete graph $(V_i^*, V_i^* \times V_i^*)$ in $i_k$ different ways, i.e.,  
% there exists $i_k$ permutations $\sigma\in P$ such that $\Big\{(\sigma(i),\sigma(j)):(i,j)\in E_H\Big\}\subseteq V_i^* \times V_i^*$.


% $G_j^*$ is defined as $(V_i^*, \Big\{(\sigma(i),\sigma(j)) \in :(i,j)\in E_H\Big\})$
% \end{definition} 

% }
      



% \begin{definition}\label{def:isomorphic}
% We say two graphs $G$ and $G'$ are isomorphic (denoted as $G\simeq G'$) if there exists a bijection $f\colon V(G)\to V(G')$ such that$(u, v) \in E(G)$  if and only if $(f(u), f(v)) \in E(G')$.
% \end{definition}



% % \yue{Let $m \geq |H|$ be a positive integer, and $\cV$ be a collection of some $m$-element subsets of $V$. For example, $\cV$ can be the collection of all $m$-element subsets of $V$, or $\cV$ can be $\big\{ \{1,2,3\}, \{4,5,6\}, \ldots \big\}$. Intuitively, $\cV$ is a collection of node sets and we are interested in selecting all subgraphs with each node set. }
% {    
% Let $\cV \subseteq 2^{V}$ be a collection of some subsets of $V$, where $2^{V}$ is the set of all subsets of $V$. Intuitively, $\cV$ is a collection of node sets and we are interested in selecting all subgraphs with each node set. For example, $\cV$ can be the collection of all $|V(F)|$-element subsets of $V$. %, or $\cV$ can be $\big\{ \{1,2,3\}, \{4,5,6\}, \ldots \big\}$.  
% {Define the set of subgraphs of interest $$\mathcal{F} = \Big\{\tilde F = (\tilde V, \tilde E): \tilde F \simeq F, \text{ and there exists $V \in \cV$ such that $\tilde V \subseteq V$ }\Big\},$$
% where $F$ is the subgraph we aim to select.
%{  Intuitively ${\cal F}$ is the set of possible subgraphs candidates with the specific structure $F$ we are interested in.} 
%}


%{  Jiajun: we consider different structure }
% \begin{definition}
% We say $H=(V_H,E_H)$ can be embedded into $G = (V,E)$ (denoted by $H \subseteq G$) if there exists a map $\sigma\in P$ such that the edge set $\Big\{(\sigma(i),\sigma(j)):(i,j)\in E_H\Big\}\subseteq E$. Here $P_{V_H \mapsto  V}=\{\sigma:V_H \mapsto (v_1,v_2,.., v_m) \subseteq V\}$ is the set of all permutations from node set  $V_H$ to all  $m$-elements subsets of  $V$ and $m=|V_H|$.
% \end{definition}
%
% \begin{definition}
% We define the set of all subgraphs of $G^*$ that can be embedded into $H$  as $$\cA = \Big\{ F \subseteq G^* \biggiven F \subseteq H, |V_F| = |V_H| \Big\},$$ and define the set of ``largest'' subgraphs in $\cA$ as
% $$\cB = \Big\{ F \in \cA \biggiven \nexists F' \in \cA,\text{ such that } F \subseteq F' \Big\}.$$
% Denote $J:=|\cB|$ and $G_j^*$ is the $j$-th element in $\cB$.
% \end{definition}
%
% \begin{definition}
% Suppose $H$ can be embedded into the complete graph $(V, E)$ in $J$ different ways, i.e.,  
% there exists $J$ permutations $\sigma_1,..., \sigma_J\in P_{V_H \mapsto  V}$ leading to $J$ different edge sets $\Big\{\big(\sigma_j(i_1),\sigma_j(i_2)\big):(i_1,i_2)\in E_H\Big\}\subseteq E$. Then define $G_j^*=(V_j,E^*_j), 1 \leq j \leq J$ as subgraphs of $G^*$, where $V_j^* =\sigma_j(V_H)$ and $E_j^*=\Big\{ \big(\sigma_j(i_1),\sigma_j(i_2)\big) :(i_1,i_2)\in E_H \text{ and } \big(\sigma_j(i_1),\sigma_j(i_2)\big) \in E^*\Big\}$. 
% \end{definition}
%
%   {  Let $H:=(V_H,E_H)$ and $G:=(V,E)$. 
%   We say $H\subseteq G$ if $V_H\subseteq V$ and $E_H\subseteq E$. 
%   \[
%   \tilde{{\cal H}}_1=\Big\{(\widetilde{V},\{(\sigma(i),\sigma(j)):(i,j)\in E_H\}):\widetilde{V}\subseteq V\text{with }|\widetilde{V}|=|V_H|; \sigma \in P_{V_H\mapsto \widetilde{V}}\Big\}
%   \]
%   \[
%   H_{0j}: \tilde{{\cal H}}_1_j\not\subseteq  G^* \qquad \mbox{v.s.}\qquad H_{1j}: \tilde{{\cal H}}_1_j \subseteq G^*,\qquad 1\leq j\leq J:=|\tilde{{\cal H}}_1|. 
%   \]
%   } 




% {  Let $V\subset V$ be an $m-$nodes subset of $V$ and $E$ be a possible edges set on the $m$ nodes $V$. (i.e., for any $i,j\in V$ with $i\neq j$, $\{i,j\}\in E$). Therefore, $G=(V,E)$ forms a graph on the $m$ nodes $V$. We say $G$ is a subgraph of $G$, denoted by $G\subset G$, if $E\subset E$. We are interested in testing whether for some $V\subset V$, the graph $G$ with some specific structures (e.g., $E$ is a edge set such that $G$ is a self-avoiding cycle consists of $m$ nodes) exists in $G$.}  




% For a given structure involving $m$ nodes, we use $G_j \in \mathcal{G}$ {  delete $ \in \mathcal{G}$ }for $j = 1, \ldots, \tbinom{d}{m} := M$ to denote all of the subgraph in $\mathcal{G}$ with $m$ nodes. %Specifically, we use $\mathcal{H}_{j0}$ to denote the graph set consisting of the graphs with the same node set as $G_j$ but without the given structure, say, a cycle, or a clique. For example, if we want to detect a triangle, then $m = 3$. Let the node set of $G_1$ be $V_1 = \{1,2,3\}$ and $e_{ij} = (i,j)$, then $\mathcal{H}_{j0}$ consists of $7$ graphs, say, $\mathcal{H}_{10} = \Bigl\{    \{V_1, \emptyset \}, \{V_1, \{e_{12}\} \} , \{V_1, \{ e_{13} \} \},  \{V_1, \{ e_{23} \} \},  \{V_1, \{e_{12}, e_{13} \}\}, \{V_1, \{e_{12}, e_{23} \}\} ,\{V_1, \{e_{13}, e_{23} \}\}  \Bigr\}$.

% {  A popular scientific problem is to test which nodes in a graph (denoted by $G$) form a structure of particular interests. Let $G^*=(V,E^*)$ be a graph of such structure. For example, $G^*$ is a triangle where we can write $V=\{1,2,3\}$, $E^*=\{(1,2),(1,3),(2,3)\}$.  We are interested in which nodes in $G$ form a triangle like $G^*$. %Note that we can write $E^*=f_{G^*}(V)$ where $f_{G^*}:V\mapsto \{(x,y):x,y\in V\}$ is a map such that the edges set $f_{G^*}(V)$ forms the structure $G^*$. 
% Denote the set of the subgraphs of $G$ each of which has the same number of nodes in $G^*$ by $S(|V|,G)=\Bigl\{(V_j,E_j): |V_j|=|V|, \, E_j=\{(x,y)\in E:x,y\in V_j\}\Bigr\}$. For $1\leq j\leq \tbinom{d}{|V|}$, let $P_j=\{\sigma:V\mapsto V_j\}$ be the set of all permutations from $V$ to $V_j$. formally speaking, we say $G_j=(V_j,E_j)\in S(|V|,G)$ has a structure of $G^*=(V,E^*)$ (denoted by $G^* \subseteq G_j$) if there exists a map  $\sigma\in P_j$ such that $\{(\sigma(x),\sigma(y)):(x,y)\in E^*\}\subseteq E_j$. 



% Therefore, the multiple testing for the structure problem is}
% \[
% H_{0j}: G^*\not \subseteq G_j,\qquad \mbox{ vs }\qquad H_{1j}: G^* \subseteq G_j,\qquad 1\leq j\leq \tbinom{d}{|V|}.
% \]
% \yue{denote $\mu=|V|$ and $J=\tbinom{d}{|V|}$ for now}

% Note that the $j$-th null hypothesis $H_{0j}$ on $G_j$ is equivalent for any permutations on the nodes $V_j$. To express the problem in a more processable way,  for $1\leq j\leq \tbinom{d}{|V|}$, introduce 
% \[
% E_j=\{f_{G^*}(\sigma(V_j)):\sigma\mbox{ is a permutation}\}
% \]
% as the set of all topology structure on nodes set ${V_j}$ that is  equivalent to the interested structure $E^*$ (i.e., the edge set of $G^*$). 
%{   Equivalently, we can reformula the above problem as the following multiple testing problem on the hidden structure $\Theta^{\star}$
% \[
% H_{0j}:\max_{E\in E_j }\Bigl\{\min\Bigl(\Theta^{\star}_{E}\Bigr)\Bigr\}=0,\qquad\mbox{vs}\qquad H_{1j}:\max_{E\in E_j}\Bigl\{\min\Bigl(\Theta^{\star}_{E}\Bigr)\Bigr\}>0,\qquad 1\leq j\leq \tbinom{d}{|V|},
% \]
% where we recall that $\Theta^{\star}_{E}$ denotes the set $\{\Theta^{\star}_{xy}:(x,y)\in E\}$. 
% }


% {\color{blue}Yue: Let $\mathcal{G} = (V, E)$ be the whole graph with $d$ nodes, $G_j = (V_j, E_j) \subseteq G$ be the $j$-th subgraph of $G$ (which means $V_j \subseteq V$ and $E_j \subseteq E$). $S_j=(V_j,E_j)$ is the $j$-th graph of interest (e.g., trangle, quadrilateral). Let $d_s=|V_j|$.

% In general, we aim to test 
% $$H_{0 j}: S_j \nsubseteq G_j \quad \text{ versus } \quad  H_{1 j}: S_j \subseteq G_j, \quad 1 \leq j \leq J := \tbinom{d}{d_s}$$

% Equivalently, we can test on $\Theta$.
% $$H_{0 j}: \min(|\Theta^*_{E_j}|)=0 \quad \text{ versus } \quad
% H_{1 j}: \min(|\Theta^*_{E_j}|)>0$$
% }


% Then the multiple hypotheses problem is formulated as $G_j \nsubseteq G$
% $$H_{0 j}: G_j \in \mathcal{H}_{j0} \quad \text{  v.s. } \quad  H_{1 j}: G_j \notin \mathcal{H}_{j0},$$
% for $j \in 1,\ldots, J$. For each $j \in[J]$, let $\psi_{j}=1$ if $H_{0 j}$ is rejected and $\psi_{j}=0$ otherwise. 


%{  initialize discussion the organization, first discuss the algorithm without the estimation of p-value. Then discuss the estimation of $p$-value starting from we have a $T^*$. and introduce two cases: mention GGM and ising model. Briefly discuss the conditions, needed for the $T$ statistics. Then discuss the p value of the two cases.}
\subsection{Algorithms}\label{sec:subalg}
In this section, we present our general methodology to select all subgraphs $F_j, j \in [J]$ that can be embedded into the true graph $G^*= (V, E^*)$.        %Let $W^*$ be the estimator for edge weights $W^*$, $\hat c (\alpha, E)$ be the estimator for $(1-\alpha)$-quantile of the maximum of $W^*$ over edge set $E$, and $ {\hat c}^{-1}(\tau, E)$ be the inverse function.
% estimator for $\mathbb{P}\big(T_{E} > \tau\big),$
% where
% \begin{equation}\label{eqn:TE}
% \yue 
% T_{E}=\sqrt{n}\max_{e \in E} \Bigl\{ \bigl|{\widetilde{\Theta}_{e}-\Theta^*_{e}}\bigr|\Bigr\}.    
% \end{equation}
% The details of estimation can be found in Section \ref{sec:application} for different applications. 
%We present our algorithm below in Algorithm~\ref{alg:1}. 
The main idea of our algorithm is to assign each subgraph in $\cF$ a $p$-value and then apply the Benjamini and Hochberg (BHq) procedure \citep{benjamini1995controlling} on the $J$ $p$-values to select the significant subgraphs. 

 Essentially, the most challenging part is to assign each subgraph with a $p$-value.  Compared to the estimation of the $p$-values of edges, the estimation of the $p$-value of  a graph structure requires combinatorial and uniform control on involved edges for multiple cases. As a result, the estimation of the $p$-values of edges   within and between structures  could be highly dependent.  To address this issue, maximal statistics have been used in the literature. However, computing $p$-values for maximal statistics can be computationally intensive and inefficient. For instance,  in \cite{zhang2021startrek}, they detect the hub nodes. To ensure uniform control on all possible cases of hub formation, they use maximal statistics to control the behaviors of possible edges in a hub. However, the distribution of maximal statistics is approximated through bootstrap, which requires heavy computational resources for sufficient accuracy.
Let $\{\alpha(F_j)\}_{j \in [J]}$ denote $p$-values for subgraphs $\{F_j\}_{j \in [J]}$. 
 In this paper, one of the significant discoveries is that for each subgraph $F \in \cF$ which has specific structure, its $p$-value can be simply defined as
\begin{equation}\label{eq:pvalueF}
\alpha(F)=\max_{e\in E(F)}p_e.    
\end{equation}
Here  $p_e$ denotes the $p$-value for edge $e$ and is shared across the calculations of the $p$-values of other subgraphs with overlapping edges. the estimation of edge $p$-values  from data $\bX$ in general can be separated into two scenarios, we  discuss it later in Section \ref{sec:estpvalue}.


The procedure of our Algorithm \ref{alg:1} is as follows. Suppose we have the estimated $p$-values of edges $\{p_e\}_{e \in E}$.  We begin with an initial full edge  set and initialize subgraph $p$-values $\alpha(F_j)=1$ for all $j\in [J]$. 

We then filter out edges with $p$-values greater than a threshold $q$, denoting the resulting set of edges as $E_{1}(q)= \big\{e\in E: p_e > q \big\}$. 
We only use \eqref{eq:pvalueF} to update those  $\alpha(F_j)$ values for subgraphs $F_j$ that can be embedded in the filtered graph $(V,E_1(q))$. Finally, we apply the BHq procedure to the set of updated $\alpha(F_j)$ values to select the significant subgraphs.

\begin{remark} \label{rmk:1}
Define $M:=\max_j|V(F_j)|$ as the maximal size of subgraphs of interest. By pre-screening edges in step $3$ of Algorithm \ref{alg:1}, we can significantly reduce the computational   from $\tbinom{d}{M}$ to less than $\tbinom{s}{M}$ where $s$ ($\ll d$ for sparse graphs) denotes the maximum degree in the filtered graph $(V,E_1(q))$.   It can be seen from \eqref{eq:pvalueF} that subgraphs involving edges with $p$-value larger than $q$ must have $p$-value larger than $q$ and are definitely insignificant in the BHq procedure, thus we can skip thecalculation of $p$-values for these subgraphs.
\end{remark}



% Because in order to detect subgraphs, we need to assign  $p$-values for subgraphs, which is highly dependent and thus challenging. So we start with estimating $p$-values for each edge. 

%For edges, as we introduced before, we have edge weight estimator $W^*$. 
% We start with a null edge set, and add edges one by one into our edge set from the largest-weighted edge to the smallest-weighted edge. %Each time an edge $e$ with weight $W^*_e$ is added,  we estimate $p$-value for this edge by considering all edges with smaller weights than this edge, i.e., $\{e':W^*_{e'} \leq W^*_e\}$,  since we are considering multiple edges and need uniform control over all edges.

% Then we estimate  $p$-values for subgraphs based on $p$-values for edges.
% % we let $p_k= \widehat{c}^{-1}\bigl(\sqrt{n} | \widetilde{\Theta}_{e_{(k)}}|, \{e_{(1)}, \ldots, e_{(k)}\}\bigr)$  being  the  $p$-value for edge  $e_{(k)}$, which is the edge with $k$-th smallest estimated weight in the candidate edge set $E = \{(u, v)\in E: u\neq v\}$.
% For subgraph $p$-values, in the process that we add edges one by one with weights from large to small into our edge set based on estimated weight, some subgraphs of interest (isomorphic to $F$) emerges. The first time one subgraph appears, we define $p$-value for this subgraph as the maximal edge $p$-values among all added edges. Here we need to choose the most conservative $p$-values since the existence of a subgraph depends on the least significant edge.
 

% Finally, we rank our estimated $p$-values for subgraphs $\alpha_1, \ldots, \alpha_J$, and obtain the rejection set for our multiple testing problem \eqref{eqn:hypo} by Benjamini and Hochberg (BHq) procedure \citep{benjamini1995controlling}.

%{  Compared to the methods in XXX, our procedure does not require }



%%%% Yue Sept 16
% \begin{algorithm}[H]
%     \caption{{   ALGORITHM NAME}  \label{alg:2}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     \For{$j = 1, \cdots, J$ }{
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     Let $ E_{0,j}= \big\{(j_1, j_2)\in V_j \times V_j: j_1\neq j_2\big\}$\; \label{line:start} % and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
    
%     We order the elements in the set $\bigl\{\big|\widetilde{\Theta}_e \big|:e\in {E_{0,j}}\bigr\}$ as $\big|\widetilde{\Theta}_{e_{(1)}}\big| \geq \big|\widetilde{\Theta}_{e_{(2)}}\big| \geq \ldots \geq \big|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}\big|$, where $\bigl|\widetilde{\Theta}_{e_{(k)}}\bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
%     % Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|, E^*_{j}\Bigr)$ where $E^*_{j}=\Bigl\{\ell \neq j:\Bigl|\widetilde{\Theta}_{j \ell}\Bigr| \leq\Bigr.$
%     % $\Bigl.\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|\Bigr\}$
    
%   Define $K_{j}=\min\Big\{1 \leq k \leq\left|E_{0,j}\right|:G_j \subseteq \big\{e_{(1)},  ..., e_{(k)}\big\}\Big\}$\;
   
%   Compute $\alpha_{uv}=\widehat{c}^{-1}\bigl(\sqrt{n} \big| \widetilde{\Theta}_{e_{(k)}}\big|, E_{j}^{(k)}\bigr)$  with $E_{j}^{(k)}=\big\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\big\}$, for $1 \leq k \leq K_{j}$\;
    
%     Let $\alpha_{j}=\max_{1 \leq k \leq K_{j}}\{\alpha_{uv}\}$\; \label{line:end}
%     }  
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
    
%     \vspace{10pt}
% % \begin{algorithmic}[1]
% %     \Function{Bisection}{$f,a,b,\epsilon$}
% %     \State foo
% %     \State bar
% %     \EndFunction
% %   \end{algorithmic}
  
% \SetKwFunction{FMain}{PValueEstimation}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{$F$}}{
%     $ S^{*}  \longleftarrow F $;    

%     \ForEach{$ F \in NPs $}
%     {\eIf{$ f_i = Negated $}
%         {$ N \longleftarrow f_i;$}
%         {$ S \longleftarrow f_i;$}

%     }
%     \textbf{return} $\alpha; $ 
% }
% \textbf{End Function}
% \end{algorithm}

%%% Jan 12
% \begin{algorithm}[H]
%     \caption{{   ALGORITHM NAME}  \label{alg:2}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     \For{$j = 1, \cdots, J$ }{
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
    
%     Let $\alpha_{j}=
% \texttt{PValueEstimation}(\widetilde\Theta, G_j(V_j,E_j))$\; 
%     }  
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
    
%     \vspace{10pt}

% \SetKwFunction{FMain}{PValueEstimation}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{$\widetilde\Theta,G'(V',E')$}}{
%   Let $ E_{0}= \big\{(j_1, j_2)\in V' \times V': j_1\neq j_2\big\}$\; 
    
%     We order the elements in the set $\bigl\{\big|\widetilde{\Theta}_e \big|:e\in {E_{0}}\bigr\}$ as $\big|\widetilde{\Theta}_{e_{(1)}}\big| \geq \big|\widetilde{\Theta}_{e_{(2)}}\big| \geq \ldots \geq \big|\widetilde{\Theta}_{e_{(|E_{0}|)}}\big|$, where $\bigl|\widetilde{\Theta}_{e_{(k)}}\bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;

    
%   Define $K=\min\Big\{1 \leq k \leq\left|E_{0}\right|:G' \subseteq \big\{e_{(1)},  ..., e_{(k)}\big\}\Big\}$\;
   
%   Compute $\alpha_{k}=\widehat{c}^{-1}\bigl(\sqrt{n} \big| \widetilde{\Theta}_{e_{(k)}}\big|, E^{(k)}\bigr)$  with $E^{(k)}=\big\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0}|)}\big\}$, for $1 \leq k \leq K$\;
    
%     Let $\alpha=\max_{1 \leq k \leq K}\{\alpha_{k}\}$\; 
    
%     \textbf{return} $\alpha; $ 
% }
% \textbf{End Function}
% \end{algorithm}

%%% Jan 13



\begin{algorithm}
    \caption{{General algorithm for subgraphs selection with FDR control} \label{alg:1}}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    Input: edge $p$-values $p_e$ for $e\in E$, FDR level $q$. 
    
    Initialize $\alpha_j = 1$ for $j \in [J]$\;
        
    Denote $E_{1}(q)= \big\{e\in E: p_e > q \big\}$\;
    % $E_{0}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| < \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$.
    %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$.
    % and  $G_1(q)=(V,E_1(q))$\;

    \For{$F \in \big\{F_j \in \cF:E(F_j) \subseteq  E_1(q),j\in [J] \big\} $}{
    %\If{$E(F_j) \subseteq  E_1(q)$
    %}{
    $\alpha(F)=\max_{e\in E(F)} p_e$\; 
    %}
    }
   
    Order $\alpha_{1},\ldots,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \ldots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$\;
    Let $j_{\max}=\max \bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\bigr\}$\;
    
    Output: Reject $H_{0j}$ for those $j$ such that $\alpha_{j} \leq \alpha_{(j_{\max})}$.  Reject nothing if $j_{\max}= 0$.
    
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{General estimation of $p$-values of edges}\label{sec:estpvalue}

In this section, we discuss how to estimate $p$-values for edges for the two scenarios of edge weights (continuous and discrete) as we have mentioned in Section \ref{sec:setup}.  Recall the Gaussian graphical model in Example \ref{ex:GGM}, edge weight $ W^*_{uv}:=\Theta^*_{uv}$ for any $(u,v)\in E$, and we have $W^*_{uv} \neq 0$ if and only if $(u,v) \in E^*$.
In the Ising model in Example \ref{ex:ising}, edge weight $W^*_{uv} := \E[X_uX_v]- \tanh \theta$, and we have $W^*_{uv} >0$ if and only if $(u,v) \in E^*$. These two specific  examples exemplify two general scenarios (two-sided and one-sided), which can be summarized as follows:
%
% In general, there are two types of graphical models. For example, in the Gaussian graphical model (GGM), $\Theta^*_{uv} \neq 0$ implies that $(u,v) \in E^*$. But in the Ferromagentic Ising model, $w^*_{uv} > 0$ implies $(u,v) \in E^*$.  However, $w^*_{uv}$ in \eqref{eqn:Ising} is not easy to estimate in practice. On the other hand, it has been shown that the correlation can characterize the edge via: $\E[X_uX_v]- \tanh \theta >0$ if and only if $w^*_{uv} >0$ \citep{neykov2019property}. So we will use the weight $W^*_{uv} = \E[X_uX_v]- \tanh \theta$, which is easier to estimate than $w^*_{uv}$.  So there are two kinds scenarios in our general testing procedure: two-sides for the weights in GGM and one-sided for Ising.
%
%{\color{red} Notice in the Gaussian graphical model, $\Theta^*_{jk} \neq 0$ implies that $(jk) \in E$ but in the Ferromagentic Ising model, $W{uv} > 0$ implies $(jk) \in E$.  However, w is not easy to estimate in practice. On the other hand, it can be shown that [cite] the correlation can characterize the edge via: $E[XuXv]- thatn >0$ if and only if XX. So we will use the weight $W = XXX$  So there are two kinds scenarios in our general testing procedure: two-sides for the weights in GMM and one-sided for Ising.}
%
% Recall that the true edge weights are $W^*:=\{W^*_e\}_{e\in E}$. The relationship between true edge weights and the true graph $G^*:=(V,E^*)$ can be separated into the following two scenarios
\begin{align*}
    \text{Scenario $(a)$: }& e\in E^* \text{ if and only if } W^*_e\neq 0; % \qquad \text{(e.g., Gaussian graphical model)} ; 
    \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \text{Scenario $(b)$: }& e\in E^* \text{ if and only if } W^*_e> 0. %\qquad  \text{(e.g., Ising model)}. 
\end{align*}
For the above two scenarios, suppose for each $e\in E$, we can construct an estimator $\hat{W}_e$ for true edge weight $W^*_e$ from the data $\bX_1,\ldots, \bX_n$, where $\hat{W}_e$ are expected to be asymptotically normal distribution with mean ${W}^*_e$.  {  Denote $\sigma_e^2$ as the asymptotic variance of $ \sqrt{n}\hat{W}_e$ and $\hat\sigma^2_e$ as its empirical estimator}.
%
The general assumptions that should be satisfied for $ \hat{W}_e$ and $\hat\sigma^2_e$  are presented later in Assumption \ref{assum:That:condition}.
%
Concrete examples of constructing $\hat{W}_e$ and $\hat{\sigma}_e$ from data $\bX_1,\ldots, \bX_n$ for Gaussian graphical models and Ising models  will be discussed later in Section \ref{sec:application}.  We estimate the $p$-values for edges using the following method:
\begin{align}\label{eq:That:condition0}
    \text{Scenario $(a)$: }& p_e=2\big(1-\Phi(|\sqrt{n}\hat{W}_e /\hat\sigma_e|)\big);\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \text{Scenario $(b)$: }& p_e=1-\Phi(\sqrt{n}\hat{W}_e/\hat\sigma_e).
\end{align} 

% \begin{remark}\label{rmk:1}
%     For ease of notation, we assume $\Var (\sqrt{n}\hat{W}_e) = 1$ without loss of generality. If not, we can simply use normalized weight $\hat{W}_e/\sqrt{\Var(\hat{W}_e)}$ and all the methodology and theoretical results can be generalized accordingly.
% \end{remark}
%if the estimator $\hat{W}$ satisfies the following assumption %Here $Q(\cdot)$ is the tail probability function of standard Gaussian that $Q(x)=\mathbb{P}(N(0,1)>x)$.

% We first impose an essential assumption on general test statistic $\hat T_e$.


%Other test statistics that does not satisfy the Assumption~\ref{assum:That:condition} may also be available.  \cite{neykov2019property} uses a conservative test, without normalizing the statistic.  We want to emphasis that the key of our Algorithm \ref{alg:1} is to construct reasonable estimate of $p$-value of edges even though it could be a conservative one.   In this paper, we only discuss one possible case that meets common tests, and  leave the generalization work on some specific models to the future.



% \begin{algorithm}[h]
%     \caption{   ALGORITHM}  \label{alg:2}
    
%     Input: $w$, $\hat c$, $\hat c^{-1}$, $\cV$, FDR level $q$. 
    
%     Initialize $\alpha_j = 1$ for $j \in [J]$\;
    
       
    
%     \For{$V\in \cV$}{
%     Update the $p$-values by $(\alpha_1, \ldots, \alpha_J)=\texttt{PValueEstimation}(w, V)$ \; 
%     }  
       
%     Order $\alpha_{1},\ldots,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \ldots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$\;
%     Let $j_{\max}=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$\;
    
%     Output: Reject $H_{0j}$ for those $j$ such that $\alpha_{j} \leq \alpha_{(j_{\max})}$.  Reject nothing if $j_{\max}= 0$.
    
%     \vspace{10pt}

% \SetKwFunction{FMain}{PValueEstimation}
% \SetKwRepeat{Do}{do}{while}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{$w,V$}}{
%       %Let $ E= \{(j, k)\in E: j\neq k\}$. %and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
%     Let $E = \{(u, v)\in E: u\neq v\}$\;
%     Order the edge weight estimators $\{ W{e}  : e \in E\}$ as $ W{e_{(1)}}   \leq \ldots  \leq  W{e_{(|E|)}}  $, where $ w_{e_{(k)}} $
%     denotes the $k$-th smallest estimator and $e_{(k)}$ denotes the corresponding edge\;
  
%     Initialize $k = |E|$; 
    
%     \Do{$p_{k+1}\le q$ or $k\ge 1$}{
%     Let $p_k= \widehat{c}^{-1}\bigl(\sqrt{n}   w_{e_{(k)}} , \{e_{(1)}, \ldots, e_{(k)}\}\bigr)$;
    
%     Find $I_k=\big\{ j \in [J] : F_j \subseteq (V,\{e_{(k)}, e_{(k+1)},\ldots, e_{(|E|)}\}) \big\}$\;
    
%     Update $\alpha_{j}=\max\{p_{k}, p_{k+1},\ldots,p_{|E|}\}$ for all $j \in I_k \backslash I_{k+1}$, where $I_{|E|+1}=\emptyset$\;
    
%     $k=k-1$\;
%     }
%     Output: $\{\alpha_j:1\leq j\leq J\}$.
% }  
% \textbf{End Function} 

% \end{algorithm}

% \begin{remark}
% Note that in Algorithm~\ref{alg:1}, by pre-screening edges, we avoid calculating the $p$-values of $F_j$ if one edge in $E(F_j)$ has $p$-value large than $q$. Because if the $p$-value for one edge is larger than $q$, based on our definition for subgraph $p$-values, we have that all subgraphs containing this edge will have $p$-values larger than $q$, which implies these subgraphs will never be selected in our algorithm. Thus it is the same as setting their $p$-values as 1.
% \end{remark}


% {   To understand the intuition, we provide a concrete example for Algorithm \ref{alg:2}. FIGURE HERE }


% Denote $\psi_{j,\alpha}=1$ if $\alpha_{j}\leq \alpha$ and $\psi_{j,\alpha}=0$ otherwise, for $1 \leq j \leq J$. 
% The above algorithm is equivalent to rejecting $H_{0j}$ if $\alpha_{j}\leq \hat\alpha$ where
% \begin{equation}\label{eqn:alphahat}
% \widehat{\alpha}=\sup \Bigl\{\alpha \in(0,1): \frac{\alpha J}{\max \Bigl\{1, \sum_{j \in [J]} \psi_{j, \alpha}\Bigr\}} \leq q\Bigr\},
% \end{equation}
% i.e.,  the rejection set  $\bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\bigr\}=\big\{j:  \alpha_{j}\leq \hat\alpha \big\}$. 
%
% \begin{proposition}\label{prop:1-2} 
% For $1\leq j\leq J$ and any specified significance level $\alpha \in (0,1)$, recall that  $\alpha_j$ is the estimated p-value defined in Algorithms \ref{alg:2}.  We have that  Algorithm \ref{alg:2} is equivalent to reject $H_{0j}$ if $\alpha_{j}\leq \hat\alpha$, i.e., the rejection set  $\bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\bigr\}=\big\{  \alpha_{j}\leq \hat\alpha \big\}$
%  where $\hat\alpha$ is defined in \eqref{eqn:alphahat}.
% \end{proposition}




% \begin{algorithm}[H]
%     \caption{{   Outline}  \label{alg:2.1}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     \For{$j = 1, \cdots, J$ }{
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     {   Obtain p-value $\alpha_{j}$ for subgraph $j$}    \; 
%     }  
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}


% \begin{algorithm}[H]
%     \caption{{   Obtain $\alpha_j$}  \label{alg:2.2}}
%     Let $ E_{0,j}= \big\{(j_1, j_2)\in V_j \times V_j: j_1\neq j_2\big\}$. %and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
    
%     We order the elements in the set $\bigl\{\big|\widetilde{\Theta}_e \big|:e\in {E_{0,j}}\bigr\}$ as $\big|\widetilde{\Theta}_{e_{(1)}}\big| \geq \big|\widetilde{\Theta}_{e_{(2)}}\big| \geq \ldots \geq \big|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}\big|$, where $\bigl|\widetilde{\Theta}_{e_{(k)}}\bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
    
%   Define $K_{j}=\min\Big\{1 \leq k \leq\left|E_{0,j}\right|:G_j \subseteq \big\{e_{(1)},  ..., e_{(k)}\big\}\Big\}$\;
   
%   Compute $\alpha_{uv}=\widehat{c}^{-1}\bigl(\sqrt{n} \big| \widetilde{\Theta}_{e_{(k)}}\big|, E_{j}^{(k)}\bigr)$  with $E_{j}^{(k)}=\big\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\big\}$, for $1 \leq k \leq K_{j}$\;
    
%     Let $\alpha_{j}=\max_{1 \leq k \leq K_{j}}\{\alpha_{uv}\}$    \; 
 
% \end{algorithm}



% \paragraph{   Pre-screening ALGORITHM}
% {In some extreme case, we may be interested in $\cV$ being the collection of all $|V(F)|$-element subset of $V$ . In this case, $\cV$ has $\binom{d}{|V(F)|}$ elements so $J=\binom{d}{|V(F)|}$, which will result in too many iterations in Algorithm \ref{alg:2} and will be computationally expensive. For example, we may aim to select all triangles from a graph and thus need to consider $\binom{d}{3}$ hypotheses.
% So next, we aim to deal with the computation issue and propose two ideas to make our algorithm more efficient.

% The first idea is pre-screening edges, i.e., removing edges with $p$-values larger than our pre-specified FDR level $q$. Intuitively, % since the true graph is sparse, there actually exists a large amount of edges with small estimated weights. So by doing the initial screening of edges at level $q$, we obtain a relatively sparse graph with screened edge set $E_1(q)$. The reason we can remove these edges is, 
% if the $p$-value for one edge is larger than $q$, then based on our definition for subgraph $p$-values, we have all subgraphs containing this edge will have $p$-values larger than $q$, so these graphs will never be selected by our algorithm. Thus, we can first remove these edges with $p$-values larger than  $q$, and skip some node sets in $\cV$ if there is no subgraph of interest with these node sets based on the screened edge set $E_1(q)$. 
% Note that by the pre-screening edge procedure, the algorithm is still equivalent with Algorithm~\ref{alg:2}. We will formally prove the equivalence in Proposition \ref{prop:2-3}. 
    

% The second idea to make our algorithm more efficient is running  the function \texttt{PValueEstimation} on a new collection of node set $\tilde \cV$ where elements in $\tilde \cV$ have larger cardinality than $|V(F)|$. Generally, we let $\tilde \cV$ be the collection of all $(d-c)$-element subset of $V$, where $c$ is a positive constant. % In an extreme case, we can let $\tilde \cV=\{V\}$, where we only need to run \texttt{PValueEstimation} once. 
% An example is letting $\tilde \cV$ be the collection of all $(d-1)$-element subset of $V$. Then the cardinality of $\tilde \cV$ is only $d$, i.e., we only need to run \texttt{PValueEstimation} $d$ times and the computation is thus much faster (than doing $\binom{d}{|V(F)|}$ iterations in Algorithm \ref{alg:2}). 




% However, with $\tilde \cV$, the algorithm will be more conservative because in each iteration $V \in \tilde \cV$, the cardinality of $V$ is larger, so the candidate edge set $E = \{(u, v)\in E: u\neq v\}$ will become larger. So based on the definition of edge $p$-value, $p$-values for edges will become larger, which will result in larger $p$-values for subgraphs.
   

% Based on the above two ideas, the formal algorithm is presented in Algorithm \ref{alg:3}.

% }







% We can further make Algorithm \ref{alg:2} more efficient by pre-screening the edges in the complete graph, and make the cardinality of elements in $\cV$ larger.   See Figure \ref{fig:screen} for illustration. In this figure, we have a graph with six nodes and we aim to select all triangles. (A) is the whole graph with all edges before  screening. In Algorithm \ref{alg:2}, we need to do 15 tests as there are 15 possible triangles. (B) is the sparse graph with less edges after screening. Based on this sparse graph, there are only two possible triangles (the yellow one and the blue one) as highlighted in (C) and we only have to consider these two tests.

% The formal algorithm is presented in Algorithm \ref{alg:3}. With much less tests to implement, Algorithm \ref{alg:3} is  much efficient than Algorithm \ref{alg:2}.

% \begin{figure}[h!]
% 	\begin{center}
% 		\begin{tabular}{cc}
% 		&{\quad\quad\quad\ \ (A) \quad\quad\quad\quad\quad\, (B) \quad\quad\quad\quad\quad\ \   (C) \quad\quad\quad\quad}\\
% 		&\includegraphics[width=.5\textwidth,angle=0]{./figure/screen} \\
% 			[-10pt]
% 		\end{tabular}
% 	\end{center}
% 	\caption{Illustration for the pre-screening edge procedure  in Algorithm \ref{alg:3}. Suppose we have a graph with six nodes and we aim to select all triangles from this graph. (A) is the whole graph with all edges before screening. As in Algorithm \ref{alg:2}, we need to do 15 tests as there are 15 possible triangles. (B) is the sparse graph with less edges after screening. Based on this sparse graph, there are only two possible triangles (the yellow one and the blue one) as highlighted in (C), so we only have to consider  two tests.}
% 	\label{fig:screen}
% \end{figure}

%%%% Yue Sept 16
% \begin{algorithm}[H]
%     \caption{{   VERSION 1} \label{alg:3}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
        
%     Denote $E_{1}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| \geq \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$.
%     % $E_{0}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| < \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$.
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$.
    
%     Denote screened graph $G_1(q)=(V,E_1(q))$.
      
%     \For{$j = 1, \cdots, J$}{
%     \eIf{$G_j \subseteq {G_{1}(q)}$ }{
%     $\alpha_{j}=
% \texttt{PValueEstimation}(\widetilde\Theta, G_j(V_j,E_j))$.
%     }
%     {$\alpha_j=1$.
%     }
    
    
%     % Let $ E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$. 
    
%     % We order the elements in the set $\Bigl\{|\widetilde{\Theta}_e|:e\in {E_{0,j}}\Bigr\}$ as $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}|$, where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
%     % denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
 
%     % Define $K_{j}=\min\big\{1 \leq k \leq\left|E_{0,j}\right|:G^* \subseteq \{e_{(1)},  ..., e_{(k)}\}\big\}$\;
   
%     % Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e_{(k)}}|, E_{j}^{(k)}\Bigr)$  with $E_{j}^{(k)}=\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\}$, for $1 \leq k \leq K_{j}$\;
    
%     % Let $\alpha_{j}=\max_{1 \leq k \leq K_{j}}\{\alpha_{uv}\}$    \; 
 
%     }
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}

% \begin{algorithm}[H]
%     \caption{Pre-screening {   ALGORITHM NAME} \label{alg:3}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     Denote $E_{1}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| \geq \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$,
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$
%     $E_{0}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| < \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$.
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$.
    
%     Let $G_1(q)=(V,E_1(q))$.
    
%     \For{$j = 1, \cdots, J$ where  $J:=\binom{d}{m}$}{
    
%     \If{$G_j \subseteq {G_{1}(q)}$ }{
%     Let $ E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$. 
    
%     We order the elements in the set $\Bigl\{|\widetilde{\Theta}_e|:e\in {E_{0,j}}\Bigr\}$ as $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}|$, where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
 
%     Define $K_{j}=\min\big\{1 \leq k \leq\left|E_{0,j}\right|:G^* \subseteq \{e_{(1)},  ..., e_{(k)}\}\big\}$\;
   
%     Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e_{(k)}}|, E_{j}^{(k)}\Bigr)$  with $E_{j}^{(k)}=\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\}$, for $1 \leq k \leq K_{j}$\;
    
%     Let $\alpha_{j}=\max_{1 \leq k \leq K_{j}}\{\alpha_{uv}\}$    \; 
    
%     }
%     }
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}

% \begin{algorithm}[H]
%     \caption{{   ALGORITHM} \label{alg:3}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
    
%     Input: $w$, $\tilde\cV$, FDR level $q$. 
    
%     Initialize $\alpha_j = 1$ for $j \in [J]$\;
        
%     Denote $E_{1}(q)= \Big\{e\in E: \sqrt{n}  w_{e}  \geq \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$\;
%     % $E_{0}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| < \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$.
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$.
%     % and  $G_1(q)=(V,E_1(q))$\;

%     \For{$V \in  \tilde\cV$}{
%     \If{
%     there exists $F_j, j \in [J]$ such that $F_j \subseteq \big(V, \{E\} \cap E_1(q) \big)$
%     }{
%     Update the $p$-values by $(\alpha_1, \ldots, \alpha_J)=\texttt{PValueEstimation}(w, V)$\; 
%     }
%     }
   
%     Order $\alpha_{1},\ldots,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \ldots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$\;
%     Let $j_{\max}=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$\;
    
%     Output: Reject $H_{0j}$ for those $j$ such that $\alpha_{j} \leq \alpha_{(j_{\max})}$.  Reject nothing if $j_{\max}= 0$.
    
% \end{algorithm}


% \begin{algorithm}[H]
%     \caption{{   VERSION 3} \label{alg:4}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
        
%     Denote $E_{1}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| \geq \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$\;
%     % $E_{0}(q)= \Big\{e\in E: \sqrt{n}|\widetilde{\Theta}_{e}| < \widehat{c}\bigl(q, \{e\}\bigr) \Big\}$.
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$.
    
%     Denote screened graph $G_1(q)=(V,E_1(q))$\;
    
%      Let $\mathcal{I}=\big\{j \in [J]: G_j \subseteq {G_{1}(q)}\big\}$.
     
%     \For{$j \in\mathcal{I}$}{
%     $\alpha_{j}=
% \texttt{PValueEstimation}(\widetilde\Theta, G_j(V_j,E_j))$.
%     }

   
%     Order $\alpha_{\mathcal{I}}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(|\mathcal{I}|)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq |\mathcal{I}|: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\bigl\{j \in \mathcal{I}: \alpha_{j} \leq \alpha_{(j_{\max })}\bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}  

% \begin{remark}
% \yue{
% Intuitively, in Algorithm \ref{alg:3}, we do not need to update $p$-values by running \texttt{PValueEstimation} for all elements in $\cV$.  In the beginning of  Algorithm \ref{alg:3}, we first do the initial screening of edges at level $q$  and remove edges with $p$-values larger than $q$. 
% Then we can just skip some node sets in $\cV$ if there is no subgraph of interest with these node sets based on $E_1(q)$. Thus, we define a new node set $\tilde \cV \subseteq \cV$, and run the function \texttt{PValueEstimation} for $\tilde \cV$.
% }
% \end{remark}

% \begin{algorithm}[htbp]
%     \caption{Test $j$-th subgraph \label{alg:1}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$, $E_j$,  significance level $\alpha$. }
%     Initialize {  $t=0,\, E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$, and $E_{0,j}^c=\emptyset.$}%\{(j_1, j_2)\in V_j \times V_j:j_1\neq j_2\}$}. %\{(j_1, j_2): \text{all edges between the $j$-th set of nodes $V_j$}\}$.
   
%     \Repeat{${  G^* \subseteq  (V_j,E_{t,j}^{c})} \mbox{ or } \mathcal{R}=\varnothing$}
%     { 
%     $t \leftarrow t+1$\;
    
%     Select the rejected edges $\mathcal{R} \leftarrow\Bigl\{(j_1, j_2) \in E_{t-1,j}:\,\sqrt{n}| \widetilde{{\Theta}}_{j_1 j_2}\big|>\widehat{c}\Bigl(\alpha, E_{t-1,j}\Bigr)\Bigr\}$\;
    
%     $E_{t,j} \leftarrow E_{t-1,j} \backslash \mathcal{R}$ and  $E_{t,j}^c \leftarrow E_{t-1,j}^c \cup \mathcal{R}$\;
%     }
%   	\Output{$\psi_{j, \alpha}=1$ if $G^* \subseteq{  (V_j,E_{t,j}^{c})}$, $\psi_{j, \alpha}=0$ otherwise.}%$G^* \subseteq E_{t,j}^{c}$, $\psi_{j, \alpha}=0$ otherwise.}
% \end{algorithm}


% {  Note that for each structure $G^*$, we may need an additional algorithm to test if $G^* \subseteq  (V_j,E_{t,j}^{c})$. We will discuss this later.}
% \begin{algorithm}[htbp]
%     \caption{Select structures of interest with FDR control \label{alg:2}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     \For{$j = 1, \cdots, J$ and $\sigma_{jl} \in  P_j$ where  $J:=\binom{d}{|V|}$, $l=1,\ldots,|P_j|$ and $P_j:=\{\sigma:V\mapsto V_j\}$}{
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     Let $ E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$. %and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
    
%     We order the elements in the set $\Bigl\{|\widetilde{\Theta}_e|:e\in {E_{0,j}}\Bigr\}$ as $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}|$, where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
%     % Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|, E^*_{j}\Bigr)$ where $E^*_{j}=\Bigl\{\ell \neq j:\Bigl|\widetilde{\Theta}_{j \ell}\Bigr| \leq\Bigr.$
%     % $\Bigl.\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|\Bigr\}$
    
%     \For{$\sigma_{jl} \in  P_j$ where $l=1,\ldots,|P_j|$ and $P_j:=\{\sigma:V\mapsto V_j\}$}{Let $ E^*_{jl} = \Bigl\{\Bigl(\sigma_{jl}(x), \sigma_{jl}(y)\Bigr): (x,y)\in E^* \Bigr\}$\;
    
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     For $k$ \mbox{ satisfying }  $e_{(k)} \in \cup_{1\leq l\leq |P_j|}E^*_{jl}$, compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e_{(k)}}|, E_{0,uv}\Bigr)$  with $E_{0,uv}=\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\}$\;
%     }
%     Let $\alpha_{j}=\min_{1\leq l \leq |P_j|}\max_{e_{(k)} \in E^*_{jl}}\{\alpha_{uv}\}$\; 
%     }  
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}

\iffalse

 \begin{algorithm}[htbp]
     \caption{Test $j$-th subgraph \label{alg:12} (more exact version)}
     \SetKwInOut{Input}{Input}
     \SetKwInOut{Output}{Output}
     \Input{$\widetilde{{\Theta}}$, $E_j$,  significance level $\alpha$. }
     
     \For{ $\sigma_{jl} \in  P_j:=\{\sigma:V\mapsto V_j\}$}{
     Initialize {  $t=0,\, E_{0,jl}= E^*_{jl}$, and $E_{0,jl}^c=\emptyset.$}%\{(j_1, j_2)\in V_j \times V_j:j_1\neq j_2\}$}. %\{(j_1, j_2): \text{all edges between the $j$-th set of nodes $V_j$}\}$.
   
     \Repeat{${  G^* \subseteq  (V_j,E_{t,jl}^{c})} \mbox{ or } \mathcal{R}=\varnothing$}
     { 
     $t \leftarrow t+1$\;
    
     Select the rejected edges $\mathcal{R} \leftarrow\Bigl\{(j_1, j_2) \in E_{t-1,jl}:\,\sqrt{n}| \widetilde{{\Theta}}_{j_1 j_2}\big|>\widehat{c}\Bigl(\alpha, E_{t-1,jl}\Bigr)\Bigr\}$\;
    
    $E_{t,jl} \leftarrow E_{t-1,jl} \backslash \mathcal{R}$ and  $E_{t,jl}^c \leftarrow E_{t-1,jl}^c \cup \mathcal{R}$\;
     }
     If $G^* \subseteq{  (V_j,E_{t,jl}^{c})}$, break\;
   	}
   	\Output{$\psi_{j, \alpha}=1$ if $G^* \subseteq{  (V_j,E_{t,jl}^{c})}$, $\psi_{j, \alpha}=0$ otherwise.}%$G^* \subseteq E_{t,j}^{c}$, $\psi_{j, \alpha}=0$ otherwise.}
 \end{algorithm}

 \begin{algorithm}[htbp]
     \caption{Select structures of interest with FDR control (more exact version) }\label{alg:22}
     \SetKwInOut{Input}{Input}
     \SetKwInOut{Output}{Output}
     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
     \For{$j = 1, \cdots, J$ and $\sigma_{jl} \in  P_j$ where  $J:=\binom{d}{|V|}$, $l=1,\ldots,|P_j|$ and $P_j:=\{\sigma:V\mapsto V_j\}$}{
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     Let $ E^*_{jl} = \Bigl\{\Bigl(\sigma_{jl}(x), \sigma_{jl}(y)\Bigr): (x,y)\in E^* \Bigr\}$. %and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
         We order the elements in the set $\Bigl\{|\widetilde{\Theta}_e|:e\in {E^*_{jl}}\Bigr\}$ as $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E^*_{jl}|)}}|$, where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge. \;
    %  Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|, E^*_{j}\Bigr)$ where $E^*_{j}=\Bigl\{\ell \neq j:\Bigl|\widetilde{\Theta}_{j \ell}\Bigr| \leq\Bigr.$ $\Bigl.\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|\Bigr\}$
     Compute $\alpha_{jlk}=\widehat{c}^{-1}\Bigl(\sqrt{n} | \widetilde{\Theta}_{e_{(k)}}|, E^*_{jlk}\Bigr), 1\leq k \leq |E^*_{jl}|$ with $E^*_{jlk}=\{e_{(k)}, e_{(k+1)}, ..., e_{(|E^*_{jl}|)}\}$\;
     Let $\alpha_{j}=\min_{1\leq l \leq |P_j|}\max_{1\leq k \leq |E^*_{jl}|}\{\alpha_{jlk}\}$\; 
     }  
    
     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
 \end{algorithm}
\fi

% \begin{algorithm}[htbp]
%     \caption{Test $j$-th subgraph \label{alg:1}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\{\widetilde{{\Theta}}\}$,  significance level $\alpha$. }
  	
%   	\Output{$\psi_{j, \alpha}=1$ if $\min_{e \in E_{j}} \Bigl\{\sqrt{n}| \widetilde{{\Theta}}_{e}| >\widehat{c}\Bigl(\alpha, E_{j}\Bigr)\Bigr\}$ and $\psi_{j, \alpha}=0$ otherwise.}
% \end{algorithm}


    

% The following proposition shows that Algorithms \ref{alg:2} and  \ref{alg:3} are equivalent if $\tilde\cV = \cV$. The proof of Proposition  \ref{prop:2-3} can be found in Section \ref{pf:prop:2-3}.


% \begin{proposition}\label{prop:1-2} 
% For $1\leq j\leq J$ and any specified significance level $\alpha \in (0,1)$, recall that $\psi_{j,\alpha}$ is  the result of $j$-th test  defined in Algorithms \ref{alg:1}, and $\alpha_j$ is the estimated p-value defined in Algorithms \ref{alg:2}.  We have that
% $\psi_{j,\alpha}=1$ if and only if $\alpha_j\leq \alpha$, i.e., Algorithms \ref{alg:1} and \ref{alg:2} are equivalent.

% \end{proposition}


% \begin{proposition}[]\label{prop:2-3} 
% With the same edge weight estimator $w$, pre-specified FDR level $q$ and $\tilde\cV = \cV$, we have that Algorithms \ref{alg:2} and \ref{alg:3} are equivalent, i.e.,  the rejection sets for two algorithms   are the same.
% \end{proposition}



% \begin{lemma}[Single test analysis]\label{lem:test}
% Under the same conditions as in Lemma 2.1 of \cite{zhang2021startrek}, for each $j$-th single test in Algorithm \ref{alg:1}, we have the following results on type I error and power.

% (i) Under the alternative hypothesis $H_{1,j}$, assuming $\min_{\{e \in V_j \times V_j: \Theta^*_{e}\neq 0\}}\{| \Theta^*_{e}|\} > 2C_{0} \sqrt{\frac{\log d}{n}}$ for some positive constant $C_0$, for $   \alpha=w(d^{-|V|})$
% \begin{equation*}
% \min_{{   j \in [J]}} 
% \mathbb{P}\Bigl(\psi_{j, \alpha}=1\Bigr) \rightarrow 1.    
% \end{equation*}

% (ii) Under the null hypothesis $H_{0,j}$, we have
% \begin{equation*}
% \lim _{(n, d) \rightarrow \infty} \P\Bigl(\psi_{j, \alpha}=1\Bigr) \leq \alpha.    
% \end{equation*}

% \end{lemma}


% {  If we need to add the rate of convergence (e.g., $o(d^{-|V|})$). Here $\min_{\{e \in E: \Theta^*_{e}\neq 0\}} \{| \Theta^*_{e}| \}> 2C_{0} \sqrt{\frac{\log d}{n}}$ is the signal strength condition for power analysis.}


\section{General theoretical results for subgraph selection}\label{sec:thm}
In this section, we will first introduce the assumptions that underlie our algorithm, and then we will present the statistical properties of the algorithm.
%
Recall that our goal is to control FDR in multiple testing problem \eqref{eqn:hypo}, we need to first impose some assumptions on the estimator $\hat{W}_e$. To be specific, we need the asymptotic normality of $\hat W_e$. we impose the following assumptions.

\begin{assumption}[General assumption on the test statistic]\label{assum:That:condition}
For some constant $C>0$, $\hat{W}_e$ satisfies that 
\begin{equation}\label{eq:That:condition}
    \mathbb{P}\Bigl( \sup_{e\in E}\frac{\big|\hat{W}_e-W_e-W^*_e\big|}{\sigma_e}\leq\frac{C}{\sqrt{n\log d}},
\ 
\sup_{e\in E}\Big|\frac{\sigma_e}{\hat{\sigma}_e}-1\Big|\leq \frac{C}{\log d} \Bigr)=1-o(1),
 \end{equation}
 where
\begin{equation}
W_e:=\frac{1}{n}\sum_{i=1}^n\xi_{i}(e), 
\ 
%   \sigma_e^2 = \lim \Var( \sqrt{n}\hat{W}_e).%, \ \hat\sigma^2_e \text{ is empirical estimator of } \sigma_e^2.  
\end{equation}   
% \begin{equation}
%     \mathbb{P}\Bigl( \sup_{e\in E} \big|{  \frac{\hat{W}_e-W^*_e}{\mathrm{sd}(\hat{W}_e)}-W_e}\big|>\frac{C}{\sqrt{n\log d}}\Bigr)=o(1),\qquad\text{with }W_e:=\frac{1}{n}\sum_{i=1}^n\xi_{i}(e),
% \end{equation}   
for each edge $e\in E$, and $\xi_{i}(e)$, $i = 1, 2, \ldots, n$ are i.i.d. random variables with bounded $\psi_1$-orlicz norm. %We also assume $\max_{e \in {E}} \sigma_e \leq C$ for some constant  $C$. %$c \leq \min_{e \in {E}} \sigma_e \leq \max_{e \in {E}} \sigma_e \leq C$ for some constants $c$ and $C$.
 \end{assumption}


Intuitively, $\hat W_e$ is composed of three parts: (1) dominating error $W_e$, which is asymptotically normal; (2) $W^*_e$, the true edge weight; (3) the remainder term, which is at the order of $1/\sqrt{n\log d}$. Here $O(1/\sqrt{n})$ is a standard convergence rate for $n$ samples  in statistical inference, and $1/\sqrt{\log d}$ is to control the multiplicity of hypotheses in \eqref{eqn:hypo}.
Such decomposition has been achieved under different graphical models \citep{van2014asymptotically, neykov2019property}.  We refer to Section \ref{sec:application} for the concrete example of edge weight estimator $\hat W_e$ under the Gaussian graphical model  and the Ising model. 


Next, we introduce signal strength condition. We define
\begin{align}\label{eqn:h1tilde}
    \text{Scenario $(a)$: }&\widetilde{{\cal H}}_1=
\Big\{j\in {\cal H}_1:{ \min_{e\in E(F_j)}|W^*_e|} \geq \sqrt{C(\log d)/n} \Big\};\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\text{Scenario $(b)$: }&\widetilde{{\cal H}}_1=
\Big\{j\in {\cal H}_1: \min_{e\in E(F_j)}{ W^*_e} \geq \sqrt{C(\log d)/n} \Big\},
\end{align} 
where $\widetilde{{\cal H}}_1$ the set of hypotheses such that all edges in the subgraph satisfy the sufficient signal conditions.

Then we aim to characterize the dependence in multiple testing \eqref{eqn:hypo}. 
Recall that $\xi_1(\cdot)$ is defined in \eqref{eq:That:condition}. We introduce $N_j=\{e\in E(F_j):W^*_e=0\}$, $j=1,2,\ldots,J$, which is the null edge set of the structure $F_j$ in the graph $G^*$. Let $e_j$ be some edge in set $N_j$ for $j \in {\cal H}_0$. To quantify the dependence, we define the following dependence set that captures the dependence between null hypotheses:
\begin{equation}
 \begin{aligned}
   S(\{e_{j}\}_{j \in \cH_0})=
& \Big\{
 (j_1,j_2)\in {\cal H}_0 \times {\cal H}_0: j_1\neq j_2, \\
& \big|\text{Cov}(\xi_1(e_{j_1}),\xi_1(e_{j_2})) \big|\geq C(\log d)^{-2-\gamma} \Big\}  
 \end{aligned}   
\end{equation}
for some constant $C$ and $\gamma>0$. Intuitively, for $(j_1,j_2)\in {\cal H}_0 \times {\cal H}_0$ and edges $e_{j_1} \in N_{j_1}, e_{j_2} \in N_{j_2}$,  $|\text{Cov}(\xi_1(e_{j_1}),\xi_1(e_{j_2}))|\geq C\log d^{-2-\gamma}$ means that the covariance between the pair of edges $(e_{j_1}, e_{j_2})$ is large, which implies that the null hypotheses $H_{0j_1}$ and $H_{0j_2}$ are somehow ``dependent'' or ``correlated''.
% 
The cardinality of $S(\{e_{j}\}_{j \in \cH_0})$ quantifies the dependence between weight estimators in null hypotheses. We aim to choose one edge $e_j$ for each $N_j$ such that the cardinality of $S(\{e_{j}\}_{j \in \cH_0})$ is minimized. This gives us the following quantity that captures the dependence among null hypotheses:
\begin{equation}\label{eq:S}
 \begin{aligned}
S = \min \Big\{ \big|S(\{e_{j}\}_{j \in \cH_0})\big|: & \text{ for all possible choices of} \\
& e_j \in N_j, j \in \cH_0 \Big\}.
\end{aligned}
\end{equation}
We will quantify the magnitude $S$ under the Gaussian graphical model and the Ising model in Sections \ref{sec:example:GGM} and  \ref{sec:example:Ising}, respectively.




% We introduce  We also define $N_j=\{e\in E(F_j):W^*_e=0\}$, $j=1,2,\ldots,J$, which is the null edge set of structure $F_j$ in the graph  $G^*$.

% Recall that $\xi_1(\cdot)$ is defined in \eqref{eq:That:condition}. Introduce $\widetilde{\cal H}_1=\{j\in {\cal H}_1:|W^*_e|>\sqrt{4(\log d)/n},e\in E(F_j)\}$ and $N_j=\{e\in E(F_j):W^*_e=0\}$,   $j=1,2,\ldots,J$. We can interpret $\widetilde{\cal H}_1$ as the set of alternative hypotheses satisfying sufficient signal conditions and $N_j$ is the null edge set of structure $F_j$ in the graph  $G^*$. Further, we define a set that captures the dependence between null hypotheses by
% \[
% S=\min_{\{e_j\in N_j:j\in{\cal H}_0\}}\big|\{(j_1,j_2)\in {\cal H}_0 \times {\cal H}_0: j_1\neq j_2, |\text{Cov}(\xi_1(e_{j_1}),\xi_1(e_{j_2}))|\geq C\log d^{-2-\gamma} \}\big|.
% \]

% Define $N_j$. Let $e_j$ be some edge in $N_j$ for j in $H_0$. We define the set XXXXXXX
% \[
% S(\{e_{j}\}_{j \in \cH_0})=\{(j_1,j_2)\in {\cal H}_0 \times {\cal H}_0: j_1\neq j_2, |\text{Cov}(\xi_1(e_{j_1}),\xi_1(e_{j_2}))|\geq C\log d^{-2-\gamma} \}
% \]
% for some constant $C$ and $\gamma>0$. {   intuition: pair of edges with large cov}. The cardinality of $S$ characterizes the how dependent between weight estimators in null hypotheses. We aim to choose one edge $e_j$ for each $N_j$ such that the cardinality of S is minimized. This gives us the following quantity:
% \[
% S = \min \{ |S(\{e_{j}\}_{j \in \cH_0})|: \text{ for all possible choices of $e_j \in N_j, j \in \cH_0$} \}
% \]
\color{black}
    

Next we present the trade-off between quantities $|\cH_0|, |\cH_1|, |\tilde \cH_1|$ and $S$. 
Recall that $\cH_0=\bigl\{1\leq j \leq J \biggiven  F_j \not\subseteq G^* \bigr\}$, ${\cal H}_1=\bigl\{1\leq j \leq J \biggiven  F_j \subseteq G^* \bigr\}$ and $\widetilde{{\cal H}}_1 \subseteq \cH_1$ is defined in \eqref{eqn:h1tilde}. To control the sparsity effect and dependence effect of the problem, we assume the following condition.
\begin{assumption}[Sparsity and dependence conditions]\label{ass:spadepend} 
We assume   
\[ 
\underbrace{ \frac{|{\cal H}_0| + |{\cal H}_1|}{|{\cal H}_0|\cdot |\widetilde{{\cal H}}_1|}}_{\text{Sparsity effect}} +\underbrace{S\frac{|{\cal H}_0| + |\cH_1|}{|{\cal H}_0|^2|\widetilde{{\cal H}}_1|}}_{\text{Dependence effect}}=o\Big(\frac{1}{\log d}\Big).
\]
\end{assumption}
Assumption \ref{ass:spadepend} comprises two conditions.  The first condition is about signal strength. In specific, when $|\cH_0|$ are at the same order of $|\cH_0| + |\cH_1|\asymp d^M$ where $M$ is defined in Remark \ref{rmk:1}, the first condition requires $|\tilde \cH_1| = \omega(\log d)$. This means we only need a small proportion of true alternative hypotheses with strong signal strength.
% 
The second condition is about dependence. 
Recall that the quantity $S$ represents the dependence level among null hypotheses. Intuitively, When $S$ is larger, indicating higher dependence, the multiple testing problem is more challenging.  To be specific, when $|\cH_0|$ is at the same order of $|\cH_0| + |\cH_1|$, Assumption~\ref{ass:spadepend} requires $S = o\Big(\frac{|{\cal H}_0| \cdot |\widetilde{{\cal H}}_1|}{\log d}\Big)$.
In Propositions \ref{prop:GGM} and \ref{prop:Ising}, we show that this condition can be achieved   for a wide range of Gaussian graphical models and the Ising models.


\color{black}
% By definitions, $\widetilde{{\cal H}}_1 \subseteq \cH_1$ can be interpreted as the set of alternative hypotheses that have strong signals.  $|\widetilde{{\cal H}}_1|$ is just to count the number of alternative hypotheses with signals larger than $ \sqrt{4\log d/n}$. 
% % containing true alternative hypotheses where all edges of these subgraphs have signal strength  exceeding $\sqrt{\log d/n}$.
% We also need a trade-off between $|{\cal H}_0|$ and  $|\widetilde{{\cal H}}_1|$. Because for the sparsity condition  in Assumption \ref{ass:spadepend} to hold, the ideal case is that both $|{\cal H}_0|$ and $\tilde |{\cal H}_1|$ are large, while there is a natural constraint that  $|{\cal H}_0| + |\widetilde{{\cal H}}_1| \leq J$. So there is a balance between  $|{\cal H}_0|$ and $|\widetilde{{\cal H}}_1|$ should be achieved. As for the dependence
%  part, recall that the quantity $S$ represents the dependence level. Intuitively, when $S$ is larger, i.e., dependence is higher, the multiple testing problem is harder. So as in Assumption \ref{ass:spadepend},
% $S$ can not be too large.
%  We will see later in Section \ref{sec:application} that it is a mild assumption both for Gaussian graphical models and Ising models that $S=O(s^2|{\cal H}_0|d^{M-2})$. And so if we can have $|\widetilde{{\cal H}}_1|\gg (s^2\log d/d^2)J$ and $|{\cal H}_0|\geq C J$ (i.e., the alternative hypotheses satisfying signal strengthen are not too little), then Assumption \ref{ass:spadepend} holds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Based on Algorithm \ref{alg:1}, the following theorem provides a bound on the tail probability of FDP and FDR.
\begin{restatable}[General FDR control]{theorem}{thmgeneralfdp}\label{thm:generalfdp} 
 Suppose $\log d/\log n=O(1)$. Under Assumptions~\ref{assum:That:condition} and~\ref{ass:spadepend}, we have that the $\{\psi_j\}_{j \in [J]}$ determined by Algorithm \ref{alg:1} satisfies
\[
\text{FDP}\leq q\frac{|{\cal H}_0|}{J}+o_{P}(1),\qquad \text{FDR}\leq q\frac{|{\cal H}_0|}{J}+o(1).
\]
%where $|{\cal H}_0|=|{\cal H}_0|$ and $J=|{\cal H}_0|+|{\cal H}_1|$.

\end{restatable}
The theorem guarantees asymptotic control over the tail probability of FDP and FDR  if the dimension of the graph is bounded by $n^C$ for some constant $C>0$,  the edge weight estimator satisfies certain regularity conditions, and certain sparsity and dependence conditions hold. The proof of this theorem is deferred to Section \ref{sec:pfthm:generalfdp} in the appendix. 
  
In addition, for the power performance of our algorithm, which measure the ability of discovering true subgraphs, we  have the following theorem.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}[Power Analysis]{theorem}{thmpower}\label{thm:power}
For $\{\psi_j\}_{j \in [J]}$ determined by Algorithm \ref{alg:1}, under the same conditions of Theorem \ref{thm:generalfdp},  we have %for any $\alpha \in [q/J,q]$,
\begin{equation*}
\mathbb{P}\Bigl(\psi_j=1,\text{ for all }j\in \widetilde{{\cal H}}_1\Bigr) = 1 -  o(1),
\end{equation*}   
where $\widetilde{{\cal H}}_1$ is defined in \eqref{eqn:h1tilde}.
\end{restatable}
This theorem guarantees that the true alternative hypotheses satisfying certain signal strength condition will be selected with probability going to $1$. The proof of this theorem can be found in Section \ref{sec:pfthm:power} in the appendix.

% \begin{assumption}[Scaling condition]\label{ass:scaling}
% We assume the following conditions hold:
% \begin{equation}\label{eqn:scaling}
% \frac{\log d }{\rho} \cdot \bigg( \frac{(\log d)^{19 / 6}}{n^{1 / 6}} + \frac{(\log d)^{11 / 6} }{n^{1 / 6} \rho^{1 / 3}} + s\frac{(\log d)^{3} }{\sqrt{n}}  + \frac{1}{d^{   m+1} \rho^{1/3}} + \frac{1}{|{\cal H}_0|} \bigg) = o(1).  
% \end{equation} 
% {   check scaling}
% Here for Gaussian graphical models, \begin{equation}\label{eqn:tilde H_1}
% \tilde{\mathcal{H}}_{1}:=\Bigl\{j \in \mathcal{H}_{1}: \forall e \in E(F_j),  \bigl|\Theta^*_{e}^*\bigr|> C_0 \sqrt{\log d / n}\Bigr\} \subseteq \cH_1, 
% \end{equation}
% for Ising models,
% \begin{equation}
% \tilde{\mathcal{H}}_{1}:=\bigg\{j \in \mathcal{H}_{1}: \forall e \in E(F_j),     M^*_{e} > \tanh(\theta) \bigg\} 
% \end{equation}
% and $\rho=\frac{|\tilde{\mathcal{H}}_{1}|}{J}$ is the proportion of  true subgraphs have signal strength exceeding $\sqrt{\log d/n}$ in all hypotheses.
% {   1. Check need to add assumptions on $\theta$, 2. Unify 4.2 and 4.3}
% \end{assumption}

%  \yue{unify (4.2) (4.3)}
 
%  \yue{condition is $W^*>0$ or $>\sqrt{\log d/n}$ }
 
% Condition \eqref{eqn:scaling} is the scaling condition required for validity of maximum quantile estimation by Gaussian bootstrap procedure \cite{Chernozhukov2013Gaussian}.
% Note that $\tilde \cH_1$ is defined in \eqref{eqn:tilde H_1} and $\rho=\frac{|\tilde{\mathcal{H}}_{1}|}{J}$.  Here for condition \eqref{eqn:scaling} to hold, we do not need signal strength for all true subgraphs, and we only require the proportion $\rho$  satisfying similar condition as in (5.4) in \cite{zhang2021startrek}.
% See detailed discussions in \cite{zhang2021startrek}.
% {  
% For example, let $J:=\binom{d}{m}$ and $|\cH_0|$ both be at the order of $O(d^m)$,
% we require
% \begin{equation}   
% |\widetilde{{\cal H}}_1| = w \bigg(  
%  \frac{d^m (\log d)^{25 / 6}}{n^{1 / 6}} + {\frac{d^{m} (\log d)^{17 / 8}}{n^{1 / 8} }} + 
%  s\frac{d^m (\log d)^{4} }{\sqrt{n}} + 
%   d^{(m-1)/2}\sqrt{\log d} + \log d \bigg) 
% \end{equation} 
% for  \eqref{eqn:scaling}  to hold.
% }
  %
  \section{Examples for Gaussian Graphical Model and Ising Model }\label{sec:application}
%  \subsection{Theoretical guarantee for subgraphs selection under  GGM}
  


In this section, we illustrate our general inferential framework on two class of  models: Gaussian graphical models and high-temperature Ising models.    

\subsection{Subgraph selection on Gaussian graphical models}\label{sec:example:GGM}
In the Gaussian graphical model introduced in Example \ref{ex:GGM}, 
% the random vector $\bX$ follows a multivariate Gaussian distribution $N_d(\bm{0},\Sigma^*)$ with mean vector $\bm{0}$ and covariance matrix $\Sigma^*$.
% 
% Let the precision matrix $\Theta^* = {\Sigma^*}^{-1}$ and define the weighted graph by $W^*_{uv}=\Theta^*_{uv}/\sqrt{\Theta^*_{uu}\Theta^*_{v v}}$ for any $(u,v)\in E^*$. 
we have $W^*_{uv}=0$ if and only if $(u,v) \notin E^*$ where $ W^*_{uv}:=\Theta^*_{uv}$. 
We consider the following parameter space for the precision matrices
\begin{equation}\label{eqn:us}
\mathcal{U}(s)=\Big\{\Theta^* \in \mathbb{R}^{d \times d} \mid 1/\rho \leq \lambda(\Theta^*) \leq \rho, 
\max_{j \in[d]} \|\Theta^*_{\cdot j}\|_{0} \leq s,\|\Theta^*\|_{1} \leq M \Big\},
\end{equation} 
which requires $\Theta^*$ has at most $s$ non-zero entries per column, and therefore the induced graph have maximum degree at most $s$.
%
Also, we assume $1/\rho \leq \lambda(\Theta^*) \leq \rho$, which  means that $\lambda_{\min }(\Theta^*) \geq 1 / \rho$ and $\lambda_{\max }(\Theta^*) \leq \rho$, i.e., the minimum and maximum eigenvalues of $\Theta^*$ are  bounded by $1/\rho$ and $\rho$.
%
So the parameter space $\mathcal{U}(s)$
restricts our precision matrix $\Theta^*$ to well-conditioned matrices.

In the following, we will discuss the estimation of edge weights under the Gaussian graphical model, followed by the verification of sparsity and dependence conditions, and finally the presentation of theoretical results for the Gaussian graphical model.



\paragraph{Estimation}   
First, in the setup of Gaussian graphical model, we need an appropriate estimator of the precision matrix $\Theta^*$, based on $n$ i.i.d. observations $\bX_1, \ldots, \bX_n$ following the distribution of $\bX$. % Let $\boldsymbol{X}=(\bX_{1}, \ldots, \bX_{n})^\top$
There is already significant work in literature to achieve  inverse covariance estimation. % For example, we can estimate ${\Theta^*}$ by the graphical lasso estimator  \citep{friedman2008sparse} or the method of constrained $\ell_1$-minimization for inverse matrix estimation (CLIME) \citep{cai2011constrained}.
We can % obtain estimator $\hat\Theta$   by the graphical lasso estimator  \citep{friedman2008sparse} or the method of constrained $\ell_1$-minimization for inverse matrix estimation (CLIME) \citep{cai2011constrained}.
% Then in order to achieve asymptotic normality of each entry of $\hat \Theta$, we 
consider the unbiased estimator $\hat\Theta^{\mathrm{d}}=\{\widehat{\Theta}_{uv}^{\mathrm{d}}\}_{(u,v) \in E}$ in (S.34) of \cite{lu2017adaptive},
\begin{equation}
\widehat{\Theta}_{uv}^{\mathrm{d}}:=\widehat{\Theta}_{uv}-\frac{\widehat{\Theta}_{\cdot u}^{\top}\big(\widehat{\Sigma} \widehat{\Theta}_{\cdot v}-\mathbf{e}_{v}\big)}{\widehat{\Theta}_{\cdot u}^{\top} \widehat{\Sigma}_{\cdot u}},
\end{equation}
% where $\widehat{\Sigma}=1/n \sum_{i=1}^n \bX_i\bX_i^\top$ is the sample covariance matrix, $\widehat{\Theta}_{\cdot j}, \widehat{\Sigma}_{\cdot j}$ is the $j$-th column of matrix $\widehat{\Theta}, \widehat{\Sigma}$ respectively, and $\mathbf{e}_{k} \in \RR^d$ is the $k$-th natural basis with only the $k$-th entry being 1.
% If $\hat{\Theta}$ satisfies (3.3) and (3.4) in \cite{neykov2019combinatorial}, $\hat\Theta^\mathrm{d}_{uv}$ can be decomposed into:
% \begin{equation}\label{eqn:decomp}
%  \sqrt{n} \widehat{\Theta}^\mathrm{d}_{uv}=n^{-1 / 2} \sum_{i=1}^{n}\big(\Theta^*_{\cdot j}^{* \top} \bX_i\bX_i^\top \Theta^*_{\cdot v}^{*}-\Theta^*_{uv}^{*}\big)+o_{P}(1)  
% \end{equation}
which is asymptotically normal distributed that  $\sqrt{n}\big(\widehat{\Theta}_{uv}^{\mathrm{d}}- \Theta^*_{uv}\big) \rightsquigarrow N\big(0, \Theta^*_{uu}\Theta^*_{vv}+\Theta^{*^2}_{uv}\big)$. Here $\widehat{\Theta}_{uv}$ is estimator of  $\Theta^*_{uv}$, which can come from  the graphical lasso estimator  \citep{friedman2008sparse} or the method of constrained $\ell_1$-minimization for inverse matrix estimation (CLIME) \citep{cai2011constrained}.

% Noting that 
% \[
% \text{Var}(\Theta^*_{j \cdot}^TXX^\top\Theta^T_{\cdot v})=
% \]
Recall that  $ W_{uv}^*:=  {\Theta}^*_{uv} $, 
% and let edge weight estimator $W^*_{uv}:=|\widetilde{\Theta}_{uv}|$. \yue{Here we abuse the notation of ${\Theta}_{uv}^*$ when its meaning is clear in the context.}
  we propose the following $\hat{W}_{uv}$ (i.e.,  $\widehat{\Theta}_{uv}^{\mathrm{d}}$) and  $W_{uv}$ for the Gaussian graphical model: for any edge $(u,v)\in E$,
\begin{equation}\label{eq:That:GGM}  
  \hat{W}_{uv}= \widehat{\Theta}_{uv}^{\mathrm{d}},\qquad W_{uv}=\frac{1}{n }\sum_{i=1}^n\Theta^*_{u\cdot}\bX_i\bX_i^\top\Theta^*_{\cdot v}.
  \end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We have the following theoretical guarantee. The proof of this proposition is deferred to Section \ref{sec:pflem:GGM} in the Appendix.
\begin{restatable}[]{prop}{lemGGM}\label{lem:GGM} 
For GGM with $\Theta \in {\cal U}(s)$ defined in \eqref{eqn:us}, suppose $s^2\log^4(dn)/n=o(1)$ hold, the estimator $\hat{W}$ defined in \eqref{eq:That:GGM} for the GGM satisfies 
% with probability at least $1-o(1/\log d)$ for all $j\in {\cal H}_0$, $e_j\in N_j$ with $| N_j|\leq C$, we have 
\[
\mathbb{P}\Bigl( \sup_{e\in E}\big|\hat{W}_e-W_e-W^*_e\big|/\sigma_e\leq\frac{C}{\sqrt{n\log d}},
\ 
\sup_{e\in E}\big|\sigma_e/\hat{\sigma}_e-1\big|\leq \frac{C}{\log d}\Bigr)=1-o(1),
\]
where {   $\sigma_{uv}:=\sqrt{\Theta^*_{uu}\Theta^*_{vv} + (\Theta^*_{uv})^2}$ and $\hat \sigma_{uv}:=\sqrt{\widehat{\Theta}_{uu}^{\mathrm{d}} \widehat{\Theta}_{vv}^{\mathrm{d}}  + (\widehat{\Theta}_{uv}^{\mathrm{d}} )^2 }$ for $(u,v) \in E$. }
\end{restatable}



%Moreover, it is obvious that  $\sqrt{n}W^*(\cdot)$ defined in (\ref{eq:That:GGM}) satisfies Scenario $(a)$ in (\ref{con:Tstar}). 

     \paragraph{Assumptions}
Next we check that the sparsity and dependence conditions in Assumption  \ref{ass:spadepend} also hold under the Gaussian graphical model with $\Theta \in {\cal U}(s)$. In fact, under the notation system of Gaussian graphical models, we can determine that
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{small}
\begin{align}
\begin{split}\label{eq:NHS:GGM}
S\big(\{e_{j}\}_{j \in \cH_0}\big)=
\Big\{
& (e_{j_1},e_{j_2}): j_1\neq j_2,(u,v)=e_{j_1},(u',v')=e_{j_2}, \\
& \frac{|\Theta^*_{uu'}\Theta^*_{vv'}+\Theta^*_{uv'}\Theta^*_{u'v}|}{\sqrt{\Theta^*_{uu}\Theta^*_{u'u'}\Theta^*_{vv}\Theta^*_{v'v'}}}  \geq\frac{C}{(\log d)^{2+\gamma}} \Big\}.
\end{split}
\end{align} 
\end{small}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The following proposition tells us that given the constraint in $S$, the maximum possible cardinality of $S$ can be reduce from $O(|{\cal H}_0|^2)$ to  $O(|{\cal H}_0|d^{M-2}s^2)$, where we recall that $M=\max_j|V(F_j)|$.
\begin{proposition}\label{prop:GGM}   
For Gaussian graphical models with $\Theta \in {\cal U}(s)$ where the maximum degree of the graph $G^*$  is $s$.  We have  $S=O(|{\cal H}_0|d^{M-2}s^2)$.
%,  and $\frac{\rho |{\cal H}_0|^2 }{ \log d} =O(\frac{d^{2m}}{\log d})$.
\end{proposition}
%The proof of this proposition is deferred to Section \ref{sec:pfprop:GGM} in the appendix.

 So by  Proposition
\ref{prop:GGM}, if $|{\cal H}_0|\asymp |{\cal H}_0| + |{\cal H}_1|\asymp d^M$, dependence condition in Assumption \ref{ass:spadepend} for GGM can be implied by
$$
\frac{d^{M-2}s^2}{|\widetilde{{\cal H}}_1|}=o\Big(\frac{1}{\log d}\Big) \text{ or equivalently } 
|\widetilde{{\cal H}}_1| = \omega(s^2 d^{M-2} \log d).
$$
% \[
% \frac{J^2s^2}{|{\cal H}_0||\widetilde{{\cal H}}_1|d^2}= o \bigg( \frac{1}{ \log d}  \bigg),\qquad \text{or equivalently}\qquad  |\widetilde{{\cal H}}_1|\gg \frac{s^2\log d J }{d^2|{\cal H}_0|}J
% \]
% {   When we have $|{\cal H}_0|\asymp  |{\cal H}_1|$ and $|\widetilde{{\cal H}}_1|\gg \frac{s^2 \log d}{d^2} |{\cal H}_1|$, the above can hold. Note that the maximum degree $s$ can be as least as  $O(1)$ for sparse graphs and so the dependence condition in Assumption \ref{ass:spadepend} for GGM is a {   mild} assumption. } 
% That is dependence condition can be satisfied if   $|\widetilde{{\cal H}}_1|$ to be slightly larger than  $(s^2\log d) /d^2$ proportion of $|{\cal H}_0|$ (i.e., a small proportion of null hypotheses). 
The proof is deferred to Section \ref{sec:pfprop:GGM} in the appendix.

\paragraph{Theoretical results}

We have the following corollary for the statistical guarantee of the performance of Algorithm \ref{alg:1} under the Gaussian graphical model above.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\begin{restatable}[FDR and power guarantee under GGM]{corollary}{corFDRPOWGGM}\label{cor:FDRPOW:GGM} Under the same conditions of Proposition \ref{lem:GGM}.
Suppose $\log d/\log n=O(1)$,
then under Assumption \ref{ass:spadepend} with $S$ defined in \eqref{eq:NHS:GGM}, we have
\[
\text{FDP}\leq q\frac{|{\cal H}_0|}{J}+o_{P}(1),\qquad \text{FDR}\leq q\frac{|{\cal H}_0|}{J}+o(1),
\]
 and we have uniform power control %where $|{\cal H}_0|=|{\cal H}_0|$ and $J=|{\cal H}_0|+|{\cal H}_1|$,
\begin{equation*}
\mathbb{P}\Bigl(\psi_j=1,\text{ for all }j\in \widetilde{{\cal H}}_1\Bigr) = 1 -  o(1).
\end{equation*}   

\end{restatable}
The idea to prove this is by combining Proposition \ref{lem:GGM} and Theorem \ref{thm:generalfdp}. Its proof is postponed to Section \ref{sec:cor:FDRPOW:GGM} in the appendix. 

Next we consider a high-temperature Ising model and propose the corresponding test statistic.


% if this does not cause confusion
% \paragraph{Maximum Quantile Approximation}
% Second, we approximate the null distribution of the maximum statistic 
% \begin{equation}\label{eqn:TE-GGM}
% T_{E}=\sqrt{n}\max_{(u,v) \in E}
% \Big|
% \widetilde{\Theta}_{uv}
% -
% {\Theta}_{uv}^* 
% \Big|.    
% \end{equation}
% Let $\hat c (\alpha, E)$ denote the estimator for $(1-\alpha)$-quantile of the statistic $T_{E}$ by Gaussian multiplier bootstrap in  \citep{Chernozhukov2013Gaussian}. 
% We also denote
% $ {\hat c}^{-1}(\tau, E) $
% as an estimator for $\mathbb{P}\big(T_{E} > \tau\big).$ The details on $\hat c (\alpha, E)$ can be found in Section 5 of \cite{lu2017adaptive}. 

% \begin{lemma}\label{lem:GMB-GGM}
% For Gaussian graphical models, suppose $\Theta \in \mathcal{U}(s)$ and $(\log (d n))^{7} / n+s^{2}(\log d n)^{4} / n=o(1)$. We obtain $\hat c(\alpha, E)$ from (2.4) in \cite{zhang2021startrek}. Then for any edge set $E \subseteq E$, we have
% $$
% \lim_{(n, d) \rightarrow \infty} \sup _{\boldsymbol{\Theta} \in \mathcal{U}(s)} \sup _{\alpha \in(0,1)}\Big|\mathbb{P}\Big(\max_{(u,v) \in E} \sqrt{n}
% \Big|
% \widetilde{\Theta}_{uv}
% -
% {\Theta}_{uv}^* 
% \Big|
% >\widehat{c}(\alpha, E)\Big)-\alpha\Big|=0.
% $$

% \end{lemma}


% To be specific, motivat ed by the decomposition in \eqref{eqn:decomp}, we construct the following Gaussian multiplier bootstrap statistic  \citep{Chernozhukov2013Gaussian}:
% \begin{equation}\label{eqn:bootstrap stat}
%     T_{E}^{\mathcal{B}}:=\max _{(j, k) \in E} \frac{1}{\sqrt{n \widehat{\Theta}_{uu} \widehat{\Theta}_{vv}}}\bigg|\sum_{i=1}^{n} \widehat{\Theta}_{\cdot j}^{\top}\bigl(\bX_{i} \bX_{i}^{\top} \widehat{\Theta}_{\cdot v}-\mathbf{e}_{k}\bigr) \xi_{i}\bigg|,    
% \end{equation}
% where $\xi_{i} \sim N(0,1), i \in[n]$ are independent and identically distributed.   
% Let $\hat c (\alpha, E)$ denote the $(1-\alpha)$-quantile of the statistic $T_{E}^{\mathcal{B}}$ (conditioning on the data $\bX: \bX_1, ..., \bX_n$). Formally, we define
% \begin{equation}\label{eqn:chat}
%  \hat c(\alpha, E):=\inf _{t \in \mathbb{R}}\Big\{t \biggiven \mathbb{P}\big(T_{E}^{\mathcal{B}} \leq t \biggiven \bX \big) \geq 1-\alpha\Big\}   
% \end{equation}
% as an estimator for $(1-\alpha)$-quantile of $T_E$.
% We also define the inverse function
% \begin{equation}\label{eqn:chat-1}
%  {\hat c}^{-1}(\tau, E) :=  1-\mathbb{P}\big(T_{E}^{\mathcal{B}} \leq \tau \biggiven \bX \big).
% \end{equation}




 
 

%%%% Yue Sept 16


% \paragraph{Skip-down with BHq procedure}
% For our multiple testing problem where we aim to select all subgraphs, we can consider conducting each single test by the skip-down procedure proposed by \cite{lu2017adaptive}, which was a general framework for testing monotone graph properties, such as connectivity or the maximum degree.
% The single test procedure is presented below in Algorithm \ref{alg:1}, which
% takes standardized estimator $\widetilde{\Theta}^{\d}$ as input.
% \begin{algorithm}[htbp]
%     \caption{Skip-down algorithm for testing the $j$-th subgraph \label{alg:1}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,   significance level $\alpha$. }
%     Initialize {$t=0,\, E_{0,j}= \big\{(j_1, j_2)\in V_j \times V_j: j_1\neq j_2\big\}$, and $E_{0,j}^c=\emptyset.$} 
%     % \{(j_1, j_2)\in V_j \times V_j:j_1\neq j_2\}$}. %\{(j_1, j_2): \text{all edges between the $j$-th set of nodes $V_j$}\}$.
   
%     \Repeat{${G_j \subseteq  (V_j,E_{t,j}^{c}) } \mbox{ or } \mathcal{R}=\varnothing$}
%     { 
%     $t \leftarrow t+1$\;
    
%     The rejected edge set $\mathcal{R} \leftarrow\Bigl\{e \in E_{t-1,j}:\,\sqrt{n}\big| \widetilde{{\Theta}}_{e}\big|>\chat(\alpha, E_{t-1,j})\Bigr\}$\;
    
%     $E_{t,j} \leftarrow E_{t-1,j} \setminus \mathcal{R}$ and  $E_{t,j}^c \leftarrow E_{t-1,j}^c \cup \mathcal{R}$\;
%     }
%   	\Output{$\psi_{j, \alpha}=1$ if $G_j  \subseteq (V_j,E_{t,j}^{c}) $, $\psi_{j, \alpha}=0$ otherwise.}%$G^* \subseteq E_{t,j}^{c}$, $\psi_{j, \alpha}=0$ otherwise.}
% \end{algorithm}

% \begin{figure}[h!]
% 	\begin{center}
% 		\begin{tabular}{cc}
% 		&{(A) the complete graph \   (B) $t=0$ \quad\quad\quad\quad  (C) $t=1$ \quad\quad\quad\quad  (D) $t=2$ \quad\quad\quad\quad\quad\quad\ \ \ \ \ \ \ \ \ \ \ \   }\\
% 		&\includegraphics[width=0.99\textwidth,angle=0]{./figure/alg1} \\
% 			[-10pt]
% 		\end{tabular}
% 	\end{center}
% 	\caption{Illustration of Algorithm \ref{alg:1}. Suppose we have a graph with six nodes and we aim to select all triangles. (A) is the complete graph with six nodes and thus 15 possible triangles. As an example, we only focus on  the green triangle in (B). When $t=0$, $E_{0,j}$ is the set of the three green edges. In (C), when $t=1$, we reject one edge (the red one). In (D), when $t=2$, we reject another red edge. Then in the next iteration, we reject nothing. So the algorithm ends here and we only reject two edges. So in this example, we can not reject the null hypothesis in \eqref{eqn:hypo}.}
% 	\label{fig:alg1}
% \end{figure}

% To conduct the subgraph selection (i.e., multiple testing), we need to determine an appropriate threshold $\alpha$ in Algorithm \ref{alg:1} in order to control FDR at a pre-determined level $q$ (e.g., 0.05), and we reject $H_{0j}$ if $\psi_{j, \alpha}=1$. 
% We consider Benjamini and Hochberg (BHq) procedure \citep{benjamini1995controlling}, so $\alpha$ in Algorithm \ref{alg:1} is chosen as 
% \begin{equation}\label{eqn:alphahat}
% \widehat{\alpha}=\sup \Bigl\{\alpha \in(0,1): \frac{\alpha J}{\max \Bigl\{1, \sum_{j \in [J]} \psi_{j, \alpha}\Bigr\}} \leq q\Bigr\},
% \end{equation}where $J$ is the total number of hypotheses. Normally, if the subgraph involves $m$ nodes, then $J=\binom{d}{m}$.
   
   
   

\subsection{Subgraph selection on   Ising models }\label{sec:example:Ising}
In the Ising model introduced in Example \ref{ex:ising}, $\bX=(X_{1}, X_{2}, \ldots X_{d})^{\top} \in \{1,-1\}^{d}$ follows distribution in \eqref{eqn:Ising}.
We have $w^*_e > 0$ if and only if $e \in E^*$, and $w^*_e=0$ for $e \notin E^*$. 
Suppose a lower bound $\theta$ for $w^*_e, e\in E^*$ is known, we consider the following parameter space
\begin{small}
\begin{equation}\label{model:Ising:para}
\mathcal{W}:=\Big\{w^*: 
    \min_{e\in E^*}w^*_e\geq \theta,\|w^*\|_\infty \leq \Theta, s \tanh(\Theta)<\rho,s\geq 2\rho/(1-\rho)\Big\}, 
\end{equation}% \min_{e\in E^*}w^*_e\geq \theta,\|w^*\|_\infty \leq \Theta, \rho\tanh (\Theta)\leq \tanh(\theta)\leq C/\log d,s \tanh(\Theta)<\rho^2/(1+\rho^2)\Big\}, 
\end{small}
where $\rho \in (0,1)$ is a constant.

%2022825
% \begin{equation}\label{model:Ising:para}
% \mathcal{W}:=\left\{{\wb}: \begin{array}{ll}
%     \min_{e\in E^*}w_e\geq \theta,\|\wb\|_\infty \leq M,  \frac{s\tanh^2(M)}{1-(s-1)\tanh(M)}<\tanh(\theta)\leq C/\log d,&  \\
%      1-(\tanh (M)+\frac{s\tanh^2(M)}{1-(s-1)\tanh(M)})^2>C,\text{maxdegree(G)}<s. & 
% \end{array}\right\}    
% \end{equation}
% \begin{equation}\label{model:Ising:para}
% \mathcal{W}:=\left\{{\wb}: \begin{array}{ll}
%     \|\wb\|_\infty \leq \Theta/\theta,  \frac{s\tanh^2(\Theta)}{1-(s-1)\tanh(\Theta)}<\tanh(\theta)\leq C/\log d,&  \\
%      1-(\tanh (\Theta)+\frac{s\tanh^2(\Theta)}{1-(s-1)\tanh(\Theta)})^2>C,\text{maxdegree(G)}<s. & 
% \end{array}\right\}    
% \end{equation}
% for some positive constant $C$, $\Theta$.
 

% {  These are regular conditions to ensure non-vanishing variance}

% {  discuss different $\tanh(\theta), \tanh(\Theta)\leq C/\log d$}

% {\bf condition for persistent homology under Ising models}
% \begin{equation}\label{model:phIsing:para}
% \mathcal{W}:=\left\{{\wb}: \begin{array}{ll}
%   \|\wb\|_\infty \leq \Theta/\theta,   \tanh(\Theta)+\frac{s\tanh^2(\Theta)}{1-(s-1)\tanh(\Theta)}\leq C/\log d,&  \\
%      \text{maxdegree(G)}<s. & 
% \end{array}\right\}    
% \end{equation}
This consider a high-temperature Ising model, note that \cite{neykov2019property} has proved that the testing of cycles is statistically possible if and only if $\theta =\Omega(\sqrt{\log d/n})$. In practice, the testing  under high-temperature Ising model is harder than that under low-temperature model since the former usually suffers for extremely weak and sparse signals. This suggests the superiority of our framework that it is even able to solve hard statistical testing problems with FDR controls. Below, we start by how to construct the test statistic.
%{  high tempreture,  is  a statistical possible but very hard regime.}

% $$ T_{uv}:= \hat \EE X_u X_v = \frac{1}{n} \sum_{i=1}^{n} X_{ui} X_{vi}$$

% $$U_{uv}:= \EE X_u X_v,\  u, v \in [d].$$ 

In the following, we first introduce how to estimate edge weight under the Ising model. Then we verify the sparsity and dependence conditions and finally present the theoretical results for the Ising model.


\paragraph{Estimation} Consider $n$ i.i.d. samples $\bX_1,\ldots, \bX_n \in {1,-1}^{d}$ from the Ising model, where $\bX_i=(X_{i1}, X_{i2}, \ldots X_{id})^{\top}$. To estimate the edge weight, we use $\hat{W}$ and $W$ for the Ising model as follows: for any $(u,v) \in E$,
\begin{equation}\label{eq:That:Ising}
   \hat{W}_{uv}=\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv}  - \tanh(\theta),\ W_{uv}=\frac{1}{n}\sum_{i=1}^{n} X_{iu} X_{iv}-\mathbb{E}[X_uX_v].
\end{equation}
{We also have
$\hat \sigma_{uv} = \sqrt{1-(\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv})^2}$
and $\sigma_{uv} = \sqrt{1-(\EE X_{iu} X_{iv})^2}$. }
% \begin{remark}
% In Ising model, it is slightly different from Gaussian graphical model that here we always have $\Var(\hat{W}_{uv}) = 1-(\frac{1}{n}\sum_{i=1}^{n} X_{iu} X_{iv})^2 = 1-o(1)$. So there is no need to assume $\Var(\hat{W}_{uv}) = 1$ here.
% \end{remark}
% and
% \begin{equation*}
% W^*_{uv}=\frac{\mathbb{E}[X_uX_v]-\tanh(\theta)}{\sqrt{1-(\mathbb{E}[X_uX_v])^2}}.
% \end{equation*}
We have the following theoretical guarantee for asymptotic normality of $\hat W_{uv}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Denote $m=\max\{|\mathbb{E}[X_uX_v]|^2:(u,v)\in E(F_j),j\in \widetilde{{\cal  H}}_1\}$, $m_0=\max \{|\mathbb{E}[X_uX_v]|^2:(u,v)\in N_j,j\in {\cal H}_0\}$ 
\begin{restatable}[]{prop}{lemIsing}\label{lem:Ising}  Under Ising models \eqref{eqn:Ising} with parameter space \eqref{model:Ising:para}, the estimator $\hat{W}$ defined in \eqref{eq:That:Ising} for the Ising model satisfies 
\[
\mathbb{P}\Bigl( \sup_{e\in E}\big|\hat{W}_e-W_e-W^*_e\big|/\sigma_e\leq\frac{C}{\sqrt{n\log d}},\ 
\sup_{e\in E}\big|\sigma_e/\hat{\sigma}_e-1\big|\leq \frac{C}{\log d}\Bigr)=1-o(1).
\]

 \end{restatable}
 The proof of this proposition can be found in Section \ref{sec:pflem:Ising} in the Appendix.

% {  
% \[
%  \sqrt{n}\frac{\widehat{\Theta}_{uv}^{\mathrm{d}}-\mu}{\sqrt{\widehat{\Theta}_{uv}^{\mathrm{d}}\widehat{\Theta}_{vv}^{\mathrm{d}}}},\qquad \frac{\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv}  - \tanh(\theta)-\mu}{\sqrt{1-(\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv})^2}}
% \]

% \[
% \mathbb{P}\Bigl( \sup_{e\in E}\big|\hat{W}_e-W_e-W^*_e\big|/\sigma_e>\frac{C}{\sqrt{n\log d}}\Bigr)=o(1),\qquad \mathbb{P}(\sup_{e\in E}\big|\hat{\sigma}_e-\sigma_e\big|>C/\log d)
% \]

% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Assumptions}
For Ising models, following the notations from Section \ref{sec:example:Ising},  we have
\begin{align}
\begin{split}\label{eq:NHS:Ising}
   S(\{e_j\}_{j\in {\cal H}_0})=\Big\{
   & (e_{j_1},e_{j_2}): j_1\neq j_2,(u,v)=e_{j_1},(u',v')=e_{j_2}, \\
   & \Cov(X_uX_v,X_{u'}X_{v'}) \geq \frac{C}{(\log d)^{2+\gamma}} \Big\}.
\end{split}
\end{align}
Assumption \ref{ass:spadepend} is difficult to verify under the general graph structure of Ising models. However, Proposition \ref{prop:Ising} states that a similar conclusion to Proposition \ref{prop:GGM} holds for a graph with a tree structure. 
% This suggests that Assumption \ref{ass:spadepend} may be feasible for the general graph structure of Ising models. 
The proof of Proposition \ref{prop:Ising} is presented in Appendix Section \ref{sec:pfprop:Ising}.

\begin{proposition}\label{prop:Ising}
For Ising models, assume that the graph with $d$ nodes consists of $d/s$ trees and each tree has $s$ nodes. We have  $S=O(|{\cal H}_0|d^{M-1}s)$.
%,  and $\frac{\rho |{\cal H}_0|^2 }{ \log d} =O(\frac{d^{2m}}{\log d})$.
\end{proposition}
  %%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%
      %%%%%%%%%%%%%%%%%%%%%%%%%%
Thus, if $|{\cal H}_0|\asymp |{\cal H}_0| + |{\cal H}_1|$, dependence condition in Assumption \ref{ass:spadepend} for the Ising model can be implied by
$$
\frac{d^{M-1}s}{|\widetilde{{\cal H}}_1|}=o\Big(\frac{1}{\log d}\Big) \text{ or equivalently } 
|\widetilde{{\cal H}}_1| = \omega(s d^{M-1} \log d).
$$



%{  Similar to GGM, when XXX, this will hold.}

\paragraph{Theoretical results}

Similar to the analysis of Gaussian graphical model in Section \ref{sec:example:GGM}, under Ising models, we also  have the following corollary for the theoretical guarantee of the performance of Algorithm \ref{alg:1}.

\begin{restatable}[FDR and power guarantee under Ising models]{corollary}{corFDRPOWIsing}\label{cor:FDRPOW:Ising} 
Assume the same conditions as in Lemma \ref{lem:Ising}, and $\log d/\log n=O(1)$.
Under Assumption \ref{ass:spadepend} with $S,\widetilde{{\cal H}}_1$ defined in \eqref{eq:NHS:Ising}, we have
\[
\text{FDP}\leq q\frac{|{\cal H}_0|}{J}+o_{P}(1),\qquad \text{FDR}\leq q\frac{|{\cal H}_0|}{J}+o(1),
\]
where  $J=|{\cal H}_0|+|{\cal H}_1|$, and we have uniform power control
\begin{equation*}
\mathbb{P}\Bigl(\psi_j=1,\text{ for all }j\in \widetilde{{\cal H}}_1\Bigr) = 1- o(1).
\end{equation*}   
\end{restatable}
The proof  is deferred to Section \ref{sec:pfcor:FDRPOW:Ising} in the Appendix.



% Next we illustrate condition \eqref{eqn:depend} using a simple example. Assuming our graph is Figure {   ????} with $d$ nodes and some triangles, and we aim to select all triangles. As in the figure, $\big(\{k_1,\ell_1\}, \{k_2,\ell_2\} \big)$ is counted in $S$. Since we have $d$ nodes, we have at most $d$ possible choice of $k_1$ and $d$ possible choice of $\ell_1$. 
% Also, edge $(k_1,\ell_1)$ can be in other sets $N_{j}, j \neq j_1$ in addition to $N_{j_1}$. For selecting triangles, $(k_1,\ell_1)$ can be in at most $d$ different $N_{j}$ since we only have freedom of choosing the third nodes. 
% For edge $(k_2,\ell_2)$, we observe $k_2$ should be the same node as $k_1$ and $\ell_2$ should be one node of triangle $\Delta_1$ so that $\big(\{k_1,\ell_1\}, \{k_2,\ell_2\} \big)$ satisfies the condition in \eqref{eqn:S} and is counted in $S$. Thus, $S$ is at most of the order of $d^4$. On the other hand,  if $|{\cal H}_0|$ and $J$ are  of the order of $d^3$,   Condition \eqref{eqn:depend} requires $d =o(\frac{|\widetilde{{\cal H}}_1|}{ \log d})$.



% In general, assume that the maximum degree of graph is at most $s$, and the subgraph of interest $F$ has $m=|V(F)|$ nodes.  Following the similar argument as above,  we have $S$ is at most of the order of $d^2s^2(\binom{d}{m-2})^2$ or simply $d^{2m-2}s^2$,  and $\frac{\rho |{\cal H}_0|^2 }{ \log d} $ is at most of the order of $\frac{d^{2m}}{\log d}$.

% Condition \eqref{eqn:depend} requires $d =o(\frac{|\widetilde{{\cal H}}_1|}{ \log d})$.

% Also $|\cH_0|$ is the number of true null hypotheses. If the graph is too connected (where $|\cH_0|$ is typically small) then the multiple testing problem is harder.
% For example, if $J$ and $|\cH_0|$ are at the order of $d^m$, then \eqref{eqn:depend} holds when 
% $|S| = o \Big( \frac{\rho |{\cal H}_0|^2 }{ \log d}  \Big). $




% {  
% \begin{assumption}\label{ass:signal}
% We assume the following condition hold:
% \begin{equation}\label{eqn:scaling}
% \frac{ J\log d }{|\widetilde{{\cal H}}_1|} \cdot \bigg( \frac{(\log d)^{19 / 6}}{n^{1 / 6}} + \frac{(\log d)^{11 / 6}J^{1/3}}{n^{1 / 6} |\widetilde{{\cal H}}_1|^{1 / 3}} + s\frac{(\log d)^{3} }{\sqrt{n}} + \frac{J}{d^{   m+1} |\widetilde{{\cal H}}_1|} +  \frac{1}{|{\cal H}_0|} \bigg)=o(1),    
% \end{equation} 
% \begin{equation}\label{eqn:depend}
% \frac{ J\log d }{|\widetilde{{\cal H}}_1|} \cdot  \frac{1}{|{\cal H}_0|^2} |S| = o(1).    
% \end{equation}
% \end{assumption}
  


% Recall that $\cH_0=\bigl\{1\leq j \leq J \biggiven  F_j \not\subseteq G^* \bigr\}$ is the set of true null hypotheses, and   $\cH_1=\bigl\{1\leq j \leq J \biggiven  F_j \subseteq G^* \bigr\}$ is the set of true alternative hypotheses.
% And \begin{equation}\label{eqn:tilde H_1}
% \tilde{\mathcal{H}}_{1}:=\Bigl\{j \in \mathcal{H}_{1}: \forall (u,v) \in N_{j}^c \text{ with } u \neq v,\bigl|\Theta^*_{uv}^*\bigr|> C_0 \sqrt{\log d / n}\Bigr\} \subseteq \cH_1
% \end{equation}
% is a subset of $\cH_1$, containing true alternative hypotheses where the all edges of these subgraphs have signal strength  exceeding $\sqrt{\log d/n}$.

% $S$ is a measure of dependence defined as 
% \begin{equation}\label{eqn:S}  
% S= \bigcup_{j_{1}, j_{2} \in \mathcal{H}_{0}, j_{1} \neq j_{2}} \Big\{\big( \{k_1,\ell_1\} , \{k_2,\ell_2\} \big): (k_1,\ell_1) \in N_{j_{1}}, (k_2,\ell_2) \in N_{j_{2}},  \Theta^*_{k_1k_2}   \Theta^*_{\ell_1\ell_2}+\Theta^*_{k_1\ell_2} \Theta^*_{k_2\ell_1} \neq 0 \Big\},     
% \end{equation}
% with
% $
% N_{j}=\Bigl\{e\in V(F_j) \times V(F_j): \Theta^*_{e}^*=0\Bigr\}$ and  $N_{j}^{c}=\Bigl\{(u,v)\in V(F_j) \times V(F_j): u \neq v, \bigl|\Theta^*_{uv}^*\bigr|>0\bigr\}$.




%  Condition \eqref{eqn:scaling} is the scaling condition required for validity of maximum quantile estimation by Gaussian bootstrap procedure.
% See detailed discussions in \cite{zhang2021startrek}. Note that $\tilde \cH_1$ is defined in \eqref{eqn:tilde H_1}.  Here we do not need signal strength for all true subgraphs. For example, let $J:=\binom{d}{m}$ and $|\cH_0|$ both be at the order of $O(d^m)$,
% we require
% \begin{equation}   
% |\widetilde{{\cal H}}_1| = W^* \bigg(  
%  \frac{d^m (\log d)^{25 / 6}}{n^{1 / 6}} + {\frac{d^{m} (\log d)^{17 / 8}}{n^{1 / 8} }} + 
%  s\frac{d^m (\log d)^{4} }{\sqrt{n}} + 
%   d^{(m-1)/2}\sqrt{\log d} + \log d \bigg) 
% \end{equation} 
% for  \eqref{eqn:scaling}  to hold.

% $$   \rho $$ 


% Condition \eqref{eqn:depend} is the dependence condition.
% We can think of set $S$ as a measure of dependence between null hypothesis in $\cH_0$. As shown in \eqref{eqn:S}, if $\big( \{k_1,\ell_1\} , \{k_2,\ell_2\} \big) \in S$, it intuitively means there is some ``path'' linking edges $(k_1,\ell_1)$ and $(k_2,\ell_2)$ together, which means they are somehow ``dependent'' or ``correlated''.
% Intuitively, when $|S|$ is larger, i.e., dependence is higher, the multiple testing problem is harder.  {     We also need a trade-off between $|{\cal H}_0|$ and $|\widetilde{{\cal H}}_1|$. Because the ideal case is both $|{\cal H}_0|$ and $|\widetilde{{\cal H}}_1|$ are all large for \eqref{eqn:depend} to hold. However, there is a natural constraint that  $|{\cal H}_0|+|\widetilde{{\cal H}}_1| \leq J$. 
  
% }
% % Also $|\cH_0|$ is the number of true null hypotheses. If the graph is too connected (where $|\cH_0|$ is typically small) then the multiple testing problem is harder.
% For example, if $J$ and $|\cH_0|$ are at the order of $d^m$, then \eqref{eqn:depend} holds when $$
% |S| = o \Big( \frac{d^m}{\log d} |\widetilde{{\cal H}}_1| \Big). $$
% }


% (i)
% $$   \frac{ J\log d }{|\cB|} \cdot \Big( \frac{(\log d)^{19 / 6}}{n^{1 / 6}} + \frac{(\log d)^{11 / 6}J^{1/3}}{n^{1 / 6} |\cB|^{1 / 3}} + s\frac{(\log d)^{3} }{\sqrt{n}} + \frac{J}{d^{\mu+1}|\cB|} \Big)=o(1).$$

% (ii)

% $$   \frac{ J\log d }{|\cB||{\cal H}_0|} + \frac{ J\log d }{|\cB||{\cal H}_0|^2} |S| =o(1).
% $$ 
% where $$\tilde{\mathcal{H}}_{1}:=\Bigl\{j \in \mathcal{H}_{1}: \forall (j_1,j_2) \in N_{j}^c,\bigl|\Theta^*_{j_1j_2}\bigr|> C_0 \sqrt{\log d / n}\Bigr\},$$
% and
% $$S= \bigcup_{j_{1}, j_{2} \in \mathcal{H}_{0}, j_{1} \neq j_{2}} \Big\{(k_1,l_1) \in N_{j_{1}}, (k_2,l_2) \in N_{j_{2}}: \Theta^*_{k_1k_2} \Theta^*_{l_1l_2}+\Theta^*_{k_1l_2} \Theta^*_{k_2l_1} \neq 0 \Big\},$$
% with
% \[
% N_{j}=\Bigl\{(j_1, j_2)\in V_j \times V_j: \Theta^*_{j_1j_2}=0\Bigr\}, \qquad N_{j}^{c}=\Bigl\{(j_1, j_2)\in V_j \times V_j: \Bigl|\Theta^*_{j_1j_2}\Bigr|>0\Bigr\}.
% \]






% Based on Algorithm \ref{alg:2}, we have the following theorem controlling FDP and FDR. Proof can be found in Appendix \ref{sec:pf:FDR}. 
% \begin{restatable}[FDP/FDR control]{theorem}{thmFDR}\label{thm:FDR} Suppose  Assumptions \ref{ass:regularcon} and \ref{ass:spadepend} are satisfied.
% We have that Algorithm \ref{alg:2}  satisfies: as $(n, d) \rightarrow \infty$,     
% $$   
% \mathrm{FDP} \leq q \frac{J_{0}}{J}+o_{P}(1) \quad \text { and } \quad \lim _{(n, d) \rightarrow \infty} \mathrm{FDR} \leq q \frac{J_{0}}{J}, 
% $$
% for  Gaussian graphical models and Ising models.
% \end{restatable}

% \begin{theorem}[FDP/FDR control]\label{thm:FDR}
% Suppose  Assumptions \ref{ass:scaling} and \ref{ass:depend} are satisfied.
% We have that Algorithm \ref{alg:2}  satisfies: as $(n, d) \rightarrow \infty$,     
% $$   
% \mathrm{FDP} \leq q \frac{J_{0}}{J}+o_{P}(1) \quad \text { and } \quad \lim _{(n, d) \rightarrow \infty} \mathrm{FDR} \leq q \frac{J_{0}}{J}, 
% $$
% for  Gaussian graphical models and Ising models.
% \end{theorem}

% \begin{remark}
% Because of  the equivalence of Algorithms \ref{alg:2} and \ref{alg:3} in Proposition \ref{prop:2-3} with $\tilde \cV = \cV$, we have both algorithms can control FDP and FDR.
% \end{remark}


% {   check notation below}


% The following theorem shows that our procedure is also powerful.
% \begin{theorem}[Power Analysis]\label{thm:power}
% {   Suppose conditions in
% Lemma \ref{lem:GMB-GGM} are satisfied for Gaussian graphical models, or  conditions in
% Lemma  \ref{lem:GMB-Ising} are satisfied for Ising models.}
% We have under the alternative hypothesis $H_{1j}$ in \eqref{eqn:hypo}, assuming \yue{ $\min_{e \in E(F_j), j \in [J]}| \Theta^*_{e}| >  C_{0} \sqrt{\frac{\log d}{n}}$ }
% for some sufficiently large constant $C_0$, we have
% \begin{equation*} 
%   
% \mathbb{P}\bigl(\psi_{j, \alpha}=1 \text{ for all $j \in \cH_1$} \bigr) \rightarrow 1 \ \text{ as } n,d \to \infty.    
% \end{equation*}


% \end{theorem}



 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
 \section{Inferential Analysis for Graphical Persistent Homology}
\label{sec:ph}


In the previous sections, we propose efficient methods for detecting  subgraphs that may  be linearly dependent in some algebraic space (i.e., some selected subgraphs could imply the significance of some other subgraphs).  An interesting question is: can  we  select  `holes' that are  linearly independent in topological algebra of a graph. Moreover, can  we  select  ``holes'' across multiple scales to characterize their persistence?  Important applications are, for example, depicting the persistence of various elementary topological properties  of a network;  determining whether two graphical objects are topologically equivalent (see e.g., \cite{aktas2019persistence}). 
 %{  select linearly independent cycles?}

 
 To achieve the goal, there are three main issues to address:
 \begin{enumerate}

     \item Formulate the concepts of topological properties and their persistence on a weighted graph;
     \item Develop  efficient algorithms to detect elementary  topological properties of various structures across continuous scales;
     \item Provide statistical guarantee of the persistence of the  topological properties determined by the efficient algorithms.
  %
 \end{enumerate}
 
 %which has many important applications e.g., determining whether given two graphical objects are topologically equivalent. 
 
 
 Persistent homology endows us with  a mathematical framework to analyze the topologically invariant features. It is to study the invariance of subgraph features through their lifespans of the persistent barcode. The statistical methods for persistent homology on point clouds and distributions are developed by many statisticians (e.g., \cite{fasy2013statistical}). However, the statistical method for persistent homology on graphs is deficient. 


 In Section \ref{sec:ph:pre}, we first introduce the preliminaries of persistent homology. Then we translate the problems of our interests into hypotheses testing problem and propose reasonable statistical measures in Section \ref{sec:ph:measure}. In Section \ref{sec:ph:alg}, we propose efficient solutions to estimate the persistence of subgraph features (also known as persistent barcodes). Last, we provide statistical analysis for our novel method in Section \ref{sec:ph:stat_ana}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preliminaries of Persistent Homology}\label{sec:ph:pre}
Persistent homology is a powerful tool to analyze the subgraph features on graphs. A complete introduction to persistent homology and the algebraic topology foundations can be found in \cite{horak2009persistent,aktas2019persistence}. The basic aim of persistent homology is to measure the lifetime (the birth and death) of certain topological properties (e.g.,  
 loops, 
tetrahedron etc.,) along the evolution of the graph. As edges are added to the graph in order, subgraph features may appear or disappear. The sequence of growing (or diminishing) graphs constructed in the process is known as filtration , as illustrated  in Figure \ref{fig:filtration} (a). The lifespan of each homological feature with respect to the filtration levels can be represented as an interval with left and right end points being the birth and the death 
time, respectively. All intervals yielded by this filtration process can be visualized as the persistent barcodes (See  Figure \ref{fig:filtration} (b)), which distinguish long-lasting subgraph features  from short-lived ones. % (``topology noise'')
% \begin{figure}[h!]
% 	\begin{center}
% \includegraphics[width=0.8\textwidth,angle=0]{./figure/filtration} 
% 	\end{center}
% 	\caption{Edges added between $[\mu^{(8)},\mu^{(9)}]$, $[\mu^{(6)},\mu^{(7)}]$,  $[\mu^{(5)},\mu^{(6)}]$, $[\mu^{(4)},\mu^{(5)}]$, $[\mu^{(2)},\mu^{(3)}]$ and $[\mu^{(1)},\mu^{(2)}]$ are the critical edges of $Z_1(E^*)$ between filtration interval $[\mu^{(2)},\mu^{(9)}]$, while that added in  $[\mu^{(5)},\mu^{(6)}]$ is the only critical edge of $Z_2(E^*)$ between filtration interval $[\mu^{(1)},\mu^{(8)}]$. }
% 	\label{fig:filtration}
% \end{figure}


\begin{figure}[h!]
	\begin{center}
\includegraphics[width=0.3\textwidth,angle=0]{./figure/Yue4} 
	\end{center}
\vspace{-10pt}
	\caption{
 Illustration of filtration of graphs. As level $\mu$ decreases, more edges are added to the graph and high-dimensional simplices appear.}
	\label{fig:filtration}
\end{figure}

On the other hand, a graph only has nodes and edges which can be considered as $0$-simplices and $1$-simplices respectively.
Standard persistent homology can only study connected subgraphs and loops structure of such graphs. To capture more of the topological information, it is prevalent to construct higher-order simplicial complexes from lower-order simplices in a graph and thus some graphical features corresponding to higher-order topological properties can also be encoded and studied in a filtration. One popular choice is to induce clique complex \cite{carstens2013persistent,aktas2019persistence}, which is more meaningful in interaction networks. This is done by filling various cliques into  simplices which  have higher-order faces. Below,   to statistically depict the evolution of the subgraph features captured by the generalized persistent homology, we formalize the problem in the graphical model. 

It is natural to construct the filtration process in terms of the signal strength of edges. 
For a given weighted graph $G^*=(V, E^*)$, we define the graph at filtration level $\mu$ as $G^*(\mu)=(V, E^*(\mu))$, where the edge set at level $\mu$ is  $E^*(\mu)=\big\{e\in E^*: |W^*_e| \geq \mu\big\}$ and we recall that $W^*:=\{W^*_e\}_e$ is the weight matrix  of the network. % reflecting the ground truth relationship {  (e.g., $w$ can be $|\Theta^\star|$ in the gaussian graphical model or $\omega^{\star}$ in the ising model)}.  
Therefore, for a sequence of levels $\mu^{(1)}<\mu^{(2)}<\cdots<\mu^{(t)}$, we can obtain a filtration of edge sets $E^*(\mu^{(1)}) \supseteq E^*(\mu^{(2)}) \supseteq \ldots \supseteq E^*(\mu^{(t)})$ and a corresponding filtration of graphs
\begin{equation}\label{eq:ph:filtration}
  G^*(\mu^{(1)}) \supseteq G^*(\mu^{(2)}) \supseteq \ldots \supseteq G^*(\mu^{(t)}).  
\end{equation}

%If we associate to this ordering the clique complex $K$ of each graph $G^*(\mu)$, $1\leq a\leq t$, which is a collection of complete subgraphs, we obtain a filtered complex
%\begin{equation}\label{eq:ph1}
% K^{0} \subseteq K^{1} \subseteq \cdots \subseteq K^{t}.   
%\end{equation}
%{  here}
For each filtered graph, or in general an arbitrary graph  $G_0:=(V,E_0)$, we can associate it with a clique complex $K$, which is a collection of complete subgraphs of $G_0$.  Given this filtered complex, we are interested in its corresponding persistent homology groups across different filtration levels which capture the evolution of the underlying cycles (i.e., subgraph features), and are  introduced later. To that end, for each clique complex $K$ and 
order $k$, one needs to introduce  the associated chain groups $\mathrm{C}_k(E_0)$, the boundary operators $\partial_k:  \mathrm{C}_k(E_0) \rightarrow \mathrm{C}_{k-1}(E_0)$, the cycle
groups $ Z_k(E_0)=\text{ker}~\partial_k$, the boundary groups $B_k(E_0)=\text{im}~\partial_{k+1}$ and the $k$-homology groups of~$G_0$ 

\begin{equation}\label{eq:ph:hgroup}
\mathrm{H}_k(E_0)=\frac{\text{ker}~\partial_{k}}
{\text{im}~\partial_{k+1}} = \frac{ Z_k(E_0)}{B_k(E_0)},  %\mathrm{H}_{k}^{\mu}
\end{equation}
where
\[
\mbox{ker}~\partial_k=
\big\{z\in \mathrm{C}_k(E_0):\partial_k(z)=\emptyset\big\},\quad \mbox{im}~\partial_k=
\big\{b\in \mathrm{C}_{k-1}(E_0):\exists z\in \mathrm{C}_k(E_0),\mbox{ s.t. } b=\partial_k(z)\big\}.
\]
% For instance, 
To understand these definitions, $\mathrm{C}_k(E_0)$ is a vector space  
defined on the set of $k$-dimensional oriented
simplices in $K$. The elements $c$ of the vector space $\mathrm{C}_k(E_0)$ are also denoted as $k$-chains, $c = \sum_i c_i\sigma_i$, with $\{\sigma_i\}_i$ the set of oriented $k$-simplices in $K$ and $\{c_i\in \mathbb{R}\}_i$ the particular coefficients that specify the vector $c$. The boundary operators $\partial_k$ are linear maps defined by their actions on the oriented simplices $\{\sigma_i\}_i$ in $ K$. More precisely, the image of $\partial_k$ acting on an oriented $k$-simplex $\sigma:=[v_0,v_1,\ldots,v_k]$ consists of a linear combination of its oriented $k$ facets in $\mathrm{C}_{k-1}(E_0)$:
\[
\partial_{k} (\sigma)=\sum_{i}(-1)^{i}[v_{0}, v_{1}, \ldots, v_{i-1},v_i, \ldots, v_{k}].
\]
The definitions of the vector subspaces cycle group $ Z_k(E_0)=\text{ker}~ \partial_k$ and boundary groups $B_k(E_0)=\text{im}~ \partial_{k+1}$ follow elementarily from those of the chain group and the boundary operator.    On the other hand,
it can be verified from the definition of boundary operator that $\partial_{k} \circ \partial_{k+1}=0$ and therefore $B_k(E_0)\subseteq  Z_k(E_0)\subseteq \mathrm{C}_k(E_0)$. This yields a corresponding quotient group $\mathrm{H}_k\big(E_0\big)$ for graph $G_0$ defined in (\ref{eq:ph:hgroup}). 

Basically, for each  order $k$ and each graph $G_0$, $ Z_k(E_0)$ is the set of cycles which are $k$-chains with empty boundary and  $B_k(E_0)$ is the set of $k$-chains which are boundaries of $k+1$-chains in $\mathrm{C}_k(E_0)$. 
For $k\geq 1$, the cycles of the $k$-th cycle group $ Z_k(E^*)$ in $G^*$ are  all the  $k$-order subgraph features ever appear along  the filtration while $Z_0(E^*)$ is just the group of nodes. Therefore, $\mathrm{H}_k\big(E_0\big)$ is the group of $k$-cycles where cycles that are boundaries of $k+1$-chains are removed.    Intuitively,  $\mathrm{H}_0(E_0)$ is the group of connected components;  $\mathrm{H}_1(E_0)$ is the group of loops; $\mathrm{H}_2(E_0)$ is the group of voids; and similarly for larger $k\geq 3$, $\mathrm{H}_k\big(E_0\big)$ is the group of higher-order holes. In other words, at filtration level $\mu$, the homology group $\mathrm{H}_k\big(E^*(\mu)\big)$ captures the $k$-th order subgraph features. 
%{  without including triangle's. Amining to discover more features like cliques. We consider the cycles in the  cycle group directly to characterize the homology. Note that the from XX, If we are able to estimate the cycles in , we  still be able to recover XX.}

Note that a newly formed clique will be immediately filled into a simplex as the filtration level $\mu$ decreases, since we are considering clique complex. And so cliques, like triangles, tetrahedrons which are also important features of graphs, would not be included in these homology groups.  Aiming to discover more  higher-order subgraph features, we consider  the cycle group $ Z_k(E_0)$ which complement the cycles of cliques features that vanished due to the filling to characterize the homology. One should also note that if we are able to characterize the subgraphs in $G^*$ that formed the cycles of $ Z_k(E^*)$, then by filling the cliques, we can recover the holes in $\mathrm{H}_k(E^*)$ in some sense. 
%The cycles that induce for $ Z_k(E^*)$  can be given by the {\it  Bass-Serre theory} \cite{hatcher2002algebraic}. 

 In this paper, we focus on detecting higher-order cycles  ($k\geq 1$) and leave the study of the cycles of $\mathrm{H}_0$~(i.e., connected components) as future work. {   Let $D \subseteq [d]$ be the set of dimensions of cycle group we are interested in testing and denote 
 \[
 Z(\mu)=\bigoplus_{k\in D}Z_k\big(E^*(\mu)\big),
 \]
 which is  the  cycle group of interest at filtration level $\mu$.} Based on the introduced persistent homology tools, a naive approach to characterize the evolution of the cycle group $Z(\mu)$, is to conduct the following hypotheses testing through the filtration line $\mu\geq \mu_0$ for some self-determined starting point $\mu_0$
{  

\[
H_0(\mu): Z(\mu)=Z(\mu-\epsilon)\text{ for small }\epsilon>0,
\]
v.s.
\[
H_1(\mu):Z(\mu)\subsetneq Z(\mu-\epsilon)\text{ for all } \epsilon>0.
\]
}
% \[
% H^{(k)}_0(\mu): Z_k(E^*(\mu))=Z_k(E^*(\mu-\epsilon))\text{ for small }\epsilon>0,
% \]
% v.s.
% \[
% H^{(k)}_1(\mu):Z_k(E^*(\mu))\subsetneq Z_k(E^*(\mu-\epsilon))\text{ for all } \epsilon>0.
% \]
Intuitively, the goal is to detect newly generated higher-order cycles as the filtration level moves from $\mu$ to $\mu - \epsilon$. The ultimate objective is to select all cycles as the filtration level moves from a large value to a small value. However,  the order of new cycles generated may vary across different observations  while the underlying weights determine a static true order. This imposes difficulties in testing and forming statistical measure (e.g., definitions of FDP). To that end, we  need to give an index/order for the cycles. In the next section, we present the details and rigorous definitions. %In the next section, we present the details and rigorous definitions.
%Intuitively we aim to detect new generated cycles when the filtration level move from $\mu$ to $\mu-\epsilon$. And our final goal is to select all cycles when filtration level  $\mu$ moving from large to small. However,  the order of new cycles generated is probably different for different observations while the underlying weights determine a static order. So to do cycle selection and quantify FDP, we need to give an index/order for all the cycles of interest. %In the next section, we present the details and rigorous definitions.



% {  


% We draw the barcodes as follow, define $\bar{\cal F}(\mu)$

% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
\subsection{Persistent Barcodes and Statistical Measure}\label{sec:ph:measure}
A more stringent goal we are after is to  select which linearly independent cycles that induce dimension increment and depict their persistence. As such, we can draw the persistent barcodes which summarize the topological properties and their persistence of  the graph. To formalize this  statistically, it is necessary to classify linearly dependent cycles associated to each incremented dimension. 

In fact, the cycles can be grouped according to   critical edges (will be defined formally later) that induce dimension increment on the cycle group during the filtration process (\ref{eq:ph:filtration}). Suppose, during the filtration process,  edges $e_1,e_2,\ldots,  e_{|E|}$  are added into the graph following orders on weights:
\begin{align*}
        \text{Scenario $(a)$: }&\qquad|W^*_{e_1}|\geq |W^*_{e_2}|\geq\cdots\geq |W^*_{e_{|E|}}|; \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \text{Scenario $(b)$: }&\qquad W^*_{e_1}\geq W^*_{e_2}\geq\cdots\geq W^*_{e_{|E|}}. 
\end{align*} 
{   
% Next we define critical edges, which is crucial in statistical formulation and   the testing procedure. 
We abuse use notation of $Z(\cdot)$ for the cycle group on graph $(V,\cdot)$, whenever it is clear from the context. We calculate increased dimension $\ell_i=\text{dim}(Z(\{e_1, \ldots, e_{i}\})-\text{dim}(Z(\{e_1, \ldots, e_{i-1}\}))$ when the edge $e_i$ is added in the graph, for $i=1, \ldots, |E|$. Then we define critical egde $\bar{e}_{j}= e_i$ for $j$ satisfying $\sum_{u=1}^{i-1}\ell_u < j \le \sum_{u=1}^{i}\ell_u$. Note that if $\ell_i = 0$ for some $i$, then there is no critical edge defined here. Intuitively, $\ell_i$ can be understood as the multiplicity of $e_i$, i.e., how many linearly independent cycles are generated due to the addition of $e_i$.
And  each critical edge induces exact one incremented dimension of the cycle group. Figure \ref{fig:filtration} provides a illustration for critical edges.
We denote all the critical edges as  $\{\bar{e}_j: j=1,2,\ldots \bar{J}\}$ where $\bar J = \text{dim}(Z(E))$. In fact the following proposition gives a explicit formula for the dimension of the cycle group of a complete graph.

}

% {    We say an edge $e_j$ is a critical edge of the $k$-th cycle group if $Z_k(\{e_i\}_{i=1}^j)$ has extra dimensions than $Z_k(\{e_i\}_{i=1}^{j-1})$. Without loss of generality, we discuss the case where each critical edge induce an extra dimension in $k$-th cycle group. Otherwise, we can signature multiple $k$-th  cycle group to a critical edge. We also denote all the critical edges of the $k$-th cycle group by $\{\bar{e}_k(j):j=1,2,\ldots \bar{J}_k\}$ and corresponding cycle group by $\{Z_k^j:j=1,2,\ldots \bar{J}_k\}$. Here  $\bar{J}_k$ is the dimension of the  $k$-cycle group of a $d$-clique, i.e., the maximum possible number of $   k$-th linearly independent cycles in a graph. Note that,  there could be multiple critical edges with equal weights (e.g.,  edges in $ E\setminus E^*$ could also be critical edges as long as {   its addition} induce dimension increment). We can assign their orders of adding to the graph in arbitrary rules. 
% }


% {  
% {
%     Calculate increased dimension $\ell_i=\text{dim}(Z(\{e_1, \ldots, e_{i}\})-\text{dim}(Z(\{e_1, \ldots, e_{i-1}\}))$\;
  
%     {For $i=1, \ldots, E$, if $ \sum_{u=1}^{i-1}\ell_u \le j \le \sum_{u=1}^{i}\ell_u$ },{ then 
%     $\bar{e}_{j}= e_i$
%     }
%     }
% }

%For example, see  Figure \ref{fig:filtration}, edges that appear between $[\mu^{(1)},\mu^{(2)}]$, $[\mu^{(3)},\mu^{(4)}]$,  $[\mu^{(4)},\mu^{(5)}]$, $[\mu^{(5)},\mu^{(6)}]$, $[\mu^{(7)},\mu^{(8)}]$ and $[\mu^{(8)},\mu^{(9)}]$ are the critical edges of $Z_1(E^*)$ between filtration interval $[\mu^{(1)},\mu^{(8)}]$, while that appears in  $[\mu^{(4)},\mu^{(5)}]$ is the only critical edge of $Z_2(E^*)$ between filtration interval $[\mu^{(1)},\mu^{(8)}]$. 
\begin{restatable}[Dimension of the cycle group of a $d$-clique]{proposition}{propdim}\label{prop:dim} The dimension of the $k$-cycle group of a $d$-clique is $(d-k)(d-k-1)/2$.%, where $k=1,2$.
\end{restatable}
{   By the above property, it can be seen that the dimension of the $k$-cycle group is $O(d^2)$. Recall that in the ordinary subgraph selection, the number of testing triangles in a graph requires $\tbinom{d}{3}$ hypotheses. This suggests that persistent homology is a more reasonable way to select hole-structure graph features as it rules out redundancy.} 
  
%{  mention it is used in the algorithm    not exponential, polynomial, reduce redundant} 
%{  the critical edges may be duplicated. add lemma showing the number of Jbar k is (d-k)(d-k-1)/2}

% With the notion of critical edges and associated cycle group, we can now select linearly independent cycles of each $k$-cycle group by conducting the following multiple hypotheses testing   through the whole filtration line $\mu\geq \mu_0$, for $j=1,2,\ldots,\bar{J}_k$, $k\in D$
% \begin{equation}\label{eq:ph:mt:space}
%    
%     H^{(k)}_{0j}(\mu):Z_k^j\not\subseteq Z_k(E^*(\mu)),\qquad\text{v.s.}\qquad H^{(k)}_{1j}(\mu):Z_k^j\subseteq Z_k(E^*(\mu)).
% \end{equation}


Since persistent barcodes are drawn continuously, we would like to evaluate the false discoveries  over a filtration interval $(\mu_0,\mu_1)$  (e.g., $\mu_0=-\infty$ or lower bound for the weights and $\mu_1=+\infty$ or $\mu_1=\max_{j,k}|W^*_{\bar{e}_k(j)}|$, etc., the choice of $\mu_1$ will be discussed more later in Section \ref{sec:ph:stat_ana}). Moreover, when testing  the persistent barcodes (i.e., the presence of cycles) at a given filtration level $\mu$, we would like to consider the   false discoveries cycles of multiple orders instead of one single order. {   Recall that we are interested in selecting $   
 Z(\mu)=\bigoplus_{k\in D}Z_k\big(E^*(\mu)\big)$ 
   at filtration level $\mu$.} Suppose we obtain a set of linearly independent cycles and the corresponding cycle group is $\hat{Z}(\mu)$, we propose the following uniform False Discovery Proportion (uFDP) and the uniform False Discovery Rate (uFDR) on a filtration interval $(\mu_0,\mu_1)$:   
 \begin{equation}\label{eq:ph:FDPFDR}
 \begin{aligned}
& \mathrm{uFDP}:=\sup_{\mu \in (\mu_0,\mu_1)} \frac{\text{dim}\big(\hat{Z}(\mu))-\text{dim}\big(Z(\mu)\cap \hat{Z}(\mu)\big)}{\max \Bigl\{1, \text{dim}\big(\hat{Z}(\mu)\big)\Bigr\}}, \\ 
& \mathrm{uFDR}:=\mathbb{E}[\mathrm{uFDP}].
 \end{aligned}
\end{equation}
Here at each filtration level $\mu$, $\text{dim}\big(\hat{Z}(\mu))$ counts the number of selected cycles acting as linearly independent bases and $\text{dim}\big(Z(\mu)\cap \hat{Z}(\mu)\big)$ counts that of correctly selected one. So the nominator counts the number of falsely selected cycles and $\mathrm{uFDP}$ quantifies the maximum false discovery proportion of selected linearly independent cycles on filtration level $(\mu_0,\mu_1)$. The meaning of $\text{uFDP}\leq q+o_{P}(1)$ (uFDR$\leq q+o(1)$) is as follows. On the filtration interval $\mu \in (\mu_0,\mu_1)$, the proportion of the false discoveries of linearly-independent cycles  is uniformly and asymptotically less than $q$ in probability (in expectation). Compared to classical definitions of tail probability of FDP and FDR in  \eqref{eq:classicalFDPFDR}, the control on the tail probability of uFDP and uFDR  are much stricter since it requires uniform control on finite filtration points and novel  in the sense that it discuss false discoveries on vector space. 

% \begin{remark} 

% {   move to appendix}

% It is equivalent to define uFDP in the classical way: \[
% \mathrm{uFDP}=\sup_{\mu \in (\mu_0,\mu_1)} \frac{\sum_{(j,k)\in \bar{{\cal H}}_0(\mu)}\psi^{(k)}_{j,\mu}}{\max \Bigl\{1, \sum_{k\in D}\sum_{j=1}^{\bar{J}_k} \psi^{(k)}_{j,\mu}\Bigr\}},
% \]
% where $\psi^{(k)}_{j,\mu}=0$ if and only if   $H_{0j}^{(k)}(\mu)$ is accepted, and  $\bar{{\cal H}}_0(\mu):=\{(j,k): H^{(k)}_{0j}(\mu)\text{ is true, }j\in [\bar{J}_k],k\in D\}$ is the set of all true null hypotheses at filtration level $\mu$. However, since we do not have prior knowledge of the underlying graph structure $G^*$ (or otherwise we directly obtain the cycle group), we are unable to determine which edges are critical edges and which cycles in each $Z_k^{j-1}$. Consequently,  this induces a difficulty to construct decision rule for each hypothesis. With a selected cycle, the implicit nature of the problem restricts our ability to match it with its corresponding hypotheses pair and so empirical values of  $\{\psi^{(k)}_{j,\mu}\}_{j,k}$ is unobservable. Nevertheless, in theory, we are still be able to evaluate the  $\{\psi^{(k)}_{j,\mu}\}_{j,k}$ based on selected cycles and $\{Z_k^{j-1}\}$ such that we can study theoretical behaviour of uFDP and uFDR.  As we keep focus in the main parts to our methodology and algorithms and (\ref{eq:ph:FDPFDR}) is simpler to illustrate the ideas, we leave the details about the novel design of the decision rules to the Section \ref{sec:pfthm:ph:generalfdppow} in the appendix.
 
% \end{remark}


%In the following section, we discuss a possible way to tackle the multiple testing on critical edges with controls on tail probability of uFDP and uFDR.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Efficient Algorithms to Obtain  Persistent Barcode with Statistical Control}\label{sec:ph:alg}

In this section, we first introduce a novel method  that can select linearly independent cycles at any given filtration level $\mu\geq \mu_0$, which is formalized as Algorithm \ref{alg:ph:basis}. Then  utilizing the discrete structure of the graph, we introduce Algorithm \ref{alg:ph:barcode} that  identifies the complete persistent barcodes by  running Algorithm \ref{alg:ph:basis} at only finite many filtration levels.

Suppose
%, naturally, for each $k$-th ($k\in D$) cycle group we are interested in, we have the hypothetical set of all possible topological features  that could act as cycles (e.g., for  $Z_1$, it would be all loops and the linear combination of loops). Also, 
at each filtration level $\mu$, we have a generalized estimator $p_e(\mu)$ for the $p$-value of each edge $e\in E$.   For example, for the two scenarios discussed in Section \ref{sec:estpvalue},  we generalize to use the following ways to estimate the $p_e(\mu)$ with an estimated edge weight~$\hat{W}_e$ :
\begin{align}
\begin{split}\label{eq:ph:Wpvalue}
        \text{$(a)$: }&\ \hat{W}_e(\mu)= |\hat{W}_e|-\mu,\  p_e(\mu)=2-2\Phi({\sqrt{n}  \hat{W}_e(\mu)}/\hat{\sigma}_e); \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \text{$(b)$: }&\  \hat{W}_e(\mu)=\hat{W}_e-\mu,\  p_e(\mu)=1-\Phi\big(\sqrt{n}  \hat{W}_e(\mu)/\hat{\sigma}_e\big). 
\end{split}
\end{align} 

% \begin{remark}
% Similar as previous sections, we assume $\Var(\hat W_e) = 1$ and  thus use \eqref{eq:ph:Wpvalue}. If $\Var(\hat W_e) \neq 1$, we incorporate the variance and define $\hat{W}_e(\mu)= |\hat{W}_e|-\mu/\sqrt{\Var(\hat W_e)} $ for Scenario (a) and define Scenario (b) similarly.
% \end{remark}


% \begin{remark}For the non-normalized graph, we can define
% \begin{align*}
%         \text{Scenario $(a)$: } p_e(\mu)=2\big(1-\Phi(\frac{\sqrt{n}  \hat{W}_e(\mu)}{\text{sd}(\hat{W}_e)})\big); \qquad
%     \text{Scenario $(b)$: } p_e(\mu)=1-\Phi\big(\frac{\sqrt{n}  \hat{W}_e(\mu)}{\text{sd}(\hat{W}_e)})\big). 
% \end{align*} 
% \end{remark}
We let the $p$-value of each feature $F$ be the maximum over the $p$-value of its edge:
\begin{equation}\label{eq:phgraphpvalue}
\alpha(F)=\max_{e\in E(F)}p_e(\mu).    
\end{equation}
  And we have a prior edge set $E'$, which   can be the full edge set $E$ or  a smaller edge set to reduce computation, {   e.g., $\{e\in E,p_e(\mu)\leq q\}$. }
  More advantages will be discussed later with Algorithm \ref{alg:ph:barcode}.



The main idea of Algorithm \ref{alg:ph:basis} is as follow. {   We %initialize the set of selected cycles $\bar{{\cal F}}$  as $\emptyset$. 
 start from an graph with an empty edge set $\widetilde{E}$, we keep adding edges to $\widetilde{E}$. Each time we choose the edge with the smallest $p$-value from $E'$ (denoted at $e^*$), and if $e^*$ increases the dimension  on the cycle group\footnote{Intuitively,  it is calculating the number of induced linearly independent bases due to the addition of edge $e^*$. One only needs to check the subgraph connecting $e^*$ and so can be efficiently implemented in computer.}, we add $e^*$ to $\widetilde{E}$. We also assign $p$-values to the bases induced by adding $e^*$ to $\widetilde{E}$. This ensures that the new bases are linearly independent with previous bases.
 % any cycle in the $Z_k(\{e^*\}\cup \widetilde{E})\setminus Z_k( \widetilde{E})$ into the set $\bar{{\cal F}}$. This ensures that the added cycle corresponds the incremented dimension and is linearly independent with former added cycles. According to (\ref{eq:phgraphpvalue}), we can simply assign the $p$-value of each added cycle by $p_{e^*}(\mu)$ since the latest added edge has the largest $p$-value. 
 The process ends when   all the remaining edges in $E'$ have $p$-value larger than $q$. Then we obtain the estimated graph and the corresponding cycle group by applying the BHq procedure on all the assigned $p$-values of the empirical critical edges. Note that the set of linearly independent cycles acting as the bases set of the estimated cycle group is not unique. It can be chosen arbitrary as long as it matched the cycle group.
}
% Intuitively, in Algorithm \ref{alg:ph:basis}, we  initialize the selected basis set $\bar{{\cal F}} = \emptyset$. At each iteration, we add the edge with the smallest $p$-value among all other edges in $E'$


% we choose specific feature from $\widetilde{{\cal F}}$, and add it to $\bar{{\cal F}}$. The chosen feature should be independent of all selected features in $\bar{{\cal F}}$, and has smallest $p$-value in $\widetilde{{\cal F}}$.  

% {\darkblue We initialize the edge set $E$ as the set all edges, the selected edge set $E'$ as a null set, and the selected cycles set $\bar\cF$ as a null set.
% Starting from a null graph, we add edges with small $p$-values into $E'$  until $p$-values large than the threshold $0.05$, and delete these edges from $E$. To be specific, at each iteration $j$, we choose the edge $e^*$ in $E$ with  the smallest $p$-value {  (i.e., the currently most significant edge)}. This is is equivalent to (\ref{eq:phgraphpvalue}) since the latest added edge has the largest $p$-value. And if a linearly independent basis (denoted as $F_j$) appearing when we add the edge $e^*$ to $E'$, we define the $p$-value for the basis $F_j$ as the $p$-value of $e^*$.
% When no edges can be added (i.e., all the rest edges in $E$ having $p$-values larger than $0.05$), the selected cycles set $\bar{{\cal F}}$  consists of the most  significant  cycles  at the filtration level $\mu$. Applying the BHq procedure on it, with the number of total hypotheses being $\bar{J}:=\sum_{k\in D}\bar{J}_k$, we obtain the final selected cycles. 
% }

% {\darkblue similar to Algorithm \ref{alg:1},  we first can construct a filtered graph with the $p$-value of each edge less than $q$ to  eliminate impossible hypothetical cycles and reduce computation. The remaining possible hypothetical cycles in the filtered graph is $\widetilde{{\cal F}}$.
% Then in order to select as many as possible linearly-independent cycles from $\widetilde{{\cal F}}$, at each iteration,  we select the basis that is linearly-independent with currently added cycles in $\bar{{\cal F}}$ and has the smallest $p$-value among $\widetilde{{\cal F}}$, and add it to  the set $\bar{{\cal F}}$. We also update the possible hypothetical cycles $\widetilde{{\cal F}}$ by removing those could be reconstructed by the added cycles in $\bar{{\cal F}}$. 
%  Adding cycles in this way avoids selecting  redundant  cycles that are linearly dependent. It allows us to test less linearly dependent cycles and discover more linear independent cycles and thus improve statistical efficiency. }
%  When  no cycles can be added, the collected cycles set $\bar{{\cal F}}$  consists of the most  significant  cycles  at filtration level $\mu$. Applying the BHq procedure on it, with the number of total hypotheses being $\bar{J}:=\sum_{k\in D}\bar{J}_k$, we obtain the final selected cycles. 
 
% 2022/10/25
% \begin{algorithm}[H]
%     \caption{{    {\bf P}ersistence {\bf O}f Critical {\bf E}dges {\bf T}esting (POET)}%{  {\bf S}electing {\bf NO}n-visible ${\bf W}^*_{\bar{e}}$ (SNOW) at level $\mu$}
%     }  \label{alg:ph:basis}
%     \SetKwRepeat{Do}{do}{while}
%     Input: Filtration level $\mu$, FDR level $q$, hypothetical feature sets $\{{\cal F}_k\}_{k\in D}$.  
    
%     Initialize $E=\{(u,v)\in E:u\neq v\}$, $\bar{{\cal F}}=\emptyset$ and $j=1$\; 
    
%     Determine filtered hypothetical cycles set  $\widetilde{{\cal F}}=\{F\in \cup_k {\cal F}_k:E(F)\subseteq \{e\in E:p_e(\mu)\leq q\}\}$\;

%     Calculate  the $p$-value of potential cycles by $\alpha(F)=\max_{e\in E(F)}p_e(\mu)$ for all $F\in \widetilde{{\cal F}}$.
 
%     \While{$\widetilde{{\cal F}}\neq \emptyset$}{
%     Denote  $\bar{\cal F}=\argmin_{F\in \widetilde{{\cal F}}}\alpha(F)$ and  $\alpha^*=\min_{F\in \widetilde{{\cal F}}}\alpha(F)$\;
%     \For{${\cal F}\in \{{\cal F}_k:{\cal F}_k\cap \bar{\cal F}\neq \emptyset,k \in D\}$}{
%     Let $\bar{F}$ be any one element of $\bar{\cal F}\cap {\cal F}$ with $\alpha_j:=\alpha^*$ be its $p$-value\;
%      Update  $\bar{{\cal F}}=\bar{{\cal F}}\cup \bar{F}$, $\widetilde{{\cal F}}=\widetilde{{\cal F}}\setminus \text{span}(\bar{{\cal F}})$, $j=j+1$\; 
%     }
%     }
%      Set $\alpha_{(0)}=0$ and let $j_{\max}=\max \Bigl\{0 \leq j \leq |\bar{{\cal F}}|: \alpha_j \leq q j /  \bar{J}\Bigr\}$\; 
    
%     Output: selected cycles $\{\bar{{\cal F}}(j):1\leq j\leq j_{\max}\}$.
% \end{algorithm}

% 2022/10/26 
% \begin{algorithm}[H]
%     \caption{{    {\bf P}ersistence {\bf O}f Critical {\bf E}dges {\bf T}esting (POET)}%{  {\bf S}electing {\bf NO}n-visible ${\bf W}^*_{\bar{e}}$ (SNOW) at level $\mu$}
%     }  \label{alg:ph:basis}
%     \SetKwRepeat{Do}{do}{while}
%     Input: Filtration level $\mu$, FDR level $q$, prior edge set $E'$.  
    
%     Initialize  $\widetilde{E}=\emptyset$, $\bar\cF = \emptyset$ and $j=0$\; 

%     \While{$\{e\in E':p_e(\mu) \leq q\}\neq \emptyset$ }{
%     Denote  $e^* = \argmin_{e\in E'}p_e(\mu)$\;
%     \For{$k\in D$}{
%     \If{ $Z_k( \widetilde{E})\subsetneq Z_k(\{e^*\}\cup \widetilde{E})$}{
%      Select any cycle $F_j\in Z_k(\{e^*\}\cup \widetilde{E})\setminus Z_k( \widetilde{E})$
%     and assign its $p$-value $\alpha_j = p_{e^*}(\mu)$;
    
%     Updated selected $\bar\cF = \bar\cF \cup \{F_j\}$,
%     $j = j + 1$;
    
%     }
%     }
    
    
%     $\widetilde{E} = \widetilde{E} \cup \{e^*\}$, 
%     $E' = E' \setminus \{e^*\}$;
% }
%     % \vspace{10pt}
%     % \For{${\cal F}\in \{{\cal F}_k:{\cal F}_k\cap \bar{\cal F}\neq \emptyset,k \in D\}$}{
%     % Let $\bar{F}$ be any one element of $\bar{\cal F}\cap {\cal F}$ with $\alpha_j:=\alpha^*$ be its $p$-value\;
%     %  Update  $\bar{{\cal F}}=\bar{{\cal F}}\cup \bar{F}$, $\widetilde{{\cal F}}=\widetilde{{\cal F}}\setminus \text{span}(\bar{{\cal F}})$, $j=j+1$\; 
%     % }
%     %
%     Set $\alpha_{(0)}=0$ and let $j_{\max}=\max \Bigl\{0 \leq j \leq |\bar{{\cal F}}|: \alpha_j \leq q j /  \bar{J}\Bigr\}$\; 
    
%     Output: group spanned selected cycles $\text{span}(\{F_j \in \bar{{\cal F}}: 1\leq j\leq j_{\max}\})$.
% \end{algorithm}
 
 
 \begin{algorithm}%[H]
    \caption{{ {\bf P}ersistent {\bf C}ritical {\bf E}dges {\bf T}esting (PCET) }% {\bf P}ersistence {\bf O}f Critical {\bf E}dges {\bf T}esting (POET)}%{  {\bf S}electing {\bf NO}n-visible ${\bf W}^*_{\bar{e}}$ (SNOW) at level $\mu$}
    }  \label{alg:ph:basis}
    \SetKwRepeat{Do}{do}{while}
    Input: Filtration level $\mu$, FDR level $q$, prior edge set $E'$.  
    
    Initialize  $\widetilde{E}=\emptyset$ and $j=0$\; 

    \While{$\{e\in E':p_e(\mu) \leq q\}\neq \emptyset$ }{
    Denote  $e^* = \argmin_{e\in E'}p_e(\mu)$\;
    Calculate increased dimension $\ell=\text{dim}(Z(\{e^*\}\cup \widetilde{E}))-\text{dim}(Z(\widetilde{E}))$\;
  
    \If{ $\ell \geq 1$}{
     Assign $p$-values to the extra $\ell$ bases $\alpha_i=p_{e^*}(\mu)$, for all $i=j+1,\ldots,j+\ell$\;
    $j=j+\ell$\;
    }
    
    
    
    $    \widetilde{E} = \widetilde{E} \cup \{e^*\}, E' = E' \setminus \{e^*\}$;
}

    Set $\alpha_{(0)}=0$ and let $j_{\max}=\max \Bigl\{0 \leq i \leq j: \alpha_i \leq q i /  \bar{J}\Bigr\}$\; 
    
    Output: selected cycle group $Z(\{e\in E':p_e(\mu)\leq \alpha_{j_{\max}}\})$.
\end{algorithm}
 
%{  the estimated critical edge is not the underlying critical edges  and so is global testing} 
% {  
% \begin{remark}\label{rem:decision}
%  Note that the selected cycles on an estimated graph may not be consistent with the underlying basis system of the true graph. To address this issue, we accept $\bar{H}^{(k)}_{0j}(\mu)$ (with $\psi^{(k)}_{j,\mu}=0$) if one basis that contain critical edge $\bar{e}_k(j)$ and is consist of edges having weights larger than that of $\bar{e}_k(j)$  is in the span of the selected cycles and reject (with $\psi^{(k)}_{j,\mu}=1$) otherwise. It can be seem that although we are unable to observe the empirical decision  of each hypothesis pair, in theory, we have a decision assigned to each hypothesis pair. Therefore, we are still be able to  analyze the theoretical behaviour of FDP  after cycles selection at each filtration level.
% \end{remark}
% }
 Further, to obtain the complete persistent barcodes (i.e., obtain the evolution of cycle group through the whole filtration line $\mu \in[\mu_0,+\infty)$), intuitively, one only needs to determine the filtration levels where the selected cycle group will change and then determine the corresponding cycle group between each two change points. Motivated by this, we  propose  Algorithm \ref{alg:ph:barcode}, which initially uses Algorithm \ref{alg:ph:basis} to select linearly independent cycles at $\mu=\mu_0$ and dynamically generate the next filtration level and the updated set of selected cycles. 
 
 
\begin{algorithm}[H]
\caption{{\bf P}ersistence {\bf O}f Critical {\bf E}dges {\bf M}apping (POEM)}\label{alg:ph:barcode}
    \SetKwRepeat{Do}{do}{while}
    
    Input: Estimated edge weights $\{\widehat{W}_e\}_{e \in E}$, FDR level $q$, Start point $\mu_0$.%, hypothetical feature sets $\{{\cal F}_k\}_{k\in D}$. 
       
    Initialize  $t=0$, $E^{(0)}=E$\; 
 
     Obtain cycle group at level $\mu_0$: $\hat{Z}^{(0)}:=\text{PCET}(\mu_0,q,E^{(0)})$ \;
    
\While{    $\hat{Z}^{(t)}\neq \emptyset$}{



Update filtered edge set $    E^{(t)}:=\text{edges of the cycles that span }\hat{Z}^{(t)}$\;
Determine the next change level  $\mu^{(t+1)}:=\min_{e\in E^{(t)}}L_e(\text{dim}(\hat{Z}^{(t)})q/\bar{J})$\;   

Obtain next cycle group $\hat{Z}^{(t+1)}:=\text{PCET}(\{\mu^{(t+1)},q,\{e\in E^{(t)}:L_e(\frac{\text{dim}(\hat{Z}^{(t)})q}{\bar{J}})>\mu^{(t+1)}\})$\;

$t=t+1$\;

    }
 
 Output: Estimated evolution of the cycles group $\hat{Z}(\mu):=\hat{Z}^{(t)}$ if  $\mu^{(s-1)}<\mu\leq\mu^{(s)}$ for $s\in [t]$  and $\hat{ Z}(\mu_0):=\hat{ Z}^{(0)}$, $\hat{ Z}(\mu):=\emptyset$ if $\mu>\mu^{(t)}$.
\end{algorithm}
 However, this is not a straightforward task because of the inhomogeneous  distributions of the edges and the various combinatorial structure of the cycles. To overcome this, we first introduce confidence lower bounds for the edges to determine the next filtration level.  Suppose at iteration $t$, we have the selected cycle group $\hat{Z}^{(t)}$. Based on it, we can obtain the set of edges that spanned the  selected cycles group at filtration level $\mu^{(t)}$, denoted by $E^{(t)}$. To search for the next filtration level such that Algorithm \ref{alg:ph:basis} yields a different set of selected cycles, it is to search for the confidence lower bound of edges in $E^{(t)}$. This is because if one edge in $E^{(t)}$ is not selected, it will imply that one cycle acting as a basis of the selected cycle group will not be selected in the  BHq procedure  (i.e., the $p$-value of this basis is larger than $   q \, \dim(\hat Z^{(t)})/\bar{J}$). To achieve this, suppose we have a lower bound function $L_e(q)$ for each edge $e\in E$ at confidence level $q$. 
 In general, for the two scenarios discussed in Section \ref{sec:estpvalue}, we can let
\begin{align*}
    \text{Scenario $(a)$: } L_e(q)=|\hat{W}_e|- \frac{1}{\sqrt{n}}\Phi^{-1}(1-\frac{q}{2})\hat{\sigma}_e;\qquad 
    \text{Scenario $(b)$: } L_e(q)=\hat{W}_e- \frac{1}{\sqrt{n}}\Phi^{-1}(1-q)\hat{\sigma}_e. 
\end{align*} 
Inverting (\ref{eq:phgraphpvalue}) to confidence lower bound,  we can determine the next filtration level by
 \[  
 \mu^{(t+1)}:=\min_{e\in E^{(t)}}L_e(q \, \dim(\hat Z ^{(t)})/\bar{J}).
 \]
 Then to obtain the changed  cycles group $\hat{Z}^{(t)}$, we run Algorithm \ref{alg:ph:basis} at filtration level $\mu^{(t+1)}$ with prior edge sets excluding edges that have weights exactly equal to $ \mu^{(t+1)}$. Or otherwise, the nature of BHq procedure would still select the same  set of cycles. 
% \begin{figure}[h!]
% 	\begin{center}
% \includegraphics[width=0.8\textwidth,angle=0]{./figure/dynamic} 
% 	\end{center}
% 	\caption{Each number in (outside of) bracket is the lower bound   for weight (estimated weight) of each edge. At iteration $t$, the minimum lower bound for a basis is $0.4$ instead of $0.3$. Then running Algorithm \ref{alg:ph:basis} at graph filtered by level $\mu=0.4$, we get the  select cycle group after the next change point. }
% 	\label{fig:dynamic}
% \end{figure}
Repeating the process until the  estimated cycle group reduces to an empty set yields   the selected cycle group through the whole filtration line $\mu\geq \mu_0$. See Figure \ref{fig:dynamic} which illustrates part of   the dynamic process for first-order cycle group. 



\begin{figure}[htb!]
	\begin{center}
		\begin{tabular}{c}
\\
\includegraphics[width=.5\textwidth,angle=0]{./figure/Yue3}	
	\\
[-10pt]
		\end{tabular}
	\end{center}	\caption{The left figure is an illustration of Algorithm \ref{alg:ph:barcode}. At each iteration $t$, all the edges on the graph make the filtered edge set $E^{(t)}$, the weight of the red edge(s) represents the next filtration level $\mu^{(t+1)}$, the yellow cycles represent the remaining cycle(s) in the next iteration, and the orange cycle(s) represents the disappearing cycle(s) in the next iteration. The blue horizontal lines represent the life time of each cycle along the filtration of graph. The right figure illustrates the filtration of graphs when the filtration level $\mu$ increases.
 % At iteration $t = 0$, we determine the next filtration level $\mu^(1)$, which corresponds to the red edge on (A). 
} 
	\label{fig:dynamic}
\end{figure}


% Note that the orders of the $p$-values of edges  are inconsistent across different filtration levels due to the heterogeneous distribution of edges.  Therefore, the selected cycles in $\bar{{\cal F}}(\mu)$ may not be consistent across different filtration level $\mu$, this is because Algorithm \ref{alg:ph:basis} selects cycles with smallest $p$-values at each filtration level and the order of the $p$-values of cycles may change across different filtration levels. 
% { 
% Without unified cycles, we are unable to draw persistent barcodes. To address this, for $1\leq s \leq t$, we adjust the selected cycles at filtration level $\mu$ as
%  \begin{equation}\label{eq:ph:unifybase}
%     \bar{\cal F}(\mu)=\cup_{i=s}^t\{ \bar{\cal F}^{(i-1)}\setminus \text{span}(\bar{\cal F}^{(i)})\},\qquad \mu^{(s-1)}<\mu\leq\mu^{(s)},
% \end{equation}
% which unifies the basis system through the whole filtration line $\mu\geq \mu_0$.
%  }

% To determine the cycles associated by each barcode, we can adjust the set of selected linearly independent cycle $\bar{{\cal F}}(\mu)$ at filtration level $\mu$ by 
% \begin{equation}\label{eq:ph:unifybase}
%  \bar{{\cal F}}(\mu)=\cup_{i=s}^t\text{\{cycles  in $\hat{ Z}^{(i-1)}\setminus \hat{ Z}^{(i)}$\}},\qquad \mu^{(s-1)}<\mu\leq\mu^{(s)},   
% \end{equation}
% which unifies the basis system through the whole filtration line $\mu\geq \mu_0$.

The computation of Algorithm \ref{alg:ph:barcode} is not heavy, which is not only because it requires  iterations no more than $\text{dim}(\hat{Z}^{(0)})$,  but also because the set of filtered edge set strictly also becomes smaller after each iteration. Therefore, the computational burden of running POET at each iteration would decrease when moving to next filtration  levels. The theoretical analysis of the controls on the tail probability of uFDP and uFDR of this algorithm are deferred to Section \ref{sec:ph:stat_ana}.
The significance of cycle group detection and our methodology have three main folds:

(i) Testing unrevealed targets: Note that the cycle group  is associated to critical edges of which we do not have prior knowledge of the positions. In comparison, the ordinary subgraph selection problem in Section \ref{sec:method} presumes the  acknowledge of the positions of the structure to detect in advance such that we can conduct testing on explicit targets; even for the hub nodes detection problem studied in \cite{zhang2021startrek}, one at least can know which node corresponds to each hypotheses pair though the structure of the star related to that node is unknown.  As such, unlike traditional multiple testing problem, we can not construct an explicit test statistic for  each true critical edge.  Moreover, our approach discovers that for cycles group estimation where the critical edges are unknown, we do not need maximum statistics to ensure multiplicity control like  hub nodes detection in \cite{zhang2021startrek}.% Instead, we define the decision rule in Remark \ref{rem:decision} such that we are still  able to analyze the uFDP and uFDR in theory without observing its empirical values and affecting our goal of cycles selection. 

(ii) Selecting linearly independent features: To the best of our knowledge, there is no existing work considering  multiple testing of linearly independent objectives or the corresponding group. One may wonder  at each filtration level whether we could conduct multiple testing directly on edges which would be much simpler. However, without prior knowledge, we can not differentiate which edges are the underlying critical edges. In fact, testing a critical edge is not testing  on single edge but on global property (i.e., a basis). One needs to consider whether an added edge would introduce new bases. An alternative way is to run Algorithm \ref{alg:1} at each level and determine linearly dependent cycles from all the selected features. This approach  would select redundant linearly dependent cycles and whether we have efficiently statistical control on FDP is unsure.

(iii) Depicting persistence of features efficiently: Compared to existing works on testing graph properties, our algorithm not only select linearly independent cycles but also characterize their persistence and is able to unify the bases system across different filtration scales through the cycle group. Even though at each filtration level cycles could have size as large as $d$, the problem across infinite filtration levels could be solved efficiently.

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Statistical guarantee of the persistent barcodes}\label{sec:ph:stat_ana}
%We propose $\sup_{\mu\in[0,\mu_1)}\text{FDR}(\mu)$ for some $\mu_1$ as the reasonable measure of the statistical efficiency of the obtained persistent barcode by Algorithms \ref{alg:ph:barcode}. 
%Therefore, this requirement is {   mild} in a statistical sense.


%For simplicity of notations, we remove the superscript $(k)$, and can wrap up  $\{H_{0j}^{(k)}(\mu):j\in[\bar{J}_k],k \in K\}$ as $\{{\cal H}_{0j}(\mu):j\in [\bar{J}]\}$ and $\{{\cal H}_{1j}^{(k)}(\mu):j\in[\bar{J}_k],k \in K\}$ as $\{{\cal H}_{1j}(\mu):j\in [\bar{J}]\}$ whenever they are clear from the context.. 

Similar to the analysis of linearly dependent subgraphs selection in Section~\ref{sec:thm}, we 
% 
% introduce signal strength condition, specifically at a filtration level $\mu\geq 0$. 
% 
% Recall that $W^*(\mu)$ defined in (\ref{eq:ph:Wpvalue}) is the adjusted weight at filtration level $\mu$. Define a set that characterizes hypotheses with strong signals
%  \begin{equation}\label{eq:ph:h1tildemuh1tildemu}
%    
% \widetilde{{\cal H}}_1(\mu)=\{(j,k):  \bar{   H}_{1j}^{(k)}(\mu)\text{ is true with }W^*_{\bar{e}_k(j)}(\mu)>\sqrt{C\log d/n}\}. 
% \end{equation}
%
% Compared to (\ref{eqn:h1tilde}) for the linearly dependent subgraphs, each alternative hypothesis here only relies on a particular edge, the critical edge instead of a specified subgraph, to have enough signal. This is motivated by (\ref{eq:ph:mt:criedge})  where the signal of the existence of the cycles hinges on their corresponding critical edges. 
%
% % we aim to characterize the dependence  in problem \eqref{eq:ph:mt:criedge}. 
 characterize the dependence between null critical edges at the filtration level $\mu$ by
% \[
%    
% \bar{S}(\mu)=\bigg|\Bigl\{\big((j_1,k_1),(j_2,k_2)\big): (j_1,k_1)\neq (j_2,k_2), \bar{e}_{k_1}(j_1) \notin E^*(\mu), \bar{e}_{k_2}(j_2) \notin E^*(\mu), |\text{Cov}(\xi_1(\bar{e}_{k_1}(j_1)),\xi_1(\bar{e}_{k_2}(j_2)))|  \geq \frac{C}{(\log d)^{2+\gamma}} \Bigr\}\bigg|.
% \]
\begin{equation}
\begin{aligned}
\bar{S}(\mu)=\Big|\Bigl\{
& (j_1,j_2): j_1 \neq j_2, \bar{e}_{j_1}\notin E^*(\mu), \bar{e}_{j_2}\notin E^*(\mu), \\
& \big|\text{Cov}\big( \xi_1(\bar{e}_{j_1}),\xi_1(\bar{e}_{j_2}) \big) \big|  \geq \frac{C}{(\log d)^{2+\gamma}} \Bigr\}\Big|.
\end{aligned}    
\end{equation}

%\fbox{remark to the diff to the previous S: the critical edge is unique but the subgraph edges are not.}
% \[
% \bar{S}(\mu)=\bigg|\Bigl\{\big(j_1\neq j_2, |\text{Cov}(\xi_1(\bar{e}_{k_1}(j_1)),\xi_1(\bar{e}_{k_2}(j_2)))|  \geq \frac{C}{(\log d)^{2+\gamma}} \Bigr\}\bigg|,
% \]
% where
% \begin{equation}\label{eqn:H0}
%   
% \bar{{\cal H}}_0(\mu)=\{(j,k):  \bar{ H}_{0j}^{(k)}(\mu)\text{ is true}\}. 
% \end{equation}
Intuitively, we characterize the ``dependence'' between the pair of critical edges $(\bar{e}_{j_1}, \bar{e}_{j_2})$, which implies the dependence {   between two bases of the cycle group since each critical edge corresponds to one new basis. Compared to the previous definition in \eqref{eq:S}, here we do not need to take minimum over all choices of null edges and only need to consider critical edges. The reason is in \eqref{eq:S} and Section \ref{sec:thm}, making type I error for one subgraph implies we must have wrongly selected one edge in this subgraph (could be any edge). While here in homology part, making type I error  implies that we  wrongly selected a  null critical edge.
} 
These provide a perspective of the role of critical edges playing in the sparsity and dependence structure of the problem. Suppose the following assumptions developed on critical edges are satisfied for some $\mu_1\geq 0$, 
we can characterize the asymptotic behaviour of $\text{uFDP}$ and $\text{uFDR}$ of the persistent barcodes given by Algorithm \ref{alg:ph:barcode}.


%Recall that $\xi(\cdot)$ is a random function with identical distribution of $\xi_i(\cdot)$ introduced in (\ref{eq:That:condition}). 


% \[
% \bar{S}(\mu)=\big|\{(j_1,j_2)\in  \bar{{\cal H}}_0(\mu)\times \bar{{\cal H}}_0(\mu): j_1\neq j_2,(u,v)=e^*_{j_1},(u',v')=e^*_{j_2},|\Theta^*_{uu'}\Theta^*_{vv'}+\Theta^*_{uv'}\Theta^*_{u'v}|  \geq C\log d^{-2-\gamma} \}\big|
% \]
% for some constant $C$ and $\gamma>0$.
%$|\bar{{\cal H}}_0(\mu)|:=| \bar{{\cal H}}_0(\mu)|$; $|\widetilde{{\cal H}}_1(\mu)|:=| \widetilde{{\cal H}}_1(\mu)|$; $\bar{J}_1(\mu):=|\bar{{\cal H}}_1(\mu)|$
\begin{assumption}\label{ass:phspadepend} We assume
\[  
\sup_{\mu\in(\mu_0,\mu_1)}\bigg\{ \underbrace{ \frac{\bar{J}}{|\bar{{\cal H}}_0(\mu)|\cdot|\widetilde{{\cal H}}_1(\mu)|}}_{\text{Sparsity effect}} +\underbrace{\frac{\bar{J}\bar{S}(\mu)}{|\bar{{\cal H}}_0(\mu)|^2|\widetilde{{\cal H}}_1(\mu)|}}_{\text{Dependence effect}}\bigg\}=o(\frac{1}{\log d}),
\]
where $   |\bar{{\cal H}}_0(\mu)|= \bar J -\dim(Z(\mu)), |\widetilde{{\cal H}}_1(\mu)| =  \dim(Z(\mu + C\sqrt{\log d/n}))$. 
%$\bar{S}(\mu)=\min_{\{e_j\in N_j(\mu):1\leq j\leq d\}}\big|\{(j_1,j_2)\in {\cal H}_0(\mu) \times {\cal H}_0(\mu): j_1\neq j_2,|\text{Cov}(\xi(e_{j_1}),\xi(e_{j_2}))|\geq C\log d^{-2-\gamma} \}\big|$ 
\end{assumption}


% \begin{assumption}\label{ass:signalph}
% \[
%  \sup_{0\leq \mu\leq \mu_1}\bigg\{ \underbrace{\frac{(\log d)^{25/ 6}}{\rho(\mu)n^{1 / 6}} + \frac{(\log d)^{17 / 6} }{ \rho(\mu)^{4 / 3}n^{1 / 6}} + s\frac{(\log d)^4 }{\rho(\mu)\sqrt{n}}  +  \frac{\log d}{\rho(\mu)|\bar{{\cal H}}_0(\mu)|}}_{\text{Sparsity effect}} +\underbrace{\frac{\log d \bar{S}(\mu)}{\rho(\mu)|\bar{{\cal H}}_0(\mu)|^2}}_{\text{Dependence effect}}\bigg\}=o(1),
% \]
% where 
% \[
%   \rho(\mu):=\frac{|\widetilde{{\cal H}}_1(\mu)|}{J};\qquad \bar{S}(\mu):= \sum_{\substack{j_{1}, j_{2} \in \bar{{\cal H}}_0(\mu)\\j_{1} \neq j_{2}}}|S_{j_1,j_2}(\mu)|
% \]
% with
% \begin{align*}
%  &\tilde{{\cal H}}_1(\mu)=\Bigl\{j \in \bar{{\cal H}}_1(\mu): |\Theta^\star_{e^*_j}|>\mu+ C_0 \sqrt{\frac{\log d}{n}}\Bigr\},\\
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     &S_{j_1,j_2}(\mu)=\Big\{\big(e^*_{j_1},e^*_{j_2}\big) : (k_1,l_1)=e^*_{j_1}, (k_2,l_2)=e^*_{j_2},\Theta^\star_{k_1k_2} \Theta^\star_{l_1l_2}+\Theta^\star_{k_1l_2} \Theta^\star_{k_2l_1} \neq 0 \Big\}.
% \end{align*}
% \end{assumption}
{   In the above assumption, $|\widetilde{{\cal H}}_1(\mu)|$ counts the number of critical edges with  strong signals.}
Generally, to obtain guarantee on  complete persistent barcodes, one at least needs to set $\mu_1=\max_{j\in [\bar{J}_k],k\in D}W^*_{\bar{e}_k(j)}-C\sqrt{\frac{\log d}{n}}$ for some constants $C$.  Note that if the filtration level $\mu\geq  \mu_1$,  the signals would be too weak and sparse to gain statistical power. Compared to Assumptions~\ref{ass:spadepend} with (\ref{eq:NHS:GGM}), Assumption \ref{ass:phspadepend} requires a uniform control of the conditions on a range $(\mu_0,\mu_1)$ of interest. Note that as $\mu$ increases,  $|\tilde{{\cal H}}_1(\mu)|$ counts less critical edges that satisfy the signal conditions. At the same time,  $\bar{S}(\mu)$ which measure dependence and $|\bar{{\cal H}}_0(\mu)|$ which counts true null critical edges would be larger for greater $\mu$. Similarly, it holds for many graphfical models that $\bar{S}(\mu)=O\big(|\bar{{\cal H}}_0(\mu)|\cdot s(\mu)^2|D|\big)$ where  $s(\mu)$ is the maximum degree of graph $G^*(\mu)$. As such, we only require $|\widetilde{{\cal H}}_1(\mu)|\gg |D|s(\mu)^2\log d$  for any $\mu \in (\mu_0,\mu_1)$  to control dependence effect.  If we test for bounded dimensions of cycle group (i.e., $|D|\leq C$) and so this only requires the $|\widetilde{{\cal H}}_1(\mu)|\gg s(\mu)^2\log d$  for most of the region of the barcodes except for the tail of the barcodes at the large filtration level, where signals could be too weak and are too sparse to do inference. 
Therefore, Assumption \ref{ass:phspadepend} is  only an adaptive and delicate extension of Assumption \ref{ass:spadepend} to the persistent homology setting.%{  requires stronger balance between dependence measure $\bar{S}(\mu)$ and the number of true null hypotheses $|\bar{{\cal H}}_0(\mu)|$ and that between $\rho(\mu)$ and $|\bar{{\cal H}}_0(\mu)|$ or sample size $n$.}  %To reduce large 

Now, we are ready to present  the following characterization of the statistical guarantee for the persistent barcodes obtained by Algorithms \ref{alg:ph:barcode}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}[General FDR and power guarantee  for persistent barcodes]{theorem}{thmphgeneralfdppow}\label{thm:ph:generalfdppow}
Suppose $\log d/\log n=O(1)$ and  Assumptions \ref{assum:That:condition} and \ref{ass:phspadepend} are satisfied for some $\mu_1$, we have the persistent barcodes yielded by Algorithm \ref{alg:ph:barcode}
\[
\mathrm{uFDP}\leq q+o_P(1),\qquad \mathrm{uFDR}\leq q +o(1). 
\]
We also have 
\begin{equation*}
\mathbb{P}\Bigl(Z \big(\mu + C\sqrt{\log d/n} \big) \subseteq \hat{ Z}(\mu) \text{ for all }\mu\in(\mu_0,\mu_1) \Big) = 1- o(1).
\end{equation*}
\end{restatable}

{   In the above theorem, $C\sqrt{\log d/n}$ is a signal strength condition. At level $\mu$, we are able to select the cycle group with signal strength exceeding $\mu + C\sqrt{\log d/n}$ with high probability.}

%  Note that the second claim directly implies that guarantee of power with natural definition
% \begin{equation*}
% \mathbb{P}\Bigl(\Phi^{(k)}_{j,\mu}=1,\text{ for all }(j,k)\in \widetilde{{\cal H}}_1(\mu) \text{ and all }\mu\in(\mu_0,\mu_1) \Big) = 1- o(1).
% \end{equation*} 
% However, the argument in Theorem \ref{thm:ph:generalfdppow} is stronger since it says that the whole homology group instead of one basis of the homology group can be selected. 
%The proof of this theorem is deferred to Section \ref{sec:pfthm:ph:generalfdppow} in the Appendix.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In comparison with Theorem \ref{thm:generalfdp}, Theorem \ref{thm:ph:generalfdppow}  develops uniform control of tail probability of FDP and FDR on the filtration region  $(\mu_0,\mu_1)$ rather than that on a single point $\mu=0$. 

{    Compared to Theorem \ref{thm:generalfdp}, the theoretical results here are more satisfactory for several folds.} First, it uses a simpler Assumption \ref{ass:phspadepend} where the sparsity and dependence structure between nulls are clearer through critical edges. Second, it characterizes the inherent linear independent targets (cycles) out of linear dependent targets, which is new in theory. Moreover, it does not need complicated conditions for multiplicity controls, while we note that  the cycles are global structure of the underlying graph. Third, the argument is developed on continuous filtration levels such that we are able to depict the persistence of the features with stronger statistical guarantee, which is also new in the literature.  On the other hand, Algorithm \ref{alg:1} is still useful and powerful in the sense that they  can select features that not are characterized by persistent homology, such as star, tree, etc..

The main idea of the proof of Theorem \ref{thm:ph:generalfdppow} is to utilize the following lemma. 
\begin{restatable}[Equivalence of Algorithms]{lemmma}{lemeqialgph}\label{lem:eqi:algph} The persistent barcodes determined by Algorithm \ref{alg:ph:barcode} is equivalent to that determined by running Algorithm \ref{alg:ph:basis} through the whole filtration line $\mu\geq 0$ in the sense that at each filtration level $\mu$, $\hat{ Z}(\mu)$ are the same. 
\end{restatable}
%{    Lemma \ref{lem:eqi:algph} states that the representation of the cycles does not affect their significance.}
Based on Lemma \ref{lem:eqi:algph}, it suffices to develop statistical controls on uFDP and uFDR for the cycles selected by Algorithm \ref{alg:ph:basis} on $\mu \in (\mu_0,\mu_1)$.


%\yue{switch the order of Lem 5.4 and Thm 5.3?}

% At the same time, noting that multiple testing problem (\ref{eq:ph:mt:space})  is eqivalent to the following problem 
% \begin{equation}\label{eq:ph:mt:criedge}
%      H_{0j}^{(k)}(\mu):\bar{e}_k(j)\notin E^*(\mu),\qquad\text{v.s.}\qquad H_{1j}^{(k)}(\mu):\bar{e}_k(j)\in E^*(\mu).
% \end{equation}
% Specifically,  we focus on studying multiple testing problem (\ref{eq:ph:mt:criedge}) such that the study of selected cycles could reduce to the study of critical edges where it is simpler to study FDP and power and we do not need multiplicity controls. We leave the details to the Section \ref{sec:pfthm:ph:generalfdppow} in the appendix.

Similarly to the two models discussed in Section \ref{sec:example:GGM} and \ref{sec:example:Ising}, we also have the following corollaries for the Gaussian graphical model and the Ising model.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}[Statistical guarantee on the persistent barcodes under GGM]{corollary}{corbarcodeGGM}\label{cor:ph:barcodeGGM} Suppose Assumption \ref{ass:phspadepend} is satisfied for some $\mu_1>0$ and $\log d/\log n=O(1)$. 
For Gaussian graphical model with $\Theta^*\in {\cal U}(s)$, we further assume $s^2\log^4(dn)/n=o(1)$, then the persistent barcodes obtained by Algorithm \ref{alg:ph:barcode}  satisfies: for any $\epsilon>0$ 
\[
\mathrm{uFDP}\leq q+o_P(1),\qquad \mathrm{uFDR}\leq q +o(1).
\]
and
\begin{equation*}
\mathbb{P}\Bigl(Z \big(\mu + C\sqrt{\log d/n} \big) \subseteq \hat{ Z}(\mu) \text{ for all }\mu\in(\mu_0,\mu_1) \Big) = 1- o(1).
\end{equation*}   
\end{restatable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}[Statistical guarantee on the persistent barcodes under Ising models]{corollary}{corbarcodeIsing}\label{cor:ph:barcodeIsing} Suppose Assumption \ref{ass:phspadepend} is satisfied for some $\mu_1>0$ and $\log d/\log n=O(1)$. 
For Ising models with $w^*\in {\cal W}$, then the persistent barcodes obtained by Algorithm \ref{alg:ph:barcode}  satisfies: for any $\epsilon>0$, 
\[
\mathrm{uFDP}\leq q+o_P(1),\qquad \mathrm{uFDR}\leq q +o(1),
\]
and
\begin{equation*}
\mathbb{P}\Bigl(Z \big(\mu + C\sqrt{\log d/n} \big) \subseteq \hat{ Z}(\mu) \text{ for all }\mu\in(\mu_0,\mu_1) \Big) = 1- o(1).
\end{equation*}   
\end{restatable}

%\yue{ PF can be deleted?}

% We start by outlining the technical challenges of the multiple testing problem \ref{eq:ph:mt:basis}.

% \paragraph{Heavy dependence:} Note that one critical edge may relate to homology groups of different orders. Therefore, the dependency across different dimensions could be quite heavy, and what conditions needed to control the dependence are in question.

% \paragraph{Unspecified structure of cycles:} the size of the cycles hinges on the general underlying graph structure and could be as large as $d$. How to study global properties of graph without using multiplicity control are new in the literature.

% \paragraph{Uniform control on an interval:} To provide reasonable guarantee for persistent barcodes, we need to study statistical analysis of false discoveries and power are on uniform intervals, which is new in the literature.

 
 
% \subsection{Confidence interval of the topological features}
% %{  why do we need confidence interval or why is it interesting}

% One may also be interested in evaluating the uncertainty of the death time of the topological features. Confidence interval for topological feature has been proposed in \cite{fasy2013statistical} which is for  point clouds data, but that developed on the popular graphical model here haven't been proposed in the literature. 

% Below, by the similar idea of that used in Algorithm \ref{alg:fastbc}, we provide a fast way to construct  confidence intervals of  the death level $\mu_j$ of $j$-th topological feature in the barcode with global guarantee. %Recall that $E$ is the possible edge set for the whole graph. 
% For each $j=1,2,\ldots, J$, we propose the $1-\alpha$ confidence interval for $\mu_j$  to be %(i.e., $\min_{e\in {\color{red}l_j} }\{|\Theta_e|\}$) for loop $j$ as follow
% \begin{equation}\label{eq:phCI:1}
%     \Bigl[\min_{e\in E(F_j) }\widetilde{\Theta}_e-\hat{c}(\alpha,E), \max_{e\in  E(F_j) }\widetilde{\Theta}_e+\hat{c}(\alpha,E)\Bigr],\qquad \text{where } E=\{(u,v)\in E:u\neq v\},
% \end{equation}
% where $\hat{c}(\alpha,E)$ is the $1-\alpha$ quantile of statistic $\sqrt{n}\max_{e \in E} \Bigl\{ \bigl|{\widetilde{\Theta}_{e}-\Theta^*_{e}}\bigr|\Bigr\}$.
% %where $1-\alpha$ is the simultaneous confidence level for all $J$ loops.

% These confidence intervals share a uniform confidence band and are able to provide simultaneous statistical guarantee as follow.
% \begin{restatable}[Confidence intervals for the death time with global guarantee]{theorem}{lemCIloops}\label{lem:CIloops} For any $\alpha\in (0,1)$, we have %Let $E=\{(u,v)\in E:u\neq v\}$, then we have
% \[
%  \mathbb{P}\Bigl(\mu_j\in \Bigl[\min_{e\in  E(F_j) }\widetilde{\Theta}_e-\hat{c}(\alpha,E), \max_{e\in  E(F_j) }\widetilde{\Theta}_e+\hat{c}(\alpha,E)\Bigr],j=1,2\ldots,J\Bigr)\geq 1-\alpha.
%  \]
% \end{restatable}
% Note that the proof of this theorem does not need Assumption \ref{ass:phspadepend} and only requires elementary probability statement.  One may hope to obtain   confidence intervals that are adaptive to each subgraph structure. In fact, combining the ideas of Algorithms \ref{alg:ph:barcode}-\ref{alg:fastbc}, we can generalize the bands (\ref{eq:phCI:1}) for each $j$-th topological feature  as follow: (let $c_j=\max_{V\in {\cal V}}\big\{\hat{c}(\alpha/|{\cal V}|,E_V):E_V=\{(x,y)\in {\cal V}\times {\cal V}, \text{ s.t., }E(F_j)\subseteq E_V\}\big\}$, for all $j\in [J]$)
% \[
% \Bigl[\min_{e\in E(F_j) }\widetilde{\Theta}_e-c_j, \max_{e\in  E(F_j) }\widetilde{\Theta}_e+c_j\Bigr].%,\qquad \text{where } E=\{(u,v)\in E:u\neq v\}.
% \]
% Here the length of each confidence band $c_j$ is adaptive to the structure of the $j$-th topological feature since the maximum is taken over all large subgraphs that contain that feature. The simultaneous statistical guarantee is provided by a Bonferroni correction in the confidence level in terms of the number of domain block in ${\cal V}$ i.e., changing   $\alpha$ to $\alpha/|{\cal V}|$. Note that by utilising the combinatorial struture of graph, the correction in the number of domain block is able to provide simultaneous coverage to all $J$ features (where $J$ is usually much larger than $|\cal V|$). Therefore, in practice, we may obtain narrower confidence intervals by a good use of domain knowledge in ${\cal V}$. Its proof of coverage is also by elementary probability and needs no additional assumptions.  For simplicity, we just provide theoretical results and simulations for the simpler version (\ref{eq:phCI:1}). We refer it to Section \ref{sec:CIproof} in the appendix.
% \clearpage
% %{  describe theorem, and the conditions it requires uniform bound, and how to design more complex confidence interval. proofs}
% %Recall that $E$ is the possible edge set for the whole graph. For $j=1,2,\ldots, J$, we can also construct a confidence interval for the signal level (i.e., $\min_{e\in {\color{red}l_j} }\{|\Theta_e|\}$) for loop $j$ as follow
% %\[
% %\Bigl[\min_{e\in l_j }\{\widetilde{\Theta}_e\}-\hat{c}(\alpha,E), \max_{e\in l_j }\{\widetilde{\Theta}_e\}+\hat{c}(\alpha,E)\Bigr]
% %\]
% %where $1-\alpha$ is the simultaneous confidence level for all $J$ loops.

% %\begin{restatable}[Confidence intervals for loops]{lemmma}{lemCIloops}\label{lem:CIloops}
% %\[
% % \mathbb{P}\Bigl(\min_{e\in l_j }\{|\Theta_e|\}\in \Bigl[\min_{e\in l_j }\{\widetilde{\Theta}_e\}-\hat{c}(\alpha,E), \max_{e\in l_j }\{\widetilde{\Theta}_e\}+\hat{c}(\alpha,E)\Bigr],j=1,2\ldots,J\Bigr)\geq 1-\alpha.
% % \]
% %\end{restatable}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%% OCT 14 combinatoral calcualtions. Not efficient%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \iffalse
% %%%%%%% 
% \begin{algorithm}[H]
%     \caption{ \label{alg:homology}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     Denote $\cE(q)= \big\{(x,y)\in E: \sqrt{n}|\widetilde{\Theta}_{xy}| \geq \widehat{c}\Bigl(q, \{(x,y)\}\Bigr)$, %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$
%     %$\cE_{0}(q)= \big\{(x,y)\in E: \sqrt{n}|\widetilde{\Theta}_{xy}| <  \widehat{c}\Bigl(q, \{(x,y)\}\Bigr)$.
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$.
    
%     Let $\cG(q)=(V,\cE(q))$.
    
%     \For{$j = 1,2, \ldots, J$}{
    
%     \If{$G_j^* \subseteq \cG_{j}(q):=(V_j,\cE_{j}(q))  $ where $ \cE_{j}(q)= \{(x,y)\in V_j \times V_j: (x,y)\in \cE(q) \} $}{
%     Let $ E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$. 
    
%     We order the elements in the set $\Bigl\{\widetilde{\Theta}_e:e\in {E_{0,j}}\Bigr\}$ as $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}|$, where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
 
%     Define $K_{j}=\min\Bigl\{1 \leq k \leq\left|E_{0,j}\right|:G_j^* \subseteq (V_j,\{e_{(1)},  ..., e_{(k)}\})\Bigr\}$\;
   
%     Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e_{(k)}}|, E_{j}^{(k)}\Bigr)$  with $E_{j}^{(k)}=\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\}$, for $1 \leq k \leq K_{j}$\;
    
%     Let $\alpha_{j}=\max_{1 \leq k \leq K_{j}}\{\alpha_{uv}\}$    \; 
    
%     }
%     \Else{
%     Let $\alpha_{j}=1$\;
%     }
%     }
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}
% In selecting the homology holes ($k$-dimensional circles) of a graph $G$, we can set $G^*_j$ be self-avoiding loops with size $k$ for $1\leq j\leq \tbinom{d}{k}$, $k\geq 3$ and run the algorithm. If we focus on loops with size less than $m$, then by elementary combinatorial calculations, $J=\sum_{k=3}^{m}\tbinom{d}{k}$.


% \begin{proposition}[(FDP/FDR control)]. Under Assumption {  XX}, the algorithm with {  XX} as input and the quantiles approximated by XX satisfies: as $(n,d)\rightarrow \infty$,
% \[
% \mbox{FDP}\leq q\frac{J_0}{J}+o(1),\qquad \mbox{except for $o(1)$ probability}
% \]
% and
% \[
% \lim_{(n,d)\rightarrow \infty} \mbox{FDR}\leq q\frac{d_0}{d}
% \]
% \end{proposition}


% % 3.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%% Junwei's alg  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Let $L^*_s$ denote a self-avoiding loop consist of $k$ edges, where $3\leq s\leq m$ and $m$ is a known bounded number or $m\leq \log d$. Let $M$ be a bounded number (e.g. $M=1$). For $j\in [\tbinom{d}{d-M}]$, we test whether the $j$-th subgraph has a topology hole by the following efficient algorithm
% \begin{algorithm}[htbp]
%     \caption{Selecting homologic holes in $j-$th subgraph }
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,   significance level $\alpha$. }
%     Initialize {  $t=0,\, E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$, and $E_{0,j}^c=\emptyset.$}%\{(j_1, j_2)\in V_j \times V_j:j_1\neq j_2\}$}. %\{(j_1, j_2): \text{all edges between the $j$-th set of nodes $V_j$}\}$.
   
%     \Repeat{${  L^*_s \subseteq  (V_j,E_{t,j}^{c}) }$  for some  $3\leq s\leq m$   or  $\mathcal{R}=\varnothing$}
%     { 
%     $t \leftarrow t+1$\;
    
%     Select the rejected edges $\mathcal{R} \leftarrow\Bigl\{(j_1, j_2) \in E_{t-1,j}:\,\sqrt{n}| \widetilde{{\Theta}}_{j_1 j_2}\big|>\widehat{c}\Bigl(\alpha, E_{t-1,j}\Bigr)\Bigr\}$\;
    
%     $E_{t,j} \leftarrow E_{t-1,j} \backslash \mathcal{R}$ and  $E_{t,j}^c \leftarrow E_{t-1,j}^c \cup \mathcal{R}$\;
%     }
%   	\Output{$\psi_{j, \alpha}=1$ if $L^*_s \subseteq  (V_j,E_{t,j}^{c})  \mbox{ for some } s\geq 3 $; $\psi_{j, \alpha}=0$, otherwise.}%$G^* \subseteq E_{t,j}^{c}$, $\psi_{j, \alpha}=0$ otherwise.}
% \end{algorithm}


% \begin{algorithm}[H]
%     \caption{Selecting homologic holes in $j-$th subgraph (efficient version)}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     \For{$j = 1,2, \cdots, J$ where  $J:=\binom{d}{d-M}$}{
%     \If{$ \cG_{j}(q):=(V_j,\cE_{j}(q))  $ has at least an $s$ loop where $ \cE_{j}(q)= \{(x,y)\in V_j \times V_j: (x,y)\in \cE(q) \} $ and $3\leq s\leq m$}{
    
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     Let $ E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$. %and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
    
%     We order the elements in the set $\Bigl\{\widetilde{\Theta}_e:e\in {E_{0,j}}\Bigr\}$ as $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}|$, where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
%     % Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|, E^*_{j}\Bigr)$ where $E^*_{j}=\Bigl\{\ell \neq j:\Bigl|\widetilde{\Theta}_{j \ell}\Bigr| \leq\Bigr.$
%     % $\Bigl.\Bigl|\widetilde{\Theta}_{j,\Bigl(k_{\tau}\Bigr)}\Bigr|\Bigr\}$
    
%   Define $K_{j}=\min\big\{1 \leq k \leq\left|E_{0,j}\right|:L^*_s \subseteq \{e_{(1)},e_{(2)},  ..., e_{(k)}\},\mbox{ for some }3\leq s\leq m\big\}$\;
   
%   Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e_{(k)}}|, E_{j}^{(k)}\Bigr)$  with $E_{j}^{(k)}=\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\}$, for $1 \leq k \leq K_{j}$\;
    
%     Let $\alpha_{j}=\max_{1 \leq k \leq K_{j}}\{\alpha_{uv}\}$    \; 
%         }
%     \Else{
%     Let $\alpha_{j}=1$\;
%     }
%     }  
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}
% \fi
% \iffalse
% \newpage
% \begin{algorithm}[H]
%     \caption{}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
    
%     Denote $\cE_{1}(q)= \big\{(x,y)\in \cV \times \cV: \sqrt{n}|\widetilde{\Theta}_{xy}| \geq \widehat{c}\Bigl(q, \{(x,y)\}\Bigr)$,
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$
%     $\cE_{0}(q)= \big\{(x,y)\in \cV \times \cV: \sqrt{n}|\widetilde{\Theta}_{xy}| <  \widehat{c}\Bigl(q, \{(x,y)\}\Bigr)$.
%     %(1-q) \text{ quantile of } \widetilde{\Theta}_{xy} - {\Theta}^*_{xy}\big\}$.
    
%     Let $\cG_1(q)=(\cV,\cE_1(q))$.
    
%     \For{$j = 1, \cdots, J$ where  $J:=\binom{d}{m}$}{
    
%     \If{$G^* \subseteq {   \cG_{1,j}(q):=(\cV_j,\cE_{1,j}(q)) } $ where ${   \cE_{1,j}(q)= \{(x,y)\in \cV_j \times \cV_j: (x,y)\in \cE_{1}(q) \} } $}{
%     Let $ E_{0,j}= \{(x, y)\in V_j \times V_j:x\neq y\}$. 
    
%     We order the elements in the set $\Bigl\{\widetilde{\Theta}_e:e\in {E_{0,j}}\Bigr\}$ as $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E_{0,j}|)}}|$, where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
%     denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
 
%     Define $K_{j}=\min\big\{1 \leq k \leq\left|E_{0,j}\right|:G^* \subseteq \{e_{(1)},  ..., e_{(k)}\}\big\}$\;
   
%     Compute $\alpha_{uv}=\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e_{(k)}}|, E_{j}^{(k)}\Bigr)$  with $E_{j}^{(k)}=\{e_{(k)}, e_{(k+1)}, ..., e_{(|E_{0,j}|)}\}$, for $1 \leq k \leq K_{j}$\;
    
%     Let $\alpha_{j}=\max_{1 \leq k \leq K_{j}}\{\alpha_{uv}\}$    \; 
    
%     }
%     }
    
%     Order $\alpha_{1},...,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Yue's algorithm for homology
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{algorithm}[htbp]
%     \caption{Select loops with FDR control. \label{alg:21}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{\Theta}$,  significance level $\alpha$. }
%     Denote $\cE_{1}(\alpha)= \big\{(i,j)\in \cV \times \cV: \widetilde{\Theta}_{ij} > (1-\alpha) \text{ quantile of } \widetilde{\Theta}_{ij} - {\Theta}^*_{ij}\big\}$, $\cE_{0}(\alpha)= \big\{(i,j)\in \cV \times \cV: \widetilde{\Theta}_{ij} \leq (1-\alpha) \text{ quantile of } \widetilde{\Theta}_{ij} - {\Theta}^*_{ij}\big\}$.
    
%     Let $\cG_1(\alpha)=(\cV,\cE_1(\alpha))$.
   
%     \For{\text{each possible loop } $\cL_k \subseteq \cG_1(\alpha), k = 1, \cdots, K(\alpha)$}{
%     Test if $\cL_k$ is a loop using skip-down with threshold $\alpha$.
%     }
  	
%     \Output{$\psi_{k, \alpha}=1$ if $\cL_k$ is a loop, $\psi_{k, \alpha}=0$ otherwise.}
% \end{algorithm}
% And we estimate $\alpha$ by BHq that
% \begin{equation}
% \widehat{\alpha}=\sup \left\{\alpha \in(0,1): \frac{\alpha   {(2^d-d-\binom{d}{2})}}{\max \left\{1, \sum_{k \in [K(\alpha)]} \psi_{k, \alpha}\right\}} \leq q\right\}, 
% \end{equation}
% where $K(\alpha)$ is the number of possible loops in graph $\cG_1=(\cV,\cE_1)$.
% {\color{red} what if the subgraph is very sparse? e.g., there are only $d$ edges }%Question

% \begin{algorithm}[htbp]
%     \caption{Select loops with FDR control. \label{alg:22}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{\Theta}$,  significance level $q$, upper bound of $\alpha$: $\alpha^{U}$. }
%     Denote $\cE_{1}(\alpha^{U})= \big\{(i,j)\in \cV \times \cV: \widetilde{\Theta}_{ij} > (1-\alpha^{U}) \text{ quantile of } \widetilde{\Theta}_{ij} - {\Theta}^*_{ij}\big\}$, $\cE_{0}(\alpha^{U})= \big\{(i,j)\in \cV \times \cV: \widetilde{\Theta}_{ij} \leq (1-\alpha^{U}) \text{ quantile of } \widetilde{\Theta}_{ij} - {\Theta}^*_{ij}\big\}$.
    
%     Let $\cG_1(\alpha^{U})=(\cV,\cE_1(\alpha^{U}))$.
   
%     \For{\text{each possible loop } $\cL_k \subseteq \cG_1(\alpha^{U}), k = 1, \cdots, K(\alpha^{U})$}{
%     Denote the $|\cL_k|$ edges in $\cL_k$ as $\{e_{k1},  e_{k2},...,e_{j|\cL_{k}|}\}$
    
%     We order the elements in set $\left\{\left|\widetilde{\boldsymbol{\Theta}}_{\cL_k}\right|\right\}$ as $\left|\widetilde{\boldsymbol{\Theta}}_{e_{k(1)}}\right| \geq\left|\widetilde{\boldsymbol{\Theta}}_{e_{k(2)}}\right| \geq \ldots \geq\left|\widetilde{\boldsymbol{\Theta}}_{e_{k(|\cL_k|)}}\right|$, where $\left|\widetilde{\boldsymbol{\Theta}}_{e_{k(l)}}\right|$
%     is the $l$-th largest entry. 

%     Compute $\alpha_{kl}=\widehat{c}^{-1}\left(\sqrt{n} | \widetilde{\Theta}_{e_{k(l)}}|, E_{kl}\right), 1\leq k \leq |\cL_{k}|$ where $E_{kl}=\{e_{k(l)}, e_{k(l+1)}, ..., e_{k(|\cL_{k}|)}\}$ \;
    
%     Let $\alpha_{k}=\max_{1\leq l \leq |\cL_{k}|}\alpha_{kl}$\; 
%     }  
    
%     Order $\alpha_{1},...,\alpha_{K}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(K)}$ and set $\alpha_{(0)}=0$. Let $k_{\max}=\max \left\{0 \leq k \leq K: \alpha_{(k)} \leq q k /   {K}\right\}$.
    
%     \Output{Reject $\left\{k: \alpha_{k} \leq \alpha_{\left(k_{\max }\right)}\right\}$ if $k_{\max }>0$; reject $\varnothing$ otherwise.}
% \end{algorithm}
% \yue{obtain upper bound of $\alpha$: $\alpha^{U}$}

% \fi




% % \newpage

% % \begin{figure}[h!]
% % 	\begin{center}
% % 		\begin{tabular}{cc}		
% % 		\includegraphics[height=.5\textwidth,angle=0]{./figure/barcode} \\
% % 			[-10pt]
% % 		\end{tabular}
% % 	\end{center}
% % 	\caption{Figure from CH2013.}
% % 	\label{fig:barcode}
% % \end{figure}


% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%% Appendix %%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \clearpage

% % \appendix

% %\end{equation}
% %%% Local Variables:
% %%% TeX-master: "atlas"
% %%% End:

 
\section{Numerical Experiments}\label{sec:simulation}

%\subsection{Synthetic data}

In this section, we examine the performance our method through numerical simulations. 

\subsection{Simulation for general subgraph selection}\label{sec:sim:gss}
We consider the Gaussian graphical model and the Ising model in Section \ref{sec:application}. In particular, we focus on the performance of the proposed methods as we vary the dimension $d$, sample size $n \in \{300,350,400\}$, the nominal level $q \in \{0.05,0.1\}$ and the types of sub-graphs. For illustration, in the Gaussian graphical model, we focus on the detection of triangles, four-cycles and five-cycles, while in the Ising model, we focus on the detection of five-trees, which are trees consisting of five nodes with three possible shapes, as illustrated in Figure~\ref{fig:sim0}.  We estimate the empirical FDR and power based on $100$ repetitions.


\begin{figure}[h]
\begin{tabular}{cc}
     \includegraphics[width=0.2\textwidth]{figure/Graph_Gaussian.pdf} &
 \includegraphics[width=0.2\textwidth]{figure/Graph_Ising.pdf}  \\
 (a) Sug-graphs for the Gaussian model & (b) Sug-graphs for the Ising model
\end{tabular}
\caption{Sub-graphs to test for the Gaussian graphical model and the Ising model. }
\label{fig:sim0}
\end{figure}

The Gaussian graphical model is generated as follows. First, we generate the adjacency matrix consisting of triangles, four-cycles and five-cycles: $3 m_1$ nodes form $m_1$  triangles, $4 m_2$ nodes form $m_2$ four-cycles, and  $5 m_3$ nodes form $m_3$ five-cycles, while these sub-graphs have no overlapping nodes with each other. Then dimension $d = 3m_1 + 4 m_2 +  5 m_3$. To make the problem more challenging, we randomly add one edge to the four-cycles and three edges to the five-cycles with an example of the adjacency matrix illustrated in Figure~\ref{fig:sim} (a). %In this way, the number of total triangles can be larger than $m_1$. 
We then generate the entries of precision matrix $\Theta^*$ by sampling from ${\rm Uniform}(0.85,1)$ for edges in the adjacency graph and setting other entries as zero. Finally, we add a small value $v = 0.1$ together with the absolute value of the minimal eigenvalue of $\Theta^*$ to the diagonal elements of $\Theta^*$ to ensure its positive-definiteness. We take different combinations of $(m_1,m_2,m_3)$:  $(20,10,20)$, $(20,10,30)$, $(40,20,20)$ and $(60,30,10)$, which yield $d = 200, 250, 300$ and $350$, respectively. 

%the $(d_0 + r \times i + 1)$th node to the $(d_0 + r \times i + r )$th node form a  triangles for $d_0 = 0$, $r=3$, $i = 0,\ldots,m_1$,  form a four-cycle for $i = 0,\ldots,m_1$ and $r=3$, 

The Ising model is generated similarly where the adjacency graph  consisting of $m$-trees with $m$ sampled uniformly from $6$ to $10$ as illustrated by Figure ~\ref{fig:sim} (b). The dimension $d$ is also chosen from $\{200, 250, 300,350\}$ where the last few nodes (with size smaller than $m$) are set to be disconnected with all other nodes. We sample $w_e^{*}$ from ${\rm Uniform}(0.9,1)$ for all edges $e$'s in the adjacency graph and set $w_e^{*} = 0$ otherwise. The thresholding value $\theta$ in \eqref{eq:That:Ising} is set as $0.45$. 

\begin{figure}[h]
\begin{tabular}{cc}
     \includegraphics[width=0.2\textwidth]{figure/Gaussian.pdf} &
 \includegraphics[width=0.2\textwidth]{figure/Ising.pdf}  \\
 (a)Graph of the Gaussian graphical model & (b) Graph of the Ising model
\end{tabular}
\caption{Examples of the adjacency graphs used for the Gaussian graphical model and  the Ising model.}
\label{fig:sim}
\end{figure}

The results for the Gaussian graphical model is presented in Table~\ref{tab1}. We can see that the FDRs of all configurations are well controlled by their nominal level $q$ while the power is pretty good for all configurations. Specifically, with the sample size $n$ increases, the FDRs tend to decrease. %which is reasonable since more samples can lower down the probability of making type
The FDRs for detection triangles are larger than those of four-cycles and five-cycles since there are more hypotheses to test for four cycles and five cycles compared to  triangles. 

The results for the Ising model is presented in Table~\ref{tab2}. The similar pattern is observed as the Gaussian graphical model. All FDRs are below the nominal level $q$ for different values of $n,d$ and $q$. The power increases quickly as the sample size $n$ increases. The results of the five-tree (a) and five-tree (b) are more similar compared to that of five-tree (c), as the numbers of hypotheses are same for testing five-tree (a) and five-tree (b). 


\begin{table}[]
  \centering
  \caption{ Empirical FDR and power averaged over $100$ repetitions in the detection of triangles, four-cycles and five-cycles under the Gaussian graphical model. }
      %\scalebox{0.65}
    {
    \resizebox{.97\columnwidth}{!}{
    \begin{tabular}{l|rrrrrrrrrrrr}
%    \multicolumn{13}{c}{v=1,u=0.1,omega=[0.85,1],seed=1,d=(200,250,300,350)} \\
\hline 
  $q$        & \multicolumn{3}{c|}{ $0.05$ } & \multicolumn{3}{c|}{ $0.1$ } & \multicolumn{3}{c|}{ $0.05$ } & \multicolumn{3}{c}{ $0.1$ } \\ \hline 
   $n$     & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & \multicolumn{1}{r|}{400} & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & \multicolumn{1}{r|}{400} & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & \multicolumn{1}{r|}{400} & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & 400 \\ \hline 
          & \multicolumn{6}{c|}{FDR}                      & \multicolumn{6}{c}{Power} \\ \hline 
    $d$     & \multicolumn{12}{c}{(i) Triangle} \\ 
    200   & 0.031 & 0.025 & 0.020 & 0.040 & 0.033 & 0.025 & 0.999 & 1.000 & 1.000 & 0.999 & 1.000 & 1.000 \\
    250   & 0.036 & 0.034 & 0.033 & 0.046 & 0.045 & 0.042 & 0.999 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
    300    & 0.029 & 0.030 & 0.030 & 0.037 & 0.037 & 0.039 & 0.999 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
    400    & 0.029 & 0.025 & 0.026 & 0.036 & 0.031 & 0.032 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\ \hline 
    $d$     & \multicolumn{12}{c}{(ii) Four-cycle} \\ 
    200   & 0.011 & 0.008 & 0.005 & 0.014 & 0.011 & 0.007 & 0.996 & 1.000 & 1.000 & 0.997 & 1.000 & 1.000 \\
250    & 0.012 & 0.013 & 0.012 & 0.016 & 0.016 & 0.016 & 0.992 & 0.999 & 1.000 & 0.994 & 1.000 & 1.000 \\
    300    & 0.011 & 0.009 & 0.009 & 0.013 & 0.012 & 0.012 & 0.992 & 0.998 & 1.000 & 0.994 & 0.999 & 1.000 \\
    400   & 0.011 & 0.010 & 0.011 & 0.014 & 0.013 & 0.014 & 0.990 & 0.998 & 1.000 & 0.992 & 0.999 & 1.000 \\ \hline 
   $d$     & \multicolumn{12}{c}{(iii) Five-cycle} \\
    200   & 0.001 & 0.002 & 0.001 & 0.001 & 0.002 & 0.001 & 0.961 & 0.988 & 0.997 & 0.964 & 0.989 & 0.997 \\
    250   & 0.003 & 0.004 & 0.003 & 0.004 & 0.005 & 0.003 & 0.958 & 0.987 & 0.994 & 0.965 & 0.988 & 0.994 \\
    300  & 0.002 & 0.003 & 0.002 & 0.003 & 0.003 & 0.002 & 0.941 & 0.981 & 0.992 & 0.947 & 0.982 & 0.993 \\
    400  & 0.001 & 0.002 & 0.002 & 0.002 & 0.002 & 0.003 & 0.914 & 0.976 & 0.993 & 0.925 & 0.979 & 0.994 \\
    \bottomrule
    \end{tabular}%
    }
    }
  \label{tab1}%
\end{table}%

\begin{table}[htbp]
  \centering
  \caption{ Empirical FDR and power averaged over $100$ repetitions in the detection of triangles, four-cycles and five-cycles under the Ising model.}
   %   \scalebox{0.65}
    {
    \resizebox{.97\columnwidth}{!}{
    \begin{tabular}{l|rrrrrrrrrrrr}
   % \multicolumn{13}{c}{omega=[0.9,1],beta=0.45,seed=1,m=sample(6:10,1),d=(200,250,300,350)} \\
   \hline 
  $q$        & \multicolumn{3}{c|}{ $0.05$ } & \multicolumn{3}{c|}{ $0.1$ } & \multicolumn{3}{c|}{ $0.05$ } & \multicolumn{3}{c}{ $0.1$ } \\ \hline 
   $n$     & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & \multicolumn{1}{r|}{400} & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & \multicolumn{1}{r|}{400} & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & \multicolumn{1}{r|}{400} & \multicolumn{1}{r}{300} & \multicolumn{1}{r}{350} & 400 \\ \hline  
          & \multicolumn{6}{c|}{FDP}                      & \multicolumn{6}{c}{Power} \\ 
        \hline 
    $d$     & \multicolumn{12}{c}{ Five-tree (a)} \\
    200    & 0.014 & 0.020 & 0.032 & 0.018 & 0.024 & 0.040 & 0.531 & 0.770 & 0.888 & 0.575 & 0.800 & 0.902 \\
    250    & 0.011 & 0.013 & 0.025 & 0.013 & 0.018 & 0.030 & 0.461 & 0.744 & 0.870 & 0.505 & 0.774 & 0.886 \\
    300    & 0.009 & 0.012 & 0.016 & 0.011 & 0.014 & 0.020 & 0.452 & 0.678 & 0.838 & 0.492 & 0.710 & 0.857 \\
    400  & 0.005 & 0.007 & 0.012 & 0.006 & 0.009 & 0.014 & 0.379 & 0.627 & 0.834 & 0.416 & 0.661 & 0.851 \\ \hline
    $d$     & \multicolumn{12}{c}{ Five-tree (b)} \\
    200    & 0.017 & 0.024 & 0.037 & 0.021 & 0.030 & 0.046 & 0.524 & 0.775 & 0.889 & 0.571 & 0.802 & 0.903 \\
    250    & 0.012 & 0.017 & 0.027 & 0.014 & 0.022 & 0.032 & 0.479 & 0.748 & 0.881 & 0.515 & 0.777 & 0.899 \\
    300    & 0.010 & 0.011 & 0.021 & 0.012 & 0.013 & 0.026 & 0.464 & 0.687 & 0.841 & 0.505 & 0.719 & 0.861 \\
    400    & 0.006 & 0.009 & 0.012 & 0.007 & 0.011 & 0.017 & 0.398 & 0.631 & 0.837 & 0.431 & 0.671 & 0.857 \\ \hline
    $d$     & \multicolumn{12}{c}{ Five-tree (c)} \\ 
    200    & 0.016 & 0.030 & 0.026 & 0.017 & 0.033 & 0.032 & 0.420 & 0.579 & 0.732 & 0.450 & 0.606 & 0.754 \\
    250   & 0.013 & 0.022 & 0.026 & 0.015 & 0.025 & 0.032 & 0.402 & 0.611 & 0.764 & 0.437 & 0.640 & 0.778 \\
    300   & 0.008 & 0.011 & 0.019 & 0.010 & 0.011 & 0.028 & 0.384 & 0.568 & 0.729 & 0.428 & 0.593 & 0.747 \\
    400   & 0.007 & 0.008 & 0.010 & 0.008 & 0.011 & 0.018 & 0.358 & 0.524 & 0.747 & 0.385 & 0.551 & 0.776 \\ \hline 
    \end{tabular}%
    }
    }
  \label{tab2}%
\end{table}%


\subsection{Simulation for persistent homology}
Since the true correlation graph in Ising model does not have a explicit form, we only consider the Gaussian graphical model for the simulation in persistent homology part. 

The model is generated in a similar way to the settings in Section \ref{sec:sim:gss}. First, we generate the adjacency matrix consisting of triangles, four-cliques, and five-cliques: $3m_1$ nodes form $m_1$ triangles, $4m_2$ nodes form $m_2$ four-cliques, and $5m_3$ nodes form $m_3$ five-cliques, while these sub-graphs have no overlapping nodes with each other.  The sample size $n$ is $400$ and the dimension $d$ is $3m_1 + 4m_2 + 5m_3$. Similarly to the settings in Section \ref{sec:sim:gss}, we randomly reduce the edges of five cliques with probability $p = 0.1$. An example of the adjacency matrix is illustrated in Figure \ref{HomologyGraph}. We then generate the entries of the precision matrix $\Theta^*$ by sampling from Uniform$(0,10)$ for edges in the adjacency graph and setting other entries as zero. Finally, we add a small value $v = 0.25$ together with the absolute value of the minimal eigenvalue of $\Theta^*$ to the diagonal elements of $\Theta^*$ to ensure its positive definiteness. We set ($m_1$, $m_2$, $m_3$): $(10,30,10)$, which yields $d = 200$ respectively. The filtration level is set between $0$ and $1$.

The results for the Gaussian graphical model are presented in Figure \ref{HomologyResult}. We can see that the FDR is well controlled by their nominal level $q$ while the power is above 0.4. Specifically, as the filter level increases, the FDR tends to decrease. 
 
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.2]{figure/Graph.png}
    \caption{Graph of the Gaussian graphical model for persistent homology}
    \label{HomologyGraph}
\end{figure}


\begin{figure}[htbp]
\centering
\subfigure
{
\includegraphics[scale=0.4]{figure/FDR.png} \label{1}
}
\quad
\subfigure
{
\includegraphics[scale=0.4]{figure/Power.png} \label{2} 
}
\caption{Empirical FDR and power averaged over $100$ repetitions in the detection of homology under the Gaussian graphical model.}

\label{HomologyResult}
\end{figure}


\subsection{Real-world data example: SARS-CoV-2 Spike Protein}

%The novel coronavirus (SARS-CoV-2) pandemic resulted in the largest public health crisis in recent times. Significant drug design effort against SARS-CoV-2 is focused on the receptor-binding domain (RBD) of the spike protein, although this region is highly prone to mutations causing therapeutic resistance. We applied deep data analysis methods on all-atom molecular dynamics simulations to identify key non-RBD residues that play a crucial role in spike−receptor binding and infection. Because the non-RBD residues are typically conserved across multiple coronaviruses, they can be targeted by broad-spectrum antibodies and drugs to treat infections from new strains that might appear during future epidemics.

{\red Talk about the background. Then talk about how this problem can be formulated in the testing problem in the paper.}
We used the trajectory data from \citep{ray2021distant}. The data consists of three states of the SARS-CoV-2 spike protein, the closed, partially open, and fully open states. The protein has three chains and each chain consists of XX residuals. We use the backbone dihedral angles of these residuals as the features that 

Each chain has four domain: Linker, NTD, RBD and S2.  

Our goal is to select residues that play important roles in one of the three stages. We have three types of data: (i) distance, (ii) Angle 1{\jiajun use $\Psi$ or $\Phi$}, and (iii) Angle 2, for each of the three stages. Specifically, we have $T$ repeated measures for each stage. From the perspective of a spherical coordinate system, we can treat the distance and angles of a residue as roughly independent from each other.
%Our goal is to select residues that have important roles in one of the three stages. We have three kinds of data: (i) distance; (ii) Angle 1; (ii) Angle 2, in each of the three stages. In particular, in each stage, we have $T$ repeated measures. From the view of spherical coordinate system, we can roughly treat the distance and angles of a residue as being independent from each other.

{\red Yes, we can move it forward.) At each stage (e.g., open, partially open, close), residues that have strong connections with many other residues can be considered as important. By examining the changes in these important residues across the three stages, we may be able to identify residues that play crucial roles in the infection process. Below, we discuss our procedure at each stage. }
%At each stage, residues that have strong connections with many other residues can be considered as important ones. Then by examining the changes of important residues over the three stages, we may be able to find residues that play important roles in the infection process. 

 We use all of the available data to construct a Gaussian graphical model that models the correlations between the distances and angles of each residue, treated as nodes. This is done to incorporate the influence of the distance and angles of one residue on those of other residues. %We employ a Gaussian graphical model. %Note that  the angle data is on the interval $[-\pi,\pi]$. 
To better fit for Gaussian graphical model at each stage, we transform the angle  data into the real line using $\Phi^{-1}(\hat{P}(\cdot))$, where $\hat{P}(\cdot)$ denotes the empirical distribution of the data.
%Since one residue's distance and angles may affect the distance and angles of others residue, we use all the data to run a graphical model to model the correlation between  residues' distance, angle (i.e., each is considered as a node),  respectively for each stage. We exploit the Gaussian graphical model. Note that the angle data is on $[-\pi,\pi]$. For each type of angle data at each stage, we transform them into $\mathbb{R}$ through $\Phi^{-1}(\hat{P}(\cdot))$ where $\hat{P}(\cdot)$ is its empirical distribution.


%Next, we introduce the way how we measure the importance of a residue at each stage by leveraging persistent homology. 
We evaluate the importance of each residue in terms of the presence of its distance and angles in the persistent loops acting as the bases. Specifically, suppose we obtain the evolution of cycle groups using Algorithm \ref{alg:ph:barcode}. Equivalently, we can determine the loops that form the bases of the cycle groups (conventions for determining the loops are outlined in Section \ref{sec:findconven} in the Appendix). The persistence of each loop is determined by the length of the filtration interval during which it exists. The importance score of each residue is calculated as follows: the importance score of each feature (distance, angle) of each residue is obtained by summing the length of the filtration interval of the loop basis in which it exists. Then, the importance score of each residue is calculated by summing over the importance scores of its features.

 At each stage, we pick the top $10$ residues in terms of important score, which are summarized in Figures \ref{fig:protein}. Our method can find different residues in the three stages. We also identified residues identical to those reported in \citep{ray2021distant}, such as A570 and I569, indicating the effectiveness of our approach. Furthermore, our method discovered additional residues that were not reported in \citep{ray2021distant}, primarily located in the Link domain which has significant implications for the NTD domain. This suggests that the residues we have identified may also have important functional implications.

\textcolor{red}{As the filtration level increases, the number of nodes in the four domains we identified gradually decreases, as illustrated in \ref{fig:protein homo}}


\begin{figure*}[htbp]	
\centering
\begin{tabular}{ccc}
     \includegraphics[width=0.31\textwidth]{RealData/open.png} &
 \includegraphics[width=0.31\textwidth]{RealData/partially open.png} & 
 \includegraphics[width=0.31\textwidth]{RealData/closed.png}
 \\
 (a) Open & 
 (b) Partially Open &
 (c) Closed
\end{tabular}
\caption{Chain A: Red, Chain B: Blue, Chain C: Yellow. NTD: Light Blue, RBD: Green, Linker: Grey, S2: Khaki.}
\label{fig:protein}
\end{figure*}

\begin{figure*}[htbp]	
\centering
\begin{tabular}{ccc}
     \includegraphics[width=0.31\textwidth]{RealData/OpenDomainNumber.pdf} &
 \includegraphics[width=0.31\textwidth]{RealData/PartialDomainNumber.pdf} & 
 \includegraphics[width=0.31\textwidth]{RealData/ClosedDomainNumber.pdf}
 \\
 (a) Open & 
 (b) Partially Open &
 (c) Closed
\end{tabular}
\caption{Area Plot}
\label{fig:protein homo}
\end{figure*}

 
% persistent barcodes at stage $A$ ($A=1,2,3$) based on the  graphical model, from the persistent barcodes, we can actually obtain the persistence of each critical edge (i.e., the length of the filtration interval each critical edge persists). Note that, the critical edges can be classified to $12$ classes
% \begin{enumerate}
%       \item residue $a$'s distance to residue $a$'s Angle 1
%         \item residue $a$'s distance to residue $a$'s Angle 2
%         \item residue $a$'s Angle 1  to residue $a$'s Angle 2
%        {\bf \item residue $a$'s distance to residue $b$'s distance
%         \item residue $a$'s distance to residue $b$'s Angle 1
%         \item residue $a$'s distance to residue $b$'s Angle 2
%                 \item residue $a$'s Angle 1 to residue $b$'s distance
%         \item residue $a$'s Angle 1 to residue $b$'s Angle 1
%         \item residue $a$'s Angle 1 to residue $b$'s Angle 2
%                 \item residue $a$'s Angle 2 to residue $b$'s distance
%         \item residue $a$'s Angle 2 to residue $b$'s Angle 1
%         \item residue $a$'s Angle 2 to residue $b$'s Angle 2
%         }
% \end{enumerate}
%Among them, the last $9$ classes represent the correlation between one residue and the other one. Therefore, we only consider the critical edges that belong to the last $9$ classes. Moreover, the weights of the $9$ classes measures different relationships and may have different scales. We then construct $9$ ranking tables from them. For example, in the table for the class 3 ` residue $a$'s distance to residue $b$'s distance', we can evaluate the importance (score) of a residue's distance to others' distance by summing the persistence of the critical edges that belong to this class and involve that residue's distance. In this way, we obtain a ranking table for the residues for class 3. And we can do it for the other classes.

%To summarize the importance of the residues over all the $9$ classes, we may add the ranking of each residue in the $9$ ranking tables together  and then rank the added ranks to yield a overall ranking table.

%In particular, we may use  graphical model with {\bf normalized} weights to accommondate the heterogeneous scales of different weights. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
This paper proposes a flexible and general method to detect multiple subgraphs of different shapes simultaneously. Surprisingly, our method does not need maximal statistics and bootstrap for multiplicity control, and is much simpler and faster than existing methods for simultaneous combinatorial inference. Moreover, this paper develops a novel  algorithm PCET to select linearly independent subgraph features of a graph, which is novel in the literature. This algorithm  allows one to select cycle group  at a filtration level in computationally feasible time. Based on PCET, an efficient algorithm POEM is proposed to characterize the whole persistent barcodes of the subgraph features of a graph. 
%with generated from the stochastic block model. The $d$ nodes are assigned to $p$ blocks with equal size (the last block is of size $d - \lceil \frac{d}{p} \rceil (p-1)$). The within-block connected probability is  set as $p_0$ and the between-block  connected probability is set as $0.01$. With the adjacency matrix, we determine the precision matrix similar to  \cite{zhao2012huge}. Specifically, we set the off-diagonal elements as $v = 0.4$ and the diagonal elements as  $u=0.5$ plus the absolute value of the minimal eigenvalue to  ensure the  positive-definiteness of  the precision matrix. 
%We vary the sample size $n$ from $300$ to $500$, the dimension $d$ from $200$ to $400$, and consider the detection of (i) $4$-cycle, (ii) $5$-chain and (iii) $4$-star (a node connecting with the other three nodes).  



% \begin{table}[]
%     \centering
%       \caption{Empirical FDR averaged over $100$ repetitions in the detection of triangles.}
%     \begin{tabular}{c|ccc|ccc|ccc|ccc|}
%     \hline
%      &  \multicolumn{3}{c|}{$q=0.05$} & \multicolumn{3}{c|}{$q=0.1$} &  \multicolumn{3}{c|}{$q=0.05$} & \multicolumn{3}{c|}{$q=0.1$}  \\ \hline 
%      $n$ & $300$ & $400$ & $500$ &  $300$ & $400$ & $500$ & $300$ & $400$ & $500$ &  $300$ & $400$ & $500$  \\ \hline 
%      $d$ &  \multicolumn{6}{c|}{$p=40$} & \multicolumn{6}{c|}{$p=50$} \\ \hline
%      $200$ &  0.05 & 0.03 & 0.02 & 0.05 & 0.06 & 0.04  & 0.02 & 0.02 & 0.01 & 0.04 & 0.03 & 0.03\\
% $300$ & 0.03 & 0.05 & 0.05 & 0.06 & 0.09 & 0.08 & 0.04 & 0.05 & 0.05 & 0.08 & 0.09 & 0.08\\
% $400$ & 0.04 & 0.05 & 0.06 & 0.06 & 0.10 & 0.11 & 0.04 & 0.05 & 0.06 & 0.08 & 0.09 & 0.09\\ \hline
%     \end{tabular}
%     \label{tab:fdr1}
% \end{table}

% \begin{table}[]
%     \centering
%       \caption{Empirical power averaged over $100$ repetitions in the detection of triangles.}
%     \begin{tabular}{c|ccc|ccc|ccc|ccc|}
%     \hline
%      &  \multicolumn{3}{c|}{$q=0.05$} & \multicolumn{3}{c|}{$q=0.1$} &  \multicolumn{3}{c|}{$q=0.05$} & \multicolumn{3}{c|}{$q=0.1$}  \\ \hline 
%      $n$ & $300$ & $400$ & $500$ &  $300$ & $400$ & $500$ & $300$ & $400$ & $500$ &  $300$ & $400$ & $500$  \\ \hline 
%      $d$ &  \multicolumn{6}{c|}{$p=5$} & \multicolumn{6}{c|}{$p=10$} \\ \hline
%      $200$ &  0.69 & 0.92 & 0.98 & 0.79 & 0.95 & 0.99 & 0.76 & 0.96 & 0.99 & 0.84 & 0.98 & 0.99 \\
% $300$ & 0.27 & 0.65 & 0.86 & 0.36 & 0.72 & 0.90 & 0.51 & 0.80 & 0.97 & 0.62 & 0.88 & 0.98\\
% $400$ & 0.08 & 0.33 & 0.67 & 0.14 & 0.44 & 0.76 & 0.17 & 0.55 & 0.80 & 0.28 & 0.67 & 0.88\\ \hline
%     \end{tabular}
%     \label{tab:power1}
% \end{table}

% \newpage 
% \begin{table}[htbp]
%   \centering
%   \caption{Empirical FDR and power averaged over 200 repetitions}
%   %\scalebox{0.65}
%   {
%     \begin{tabular}{c|ccc|ccc|ccc|ccc}
%     \toprule
%           & \multicolumn{3}{c|}{q=0.05} & \multicolumn{3}{c|}{q=0.1} & \multicolumn{3}{c|}{q=0.05} & \multicolumn{3}{c}{q=0.1} \\
%     \midrule
%     $n$     & 300   & 400   & 500   & 300   & 400   & 500   & 300   & 400   & 500   & 300   & 400   & 500 \\
%     \midrule
%           & \multicolumn{6}{c|}{FDP}                      & \multicolumn{6}{c}{Power} \\
%     \midrule
%     $d$     & \multicolumn{12}{c}{(i) Triangle} \\
%     $d_1$    & 0.041 & 0.043 & 0.023 & 0.052 & 0.053 & 0.030 & 0.999 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
%     $d_2$    & 0.038 & 0.038 & 0.027 & 0.048 & 0.049 & 0.035 & 0.999 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
%     $d_3$    & 0.046 & 0.043 & 0.039 & 0.057 & 0.052 & 0.0488 & 0.999 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
%     \midrule
%     $d$     & \multicolumn{12}{c}{(ii) Four-cycle} \\
%     $d_1$    & 0.015 & 0.016 & 0.008 & 0.020 & 0.019 & 0.010 & 0.997 & 0.999 & 1.000 & 0.997 & 1.000 & 1.000 \\
%     $d_2$    & 0.015 & 0.013 & 0.008 & 0.019 & 0.019 & 0.011 & 0.995 & 0.999 & 1.000 & 0.996 & 0.999 & 1.000 \\
%     $d_3$    & 0.015 & 0.011 & 0.012 & 0.017 & 0.016 & 0.016 & 0.994 & 0.999 & 1.000 & 0.995 & 1.000 & 1.000 \\
%     \midrule
%     $d$     & \multicolumn{12}{c}{(iii) Five-cycle} \\
%     $d_1$    & 0.004 & 0.002 & 0.002 & 0.006 & 0.003 & 0.003 & 0.976 & 0.999 & 1.000 & 0.978 & 0.999 & 1.000 \\
%     $d_2$    & 0.004 & 0.003 & 0.002 & 0.004 & 0.003 & 0.002 & 0.970 & 0.998 & 1.000 & 0.975 & 0.998 & 1.000 \\
%     $d_3$    & 0.002 & 0.003 & 0.002 & 0.003 & 0.004 & 0.002 & 0.962 & 0.998 & 1.000 & 0.968 & 0.998 & 1.000 \\
%     \bottomrule
%     \end{tabular}%
%     }
%  \label{tab:addlabel}%
% \end{table}%
% \begin{table}[htbp]
%   \centering
%   \caption{Empirical FDR and power averaged over 200 repetitions}
%   %\scalebox{0.65}
%   {
%     \begin{tabular}{c|ccc|ccc|ccc|ccc}
%     \toprule
%           & \multicolumn{3}{c|}{q=0.05} & \multicolumn{3}{c|}{q=0.1} & \multicolumn{3}{c|}{q=0.05} & \multicolumn{3}{c}{q=0.1} \\
%     \midrule
%     $n$     & 300   & 400   & 500   & 300   & 400   & 500   & 300   & 400   & 500   & 300   & 400   & 500 \\
%     \midrule
%           & \multicolumn{6}{c|}{FDP}                      & \multicolumn{6}{c}{Power} \\
%     \midrule
%     $d$     & \multicolumn{12}{c}{(i) Triangle} \\
%     $d_1$    & 0.0412 & 0.0431 & 0.0233 & 0.0522 & 0.0533 & 0.0296 & 0.9999 & 1.0000 & 1.0000 & 0.9999 & 1.0000 & 1.0000 \\
%     $d_2$    & 0.0387 & 0.0383 & 0.0272 & 0.0476 & 0.0489 & 0.0351 & 0.9997 & 1.0000 & 1.0000 & 0.9999 & 1.0000 & 1.0000 \\
%     $d_3$    & 0.0464 & 0.0429 & 0.0395 & 0.0569 & 0.0522 & 0.0488 & 0.9997 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
%     \midrule
%     $d$     & \multicolumn{12}{c}{(ii) Four-cycle} \\
%     $d_1$    & 0.0154 & 0.0157 & 0.0075 & 0.0202 & 0.0198 & 0.0099 & 0.9970 & 0.9999 & 1.0000 & 0.9972 & 1.0000 & 1.0000 \\
%     $d_2$    & 0.0154 & 0.0127 & 0.0083 & 0.0194 & 0.0188 & 0.0109 & 0.9955 & 0.9999 & 1.0000 & 0.9965 & 0.9999 & 1.0000 \\
%     $d_3$    & 0.0148 & 0.0112 & 0.0120 & 0.0175 & 0.0159 & 0.0156 & 0.9941 & 0.9999 & 1.0000 & 0.9949 & 1.0000 & 1.0000 \\
%     \midrule
%     $d$     & \multicolumn{12}{c}{(iii) Five-cycle} \\
%     $d_1$    & 0.0045 & 0.0018 & 0.0022 & 0.0063 & 0.0027 & 0.0027 & 0.9759 & 0.9992 & 1.0000 & 0.9784 & 0.9992 & 1.0000 \\
%     $d_2$    & 0.0040 & 0.0027 & 0.0018 & 0.0039 & 0.0032 & 0.0018 & 0.9704 & 0.9984 & 1.0000 & 0.9749 & 0.9984 & 1.0000 \\
%     $d_3$    & 0.0025 & 0.0032 & 0.0018 & 0.0029 & 0.0036 & 0.0023 & 0.9618 & 0.9976 & 1.0000 & 0.9676 & 0.9979 & 1.0000 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel}%
% \end{table}%

 	
%%% Local Variables:
%%% TeX-master: "atlas"
%%% End:


==> app_omit_GGMISING.tex <==

  \section{Theoretical Results for Gaussian Graphical Model and Ising Model }\label{sec:application}
%  \subsection{Theoretical guarantee for subgraphs selection under  GGM}
  


In this section, we present the theoretical results of applying our general inferential framework to select general subgraphs on two class of  models: Gaussian graphical models and high-temperature Ising models.    

\subsection{Subgraph selection on Gaussian graphical models}\label{sec:example:GGM}
% In the Gaussian graphical model introduced in Section \ref{sec:method},
% we have $W^*_{uv}=0$ if and only if $(u,v) \notin E^*$ where $ W^*_{uv}=\Theta^*_{uv}$. 
% We consider the following parameter space for the precision matrices
% \begin{equation}\label{eqn:us}
% \mathcal{U}(s)=\Big\{\Theta^* \in \mathbb{R}^{d \times d} \mid 1/\rho \leq \lambda(\Theta^*) \leq \rho, 
% \max_{j \in[d]} \|\Theta^*_{\cdot j}\|_{0} \leq s,\|\Theta^*\|_{1} \leq M \Big\},
% \end{equation} 
% {\blue where $\Theta^*_{\cdot j}$ refers to the $j$-th column vector of matrix $\Theta^*$. }
%  \eqref{eqn:us} requires $\Theta^*$ has at most $s$ non-zero entries per column, and therefore the induced graph have maximum degree at most $s$.
% %
% Also, we assume $1/\rho \leq \lambda(\Theta^*) \leq \rho$, which  means that $\lambda_{\min }(\Theta^*) \geq 1 / \rho$ and $\lambda_{\max }(\Theta^*) \leq \rho$, i.e., the minimum and maximum eigenvalues of $\Theta^*$ are  bounded by $1/\rho$ and $\rho$.
% %
% So the parameter space $\mathcal{U}(s)$
% restricts our precision matrix $\Theta^*$ to well-conditioned matrices.

% Subsequently, we delve into the estimation of edge weights within the context of the Gaussian graphical model, followed by the verification of sparsity and dependence conditions, and finally the presentation of theoretical results for the Gaussian graphical model.



% \paragraph{Estimation}   
% First, in the setup of Gaussian graphical model, we need an appropriate estimator of the precision matrix $\Theta^*$, based on $n$ i.i.d. observations $\bX_1, \ldots, \bX_n$ following the distribution of $\bX$. % Let $\boldsymbol{X}=(\bX_{1}, \ldots, \bX_{n})^\top$
% There is already significant work in literature to achieve  inverse covariance estimation. 
% We can 
% consider the unbiased estimator $\hat\Theta^{\mathrm{d}}=\{\widehat{\Theta}_{uv}^{\mathrm{d}}\}_{(u,v) \in \bar E}$ in (S.34) of \cite{lu2017adaptive},
% \begin{equation}
% \widehat{\Theta}_{uv}^{\mathrm{d}}=\widehat{\Theta}_{uv}-\frac{\widehat{\Theta}_{\cdot u}^{\top}\big(\widehat{\Sigma} \widehat{\Theta}_{\cdot v}-\mathbf{e}_{v}\big)}{\widehat{\Theta}_{\cdot u}^{\top} \widehat{\Sigma}_{\cdot u}},
% \end{equation}
% where $\widehat{\Sigma}=1/n \sum_{i=1}^n \bX_i\bX_i^\top$ is the sample covariance matrix, $\widehat{\Theta}_{\cdot j}, \widehat{\Sigma}_{\cdot j}$ is the $j$-th column of matrix $\widehat{\Theta}, \widehat{\Sigma}$ respectively, and $\mathbf{e}_{k} \in \RR^d$ is the $k$-th natural basis with only the $k$-th entry being 1. Here $\widehat{\Theta}_{uv}$ is estimator of  $\Theta^*_{uv}$, which can come from  the graphical lasso estimator  \citep{friedman2008sparse} or the method of constrained $\ell_1$-minimization for inverse matrix estimation (CLIME) \citep{cai2011constrained}.

% If $\hat{\Theta}$ satisfies (3.3) and (3.4) in \cite{neykov2019combinatorial}, $\hat\Theta^\mathrm{d}_{uv}$ can be decomposed into:
% \begin{equation}\label{eqn:decomp}
%  \sqrt{n} \widehat{\Theta}^\mathrm{d}_{uv}=n^{-1 / 2} \sum_{i=1}^{n}\big(\Theta_{\cdot j}^{* \top} \bX_i\bX_i^\top \Theta^*_{\cdot v}-\Theta^*_{uv}\big)+o_{P}(1)  
% \end{equation}
% which is asymptotically normal distributed that  $\sqrt{n}\big(\widehat{\Theta}_{uv}^{\mathrm{d}}- \Theta^*_{uv}\big) \rightsquigarrow N\big(0, \Theta^*_{uu}\Theta^*_{vv}+\Theta^{*^2}_{uv}\big)$. 

We introduced the Gaussian graphical model in Section \ref{GS:sec:GGM}.
Recall that  $ W_{uv}^*=  {\Theta}^*_{uv} $, 
  we propose the following $\hat{W}_{uv}$  and  $W_{uv}$ for the Gaussian graphical model: for any edge $(u,v)\in E$,
\begin{equation}\label{eq:That:GGM}  
  \hat{W}_{uv}= \widehat{\Theta}_{uv}^{\mathrm{d}},\qquad W_{uv}=\frac{1}{n }\sum_{i=1}^n\Theta^*_{u\cdot}\bX_i\bX_i^\top\Theta^*_{\cdot v}.
  \end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We have the following theoretical guarantee. The proof of this proposition is deferred to   Section \ref{sec:pflem:GGM}.
\begin{restatable}[]{prop}{lemGGM}\label{lem:GGM} 
For GGM with parameter space $\Theta \in {\cal U}(s)$ defined in \eqref{eqn:us}, suppose $s^2\log^4(dn)/n=o(1)$ hold, the estimator $\hat{W}$ defined in \eqref{eq:That:GGM} for the GGM satisfies 
% with probability at least $1-o(1/\log d)$ for all $j\in {\cal H}_0$, $e_j\in N_j$ with $| N_j|\leq C$, we have 
\[
\mathbb{P}\Bigl( \sup_{e\in \bar E}\big|\hat{W}_e-W_e-W^*_e\big|/\sigma_e\leq\frac{C}{\sqrt{n\log d}},
\ 
\sup_{e\in \bar E}\big|\sigma_e/\hat{\sigma}_e-1\big|\leq \frac{C}{\log d}\Bigr)=1-o(1),
\]
where {   $\sigma_{uv}=\sqrt{\Theta^*_{uu}\Theta^*_{vv} + (\Theta^*_{uv})^2}$ and $\hat \sigma_{uv}=\sqrt{\widehat{\Theta}_{uu}^{\mathrm{d}} \widehat{\Theta}_{vv}^{\mathrm{d}}  + (\widehat{\Theta}_{uv}^{\mathrm{d}} )^2 }$ for $(u,v) \in \bar E$. }
\end{restatable}



%Moreover, it is obvious that  $\sqrt{n}W^*(\cdot)$ defined in (\ref{eq:That:GGM}) satisfies Scenario $(a)$ in (\ref{con:Tstar}). 

     \paragraph{Assumptions}
Next we check that the sparsity and dependence conditions in Assumption  \ref{ass:spadepend} also hold under the Gaussian graphical model with $\Theta \in {\cal U}(s)$. In fact, under the notation system of Gaussian graphical models, we can determine that
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{small}
\begin{align}
\begin{split}\label{eq:NHS:GGM}
S\big(\{e_{j}\}_{j \in \cH_0}\big)=
\Big\{
 (e_{j_1},e_{j_2}): j_1\neq j_2,(u,v)=e_{j_1},(u',v')=e_{j_2},  \frac{|\Theta^*_{uu'}\Theta^*_{vv'}+\Theta^*_{uv'}\Theta^*_{u'v}|}{\sqrt{\Theta^*_{uu}\Theta^*_{u'u'}\Theta^*_{vv}\Theta^*_{v'v'}}}  \geq
 \blue
 \frac{C}{(\log d)^{2} (\log\log d)} \Big\}.
\end{split}
\end{align} 
\end{small}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following proposition tells us that given the constraint in $S$, the maximum possible cardinality of $S$ can be reduce from $O(|{\cal H}_0|^2)$ to  $O(|{\cal H}_0|d^{M-2}s^2)$, where we recall that $M=\max_j|V(F_j)|$.
% \begin{proposition}\label{prop:GGM}   
% For Gaussian graphical models with $\Theta \in {\cal U}(s)$ where the maximum degree of the graph $G^*$  is $s$.  We have  $S=O(|{\cal H}_0|d^{M-2}s^2)$.
% %,  and $\frac{\rho |{\cal H}_0|^2 }{ \log d} =O(\frac{d^{2m}}{\log d})$.
% \end{proposition}
% %The proof of this proposition is deferred to Section \ref{sec:pfprop:GGM} in the appendix.

%  So by  Proposition
% \ref{prop:GGM}, if $|{\cal H}_0|\asymp |{\cal H}_0| + |{\cal H}_1|\asymp d^M$, dependence condition in Assumption \ref{ass:spadepend} for GGM can be implied by
% $$
% \frac{d^{M-2}s^2}{|\widetilde{{\cal H}}_1|}=o\Big(\frac{1}{\log d}\Big) \text{ or equivalently } 
% |\widetilde{{\cal H}}_1| = \omega(s^2 d^{M-2} \log d).
% $$
% The proof is deferred to Section \ref{sec:pfprop:GGM}.

\paragraph{Theoretical results}

We have the following corollary for the statistical guarantee of the performance of Algorithm \ref{alg:1} under the Gaussian graphical model above. The  proof is postponed to Section~\ref{sec:cor:FDRPOW:GGM}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\begin{restatable}[FDR and power guarantee under GGM]{corollary}{corFDRPOWGGM}\label{cor:FDRPOW:GGM} Under the same conditions of Proposition \ref{lem:GGM}.
Suppose $\log d/\log n=O(1)$,
then under Assumption \ref{ass:spadepend} with $S$ defined in \eqref{eq:NHS:GGM}, we have
\[
\mathrm{FDP}\leq q\frac{|{\cal H}_0|}{J}+o_{P}(1),\qquad \mathrm{FDR}\leq q\frac{|{\cal H}_0|}{J}+o(1),
\]
 and we have uniform power control %where $|{\cal H}_0|=|{\cal H}_0|$ and $J=|{\cal H}_0|+|{\cal H}_1|$,
\begin{equation*}
\mathbb{P}\big(\psi_j=1,\text{ for all }j\in \widetilde{{\cal H}}_1\big) = 1 -  o(1).
\end{equation*}   

\end{restatable}


% Next we consider a high-temperature Ising model and propose the corresponding test statistic.


% if this does not cause confusion
% \paragraph{Maximum Quantile Approximation}
% Second, we approximate the null distribution of the maximum statistic 
% \begin{equation}\label{eqn:TE-GGM}
% T_{E}=\sqrt{n}\max_{(u,v) \in E}
% \Big|
% \widetilde{\Theta}_{uv}
% -
% {\Theta}_{uv}^* 
% \Big|.    
% \end{equation}
% Let $\hat c (\alpha, E)$ denote the estimator for $(1-\alpha)$-quantile of the statistic $T_{E}$ by Gaussian multiplier bootstrap in  \citep{Chernozhukov2013Gaussian}. 
% We also denote
% $ {\hat c}^{-1}(\tau, E) $
% as an estimator for $\mathbb{P}\big(T_{E} > \tau\big).$ The details on $\hat c (\alpha, E)$ can be found in Section 5 of \cite{lu2017adaptive}. 

% \begin{lemma}\label{lem:GMB-GGM}
% For Gaussian graphical models, suppose $\Theta \in \mathcal{U}(s)$ and $(\log (d n))^{7} / n+s^{2}(\log d n)^{4} / n=o(1)$. We obtain $\hat c(\alpha, E)$ from (2.4) in \cite{zhang2021startrek}. Then for any edge set $E \subseteq E$, we have
% $$
% \lim_{(n, d) \rightarrow \infty} \sup _{\boldsymbol{\Theta} \in \mathcal{U}(s)} \sup _{\alpha \in(0,1)}\Big|\mathbb{P}\Big(\max_{(u,v) \in E} \sqrt{n}
% \Big|
% \widetilde{\Theta}_{uv}
% -
% {\Theta}_{uv}^* 
% \Big|
% >\widehat{c}(\alpha, E)\Big)-\alpha\Big|=0.
% $$

% \end{lemma}


% To be specific, motivat ed by the decomposition in \eqref{eqn:decomp}, we construct the following Gaussian multiplier bootstrap statistic  \citep{Chernozhukov2013Gaussian}:
% \begin{equation}\label{eqn:bootstrap stat}
%     T_{E}^{\mathcal{B}}=\max _{(j, k) \in E} \frac{1}{\sqrt{n \widehat{\Theta}_{uu} \widehat{\Theta}_{vv}}}\bigg|\sum_{i=1}^{n} \widehat{\Theta}_{\cdot j}^{\top}\bigl(\bX_{i} \bX_{i}^{\top} \widehat{\Theta}_{\cdot v}-\mathbf{e}_{k}\bigr) \xi_{i}\bigg|,    
% \end{equation}
% where $\xi_{i} \sim N(0,1), i \in[n]$ are independent and identically distributed.   
% Let $\hat c (\alpha, E)$ denote the $(1-\alpha)$-quantile of the statistic $T_{E}^{\mathcal{B}}$ (conditioning on the data $\bX: \bX_1, ..., \bX_n$). Formally, we define
% \begin{equation}\label{eqn:chat}
%  \hat c(\alpha, E)=\inf _{t \in \mathbb{R}}\Big\{t \biggiven \mathbb{P}\big(T_{E}^{\mathcal{B}} \leq t \biggiven \bX \big) \geq 1-\alpha\Big\}   
% \end{equation}
% as an estimator for $(1-\alpha)$-quantile of $T_E$.
% We also define the inverse function
% \begin{equation}\label{eqn:chat-1}
%  {\hat c}^{-1}(\tau, E) =  1-\mathbb{P}\big(T_{E}^{\mathcal{B}} \leq \tau \biggiven \bX \big).
% \end{equation}




 
 

%%%% Yue Sept 16


% \paragraph{Skip-down with BHq procedure}
% For our multiple testing problem where we aim to select all subgraphs, we can consider conducting each single test by the skip-down procedure proposed by \cite{lu2017adaptive}, which was a general framework for testing monotone graph properties, such as connectivity or the maximum degree.
% The single test procedure is presented below in Algorithm \ref{alg:1}, which
% takes standardized estimator $\widetilde{\Theta}^{\d}$ as input.
% \begin{algorithm}[htbp]
%     \caption{Skip-down algorithm for testing the $j$-th subgraph \label{alg:1}}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$\widetilde{{\Theta}}$,   significance level $\alpha$. }
%     Initialize {$t=0,\, E_{0,j}= \big\{(j_1, j_2)\in V_j \times V_j: j_1\neq j_2\big\}$, and $E_{0,j}^c=\emptyset.$} 
%     % \{(j_1, j_2)\in V_j \times V_j:j_1\neq j_2\}$}. %\{(j_1, j_2): \text{all edges between the $j$-th set of nodes $V_j$}\}$.
   
%     \Repeat{${G_j \subseteq  (V_j,E_{t,j}^{c}) } \mbox{ or } \mathcal{R}=\varnothing$}
%     { 
%     $t \leftarrow t+1$\;
    
%     The rejected edge set $\mathcal{R} \leftarrow\Bigl\{e \in E_{t-1,j}:\,\sqrt{n}\big| \widetilde{{\Theta}}_{e}\big|>\chat(\alpha, E_{t-1,j})\Bigr\}$\;
    
%     $E_{t,j} \leftarrow E_{t-1,j} \setminus \mathcal{R}$ and  $E_{t,j}^c \leftarrow E_{t-1,j}^c \cup \mathcal{R}$\;
%     }
%   	\Output{$\psi_{j, \alpha}=1$ if $G_j  \subseteq (V_j,E_{t,j}^{c}) $, $\psi_{j, \alpha}=0$ otherwise.}%$G^* \subseteq E_{t,j}^{c}$, $\psi_{j, \alpha}=0$ otherwise.}
% \end{algorithm}

% \begin{figure}[h!]
% 	\begin{center}
% 		\begin{tabular}{cc}
% 		&{(A) the complete graph \   (B) $t=0$ \quad\quad\quad\quad  (C) $t=1$ \quad\quad\quad\quad  (D) $t=2$ \quad\quad\quad\quad\quad\quad\ \ \ \ \ \ \ \ \ \ \ \   }\\
% 		&\includegraphics[width=0.99\textwidth,angle=0]{./figure/alg1} \\
% 			[-10pt]
% 		\end{tabular}
% 	\end{center}
% 	\caption{Illustration of Algorithm \ref{alg:1}. Suppose we have a graph with six nodes and we aim to select all triangles. (A) is the complete graph with six nodes and thus 15 possible triangles. As an example, we only focus on  the green triangle in (B). When $t=0$, $E_{0,j}$ is the set of the three green edges. In (C), when $t=1$, we reject one edge (the red one). In (D), when $t=2$, we reject another red edge. Then in the next iteration, we reject nothing. So the algorithm ends here and we only reject two edges. So in this example, we can not reject the null hypothesis in \eqref{eqn:hypo}.}
% 	\label{fig:alg1}
% \end{figure}

% To conduct the subgraph selection (i.e., multiple testing), we need to determine an appropriate threshold $\alpha$ in Algorithm \ref{alg:1} in order to control FDR at a pre-determined level $q$ (e.g., 0.05), and we reject $H_{0j}$ if $\psi_{j, \alpha}=1$. 
% We consider Benjamini and Hochberg (BHq) procedure \citep{benjamini1995controlling}, so $\alpha$ in Algorithm \ref{alg:1} is chosen as 
% \begin{equation}\label{eqn:alphahat}
% \widehat{\alpha}=\sup \Bigl\{\alpha \in(0,1): \frac{\alpha J}{\max \Bigl\{1, \sum_{j \in [J]} \psi_{j, \alpha}\Bigr\}} \leq q\Bigr\},
% \end{equation}where $J$ is the total number of hypotheses. Normally, if the subgraph involves $m$ nodes, then $J=\binom{d}{m}$.
   
   
   


\subsection{Subgraph selection on   Ising models}\label{sec:example:Ising}

% \exising*

% \begin{example}[Ferromagentic Ising Model]\label{ex:ising}
% In the Ising model,  $\bX \in \{1,-1\}^{d}$ for each node has distribution
% \begin{equation}\label{eqn:Ising}
% \mathbb{P}(\bX = \mathbf{x}) = \frac{1}{Z(\mathbf{w}^*)} \exp \Big( \sum_{(u, v) \in E} w^*_{u v} x_{u} x_{v}\Big),
% \end{equation} 
% where $\mathbf{x} = (x_{1}, \cdots, x_{d})^\top$ is an observation of $\bX$, $\mathbf{w}^* = \{w^*_{u v}\}_{(u, v) \in E}$ is the weights on the edges, and $$Z(\mathbf{w}^*) = \sum_{\mathbf{x} \in \{1,-1\}^{d}} \exp \Big( \sum_{(u, v) \in E} w^*_{u v} x_{u} x_{v}\Big)$$ is the partition function (i.e., the normalizing constant), which ensures the distribution in \eqref{eqn:Ising} sums to $1$. We have $w^*_e > 0$ if and only if $e \in E^*$, $w^*_e=0$ for $e \notin E^*$.
% Following the literature \cite{neykov2019property}, we assume there is a known lower bound $\theta$ for $w^*_e, e\in E^*$.
% % 
% In practice, estimating the weight $w^*_{uv}$ in the Ising model \eqref{eqn:Ising0} is not easy. 
% % 
% However, Lemma 3.1 in \cite{neykov2019property} shows that  the correlation between variables can be used to characterize the edge weight. Specifically,  $\E[X_uX_v]- \tanh \theta >0$ if and only if $w^*_{uv} >0$. Moreover,  correlation $\E[X_uX_v]$ is easier to estimate than $w^*_{uv}$.
%  So we 
We introduced the Ising model in Section \ref{GS:sec:Ising}.
Recall that we focus on studying  the weight  \begin{equation}
     W^*_{uv}=\mathbb{E}[X_uX_v]-\tanh(\theta), 
 \end{equation} 
%
% In the Ising model introduced in Example \ref{ex:ising}, $\bX=(X_{1}, X_{2}, \ldots X_{d})^{\top} \in \{1,-1\}^{d}$ follows distribution in \eqref{eqn:Ising0}.
% We have $w^*_e > 0$ if and only if $e \in E^*$, and $w^*_e=0$ for $e \notin E^*$. 
% 
% We consider the following parameter space
% \begin{equation}\label{model:Ising:para}
% \mathcal{W}=\Big\{w^*: 
%     \min_{e\in E^*}w^*_e\geq \theta,\|w^*\|_\infty \leq \Theta, s \tanh(\Theta)<\rho,s\geq 2\rho/(1-\rho)\Big\}, 
% \end{equation}% \min_{e\in E^*}w^*_e\geq \theta,\|w^*\|_\infty \leq \Theta, \rho\tanh (\Theta)\leq \tanh(\theta)\leq C/\log d,s \tanh(\Theta)<\rho^2/(1+\rho^2)\Big\}, 
% where $\rho \in (0,1)$ is a constant.
% This consider a high-temperature Ising model, note that \cite{neykov2019property} has proved that the testing of cycles is statistically possible if and only if $\theta =\Omega(\sqrt{\log d/n})$. In practice, the testing  under high-temperature Ising model is harder than that under low-temperature model since the former usually suffers for extremely weak and sparse signals. This suggests the superiority of our framework that it is even able to solve hard statistical testing problems with FDR controls. Below, we start by how to construct the test statistic.
and to estimate the edge weight, we use $\hat{W}$ and $W$ for the Ising model as follows: for any $\blue (u,v) \in \bar E$,\begin{equation}\label{eq:That:Ising}
   \hat{W}_{uv}=\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv}  - \tanh(\theta),\ W_{uv}=\frac{1}{n}\sum_{i=1}^{n} X_{iu} X_{iv}-\mathbb{E}[X_uX_v].
\end{equation}
{We also have
$\hat \sigma_{uv} = \sqrt{1-\big(\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv} \big)^2}$
and $\sigma_{uv} = \sqrt{1-(\EE X_{iu} X_{iv})^2}$. }

We have the following theoretical guarantee for asymptotic normality of $\hat W_{uv}$.  The proof of this proposition can be found in Section~\ref{sec:pflem:Ising}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Denote $m=\max\{|\mathbb{E}[X_uX_v]|^2:(u,v)\in E(F_j),j\in \widetilde{{\cal  H}}_1\}$, $m_0=\max \{|\mathbb{E}[X_uX_v]|^2:(u,v)\in N_j,j\in {\cal H}_0\}$ 
\begin{restatable}[]{prop}{lemIsing}\label{lem:Ising}  Under Ising models \eqref{eqn:Ising0} with parameter space \eqref{model:Ising:para}, the estimator $\hat{W}$ defined in \eqref{eq:That:Ising} for the Ising model satisfies 
\[
\mathbb{P}\Bigl( \sup_{e\in \bar E}\big|\hat{W}_e-W_e-W^*_e\big|/\sigma_e\leq\frac{C}{\sqrt{n\log d}},\ 
\sup_{e\in \bar E}\big|\sigma_e/\hat{\sigma}_e-1\big|\leq \frac{C}{\log d}\Bigr)=1-o(1).
\]

 \end{restatable}


% {  
% \[
%  \sqrt{n}\frac{\widehat{\Theta}_{uv}^{\mathrm{d}}-\mu}{\sqrt{\widehat{\Theta}_{uv}^{\mathrm{d}}\widehat{\Theta}_{vv}^{\mathrm{d}}}},\qquad \frac{\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv}  - \tanh(\theta)-\mu}{\sqrt{1-(\frac{1}{n}\sum_{i=1}^{n}  X_{iu} X_{iv})^2}}
% \]

% \[
% \mathbb{P}\Bigl( \sup_{e\in E}\big|\hat{W}_e-W_e-W^*_e\big|/\sigma_e>\frac{C}{\sqrt{n\log d}}\Bigr)=o(1),\qquad \mathbb{P}(\sup_{e\in E}\big|\hat{\sigma}_e-\sigma_e\big|>C/\log d)
% \]

% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Assumptions}
For Ising models, following the notations from Section \ref{sec:example:Ising},  we have
\begin{align}
\begin{split}\label{eq:NHS:Ising}
\blue
   S(\{e_j\}_{j\in {\cal H}_0})=\Big\{
    (e_{j_1},e_{j_2}): j_1\neq j_2,(u,v)=e_{j_1},(u',v')=e_{j_2},  \Cov(X_uX_v,X_{u'}X_{v'}) \geq \frac{C}{(\log d)^{2} (\log\log d)} \Big\}.
\end{split}
\end{align}
% Assumption \ref{ass:spadepend} is difficult to verify under the general graph structure of Ising models. However, Proposition \ref{prop:Ising} states that a similar conclusion to Proposition \ref{prop:GGM} holds for a graph with a tree structure. 
% % This suggests that Assumption \ref{ass:spadepend} may be feasible for the general graph structure of Ising models. 
% The proof of Proposition \ref{prop:Ising} is presented in  Section \ref{sec:pfprop:Ising}.

% \begin{proposition}\label{prop:Ising}
% For Ising models, assume that the graph with $d$ nodes consists of $d/s$ trees and each tree has $s$ nodes. We have  $S=O(|{\cal H}_0|d^{M-1}s)$.
% %,  and $\frac{\rho |{\cal H}_0|^2 }{ \log d} =O(\frac{d^{2m}}{\log d})$.
% \end{proposition}
%   %%%%%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%%%
%       %%%%%%%%%%%%%%%%%%%%%%%%%%
% Thus, if $|{\cal H}_0|\asymp |{\cal H}_0| + |{\cal H}_1|$, dependence condition in Assumption \ref{ass:spadepend} for the Ising model can be implied by
% $$
% \frac{d^{M-1}s}{|\widetilde{{\cal H}}_1|}=o\Big(\frac{1}{\log d}\Big) \text{ or equivalently } 
% |\widetilde{{\cal H}}_1| = \omega(s d^{M-1} \log d).
% $$



%{  Similar to GGM, when XXX, this will hold.}

\paragraph{Theoretical results}

Similar to the analysis of Gaussian graphical model in Section \ref{sec:example:GGM}, under Ising models, we also  have the following corollary for the theoretical guarantee of the performance of Algorithm \ref{alg:1}. The proof  is deferred to Section \ref{sec:pfcor:FDRPOW:Ising}.

\begin{restatable}[FDR and power guarantee under Ising models]{corollary}{corFDRPOWIsing}\label{cor:FDRPOW:Ising} 
Assume the same conditions as in Lemma \ref{lem:Ising}, and $\log d/\log n=O(1)$.
Under Assumption \ref{ass:spadepend} with $S$ defined in \eqref{eq:NHS:Ising}, we have
\[
\mathrm{FDP}\leq q\frac{|{\cal H}_0|}{J}+o_{P}(1),\qquad \mathrm{FDR}\leq q\frac{|{\cal H}_0|}{J}+o(1),
\]
where  $J=|{\cal H}_0|+|{\cal H}_1|$, and we have uniform power control
\begin{equation*}
\mathbb{P}\big(\psi_j=1,\text{ for all }j\in \widetilde{{\cal H}}_1\big) = 1- o(1).
\end{equation*}   
\end{restatable}




% Next we illustrate condition \eqref{eqn:depend} using a simple example. Assuming our graph is Figure {   ????} with $d$ nodes and some triangles, and we aim to select all triangles. As in the figure, $\big(\{k_1,\ell_1\}, \{k_2,\ell_2\} \big)$ is counted in $S$. Since we have $d$ nodes, we have at most $d$ possible choice of $k_1$ and $d$ possible choice of $\ell_1$. 
% Also, edge $(k_1,\ell_1)$ can be in other sets $N_{j}, j \neq j_1$ in addition to $N_{j_1}$. For selecting triangles, $(k_1,\ell_1)$ can be in at most $d$ different $N_{j}$ since we only have freedom of choosing the third nodes. 
% For edge $(k_2,\ell_2)$, we observe $k_2$ should be the same node as $k_1$ and $\ell_2$ should be one node of triangle $\Delta_1$ so that $\big(\{k_1,\ell_1\}, \{k_2,\ell_2\} \big)$ satisfies the condition in \eqref{eqn:S} and is counted in $S$. Thus, $S$ is at most of the order of $d^4$. On the other hand,  if $|{\cal H}_0|$ and $J$ are  of the order of $d^3$,   Condition \eqref{eqn:depend} requires $d =o(\frac{|\widetilde{{\cal H}}_1|}{ \log d})$.



% In general, assume that the maximum degree of graph is at most $s$, and the subgraph of interest $F$ has $m=|V(F)|$ nodes.  Following the similar argument as above,  we have $S$ is at most of the order of $d^2s^2(\binom{d}{m-2})^2$ or simply $d^{2m-2}s^2$,  and $\frac{\rho |{\cal H}_0|^2 }{ \log d} $ is at most of the order of $\frac{d^{2m}}{\log d}$.

% Condition \eqref{eqn:depend} requires $d =o(\frac{|\widetilde{{\cal H}}_1|}{ \log d})$.

% Also $|\cH_0|$ is the number of true null hypotheses. If the graph is too connected (where $|\cH_0|$ is typically small) then the multiple testing problem is harder.
% For example, if $J$ and $|\cH_0|$ are at the order of $d^m$, then \eqref{eqn:depend} holds when 
% $|S| = o \Big( \frac{\rho |{\cal H}_0|^2 }{ \log d}  \Big). $




% {  
% \begin{assumption}\label{ass:signal}
% We assume the following condition hold:
% \begin{equation}\label{eqn:scaling}
% \frac{ J\log d }{|\widetilde{{\cal H}}_1|} \cdot \bigg( \frac{(\log d)^{19 / 6}}{n^{1 / 6}} + \frac{(\log d)^{11 / 6}J^{1/3}}{n^{1 / 6} |\widetilde{{\cal H}}_1|^{1 / 3}} + s\frac{(\log d)^{3} }{\sqrt{n}} + \frac{J}{d^{   m+1} |\widetilde{{\cal H}}_1|} +  \frac{1}{|{\cal H}_0|} \bigg)=o(1),    
% \end{equation} 
% \begin{equation}\label{eqn:depend}
% \frac{ J\log d }{|\widetilde{{\cal H}}_1|} \cdot  \frac{1}{|{\cal H}_0|^2} |S| = o(1).    
% \end{equation}
% \end{assumption}
  


% Recall that $\cH_0=\bigl\{1\leq j \leq J \biggiven  F_j \not\subseteq G^* \bigr\}$ is the set of true null hypotheses, and   $\cH_1=\bigl\{1\leq j \leq J \biggiven  F_j \subseteq G^* \bigr\}$ is the set of true alternative hypotheses.
% And \begin{equation}\label{eqn:tilde H_1}
% \tilde{\mathcal{H}}_{1}=\Bigl\{j \in \mathcal{H}_{1}: \forall (u,v) \in N_{j}^c \text{ with } u \neq v,\bigl|\Theta^*_{uv}^*\bigr|> C_0 \sqrt{\log d / n}\Bigr\} \subseteq \cH_1
% \end{equation}
% is a subset of $\cH_1$, containing true alternative hypotheses where the all edges of these subgraphs have signal strength  exceeding $\sqrt{\log d/n}$.

% $S$ is a measure of dependence defined as 
% \begin{equation}\label{eqn:S}  
% S= \bigcup_{j_{1}, j_{2} \in \mathcal{H}_{0}, j_{1} \neq j_{2}} \Big\{\big( \{k_1,\ell_1\} , \{k_2,\ell_2\} \big): (k_1,\ell_1) \in N_{j_{1}}, (k_2,\ell_2) \in N_{j_{2}},  \Theta^*_{k_1k_2}   \Theta^*_{\ell_1\ell_2}+\Theta^*_{k_1\ell_2} \Theta^*_{k_2\ell_1} \neq 0 \Big\},     
% \end{equation}
% with
% $
% N_{j}=\Bigl\{e\in V(F_j) \times V(F_j): \Theta^*_{e}^*=0\Bigr\}$ and  $N_{j}^{c}=\Bigl\{(u,v)\in V(F_j) \times V(F_j): u \neq v, \bigl|\Theta^*_{uv}^*\bigr|>0\bigr\}$.




%  Condition \eqref{eqn:scaling} is the scaling condition required for validity of maximum quantile estimation by Gaussian bootstrap procedure.
% See detailed discussions in \cite{zhang2021startrek}. Note that $\tilde \cH_1$ is defined in \eqref{eqn:tilde H_1}.  Here we do not need signal strength for all true subgraphs. For example, let $J=\binom{d}{m}$ and $|\cH_0|$ both be at the order of $O(d^m)$,
% we require
% \begin{equation}   
% |\widetilde{{\cal H}}_1| = W^* \bigg(  
%  \frac{d^m (\log d)^{25 / 6}}{n^{1 / 6}} + {\frac{d^{m} (\log d)^{17 / 8}}{n^{1 / 8} }} + 
%  s\frac{d^m (\log d)^{4} }{\sqrt{n}} + 
%   d^{(m-1)/2}\sqrt{\log d} + \log d \bigg) 
% \end{equation} 
% for  \eqref{eqn:scaling}  to hold.

% $$   \rho $$ 


% Condition \eqref{eqn:depend} is the dependence condition.
% We can think of set $S$ as a measure of dependence between null hypothesis in $\cH_0$. As shown in \eqref{eqn:S}, if $\big( \{k_1,\ell_1\} , \{k_2,\ell_2\} \big) \in S$, it intuitively means there is some ``path'' linking edges $(k_1,\ell_1)$ and $(k_2,\ell_2)$ together, which means they are somehow ``dependent'' or ``correlated''.
% Intuitively, when $|S|$ is larger, i.e., dependence is higher, the multiple testing problem is harder.  {     We also need a trade-off between $|{\cal H}_0|$ and $|\widetilde{{\cal H}}_1|$. Because the ideal case is both $|{\cal H}_0|$ and $|\widetilde{{\cal H}}_1|$ are all large for \eqref{eqn:depend} to hold. However, there is a natural constraint that  $|{\cal H}_0|+|\widetilde{{\cal H}}_1| \leq J$. 
  
% }
% % Also $|\cH_0|$ is the number of true null hypotheses. If the graph is too connected (where $|\cH_0|$ is typically small) then the multiple testing problem is harder.
% For example, if $J$ and $|\cH_0|$ are at the order of $d^m$, then \eqref{eqn:depend} holds when $$
% |S| = o \Big( \frac{d^m}{\log d} |\widetilde{{\cal H}}_1| \Big). $$
% }


% (i)
% $$   \frac{ J\log d }{|\cB|} \cdot \Big( \frac{(\log d)^{19 / 6}}{n^{1 / 6}} + \frac{(\log d)^{11 / 6}J^{1/3}}{n^{1 / 6} |\cB|^{1 / 3}} + s\frac{(\log d)^{3} }{\sqrt{n}} + \frac{J}{d^{\mu+1}|\cB|} \Big)=o(1).$$

% (ii)

% $$   \frac{ J\log d }{|\cB||{\cal H}_0|} + \frac{ J\log d }{|\cB||{\cal H}_0|^2} |S| =o(1).
% $$ 
% where $$\tilde{\mathcal{H}}_{1}=\Bigl\{j \in \mathcal{H}_{1}: \forall (j_1,j_2) \in N_{j}^c,\bigl|\Theta^*_{j_1j_2}\bigr|> C_0 \sqrt{\log d / n}\Bigr\},$$
% and
% $$S= \bigcup_{j_{1}, j_{2} \in \mathcal{H}_{0}, j_{1} \neq j_{2}} \Big\{(k_1,l_1) \in N_{j_{1}}, (k_2,l_2) \in N_{j_{2}}: \Theta^*_{k_1k_2} \Theta^*_{l_1l_2}+\Theta^*_{k_1l_2} \Theta^*_{k_2l_1} \neq 0 \Big\},$$
% with
% \[
% N_{j}=\Bigl\{(j_1, j_2)\in V_j \times V_j: \Theta^*_{j_1j_2}=0\Bigr\}, \qquad N_{j}^{c}=\Bigl\{(j_1, j_2)\in V_j \times V_j: \Bigl|\Theta^*_{j_1j_2}\Bigr|>0\Bigr\}.
% \]






% Based on Algorithm \ref{alg:2}, we have the following theorem controlling \mathrm{FDP} and FDR. Proof can be found in Appendix \ref{sec:pf:FDR}. 
% \begin{restatable}[\mathrm{FDP}/FDR control]{theorem}{thmFDR}\label{thm:FDR} Suppose  Assumptions \ref{ass:regularcon} and \ref{ass:spadepend} are satisfied.
% We have that Algorithm \ref{alg:2}  satisfies: as $(n, d) \rightarrow \infty$,     
% $$   
% \mathrm{\mathrm{FDP}} \leq q \frac{J_{0}}{J}+o_{P}(1) \quad \text { and } \quad \lim _{(n, d) \rightarrow \infty} \mathrm{FDR} \leq q \frac{J_{0}}{J}, 
% $$
% for  Gaussian graphical models and Ising models.
% \end{restatable}

% \begin{theorem}[\mathrm{FDP}/FDR control]\label{thm:FDR}
% Suppose  Assumptions \ref{ass:scaling} and \ref{ass:depend} are satisfied.
% We have that Algorithm \ref{alg:2}  satisfies: as $(n, d) \rightarrow \infty$,     
% $$   
% \mathrm{\mathrm{FDP}} \leq q \frac{J_{0}}{J}+o_{P}(1) \quad \text { and } \quad \lim _{(n, d) \rightarrow \infty} \mathrm{FDR} \leq q \frac{J_{0}}{J}, 
% $$
% for  Gaussian graphical models and Ising models.
% \end{theorem}

% \begin{remark}
% Because of  the equivalence of Algorithms \ref{alg:2} and \ref{alg:3} in Proposition \ref{prop:2-3} with $\tilde \cV = \cV$, we have both algorithms can control \mathrm{FDP} and FDR.
% \end{remark}


% {   check notation below}


% The following theorem shows that our procedure is also powerful.
% \begin{theorem}[Power Analysis]\label{thm:power}
% {   Suppose conditions in
% Lemma \ref{lem:GMB-GGM} are satisfied for Gaussian graphical models, or  conditions in
% Lemma  \ref{lem:GMB-Ising} are satisfied for Ising models.}
% We have under the alternative hypothesis $H_{1j}$ in \eqref{eqn:hypo}, assuming \yue{ $\min_{e \in E(F_j), j \in [J]}| \Theta^*_{e}| >  C_{0} \sqrt{\frac{\log d}{n}}$ }
% for some sufficiently large constant $C_0$, we have
% \begin{equation*} 
%   
% \mathbb{P}\bigl(\psi_{j, \alpha}=1 \text{ for all $j \in \cH_1$} \bigr) \rightarrow 1 \ \text{ as } n,d \to \infty.    
% \end{equation*}


% \end{theorem}



 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

\subsection{Theoretical results for Gaussian graphical model and  Ising model on persistent homology}\label{sec:omit:GGMIsing}

\begin{restatable}%[Statistical guarantee on the persistent barcodes under GGM]
{corollary}{corbarcodeGGM}\label{cor:ph:barcodeGGM} Suppose Assumption \ref{ass:phspadepend} is satisfied for some $\mu_1>0$ and $\log d/\log n=O(1)$. 
For Gaussian graphical model with $\Theta^*\in {\cal U}(s)$, we further assume $s^2\log^4(dn)/n=o(1)$, then the persistent barcodes obtained by Algorithm \ref{alg:ph:barcode}  satisfies: for any $\epsilon>0$ 
\[
\mathrm{uFDP}\leq q+o_P(1),\qquad \mathrm{uFDR}\leq q +o(1).
\]
and
\begin{equation*}
\mathbb{P}\Bigl(Z \big(\mu + C\sqrt{\log d/n} \big) \subseteq \hat{ Z}(\mu) \text{ for all }\mu\in(\mu_0,\mu_1) \Big) = 1- o(1).
\end{equation*}   
\end{restatable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}%[Statistical guarantee on the persistent barcodes under Ising models]
{corollary}{corbarcodeIsing}\label{cor:ph:barcodeIsing} Suppose Assumption \ref{ass:phspadepend} is satisfied for some $\mu_1>0$ and $\log d/\log n=O(1)$. 
For Ising models with $w^*\in {\cal W}$, then the persistent barcodes obtained by Algorithm \ref{alg:ph:barcode}  satisfies: for any $\epsilon>0$, 
\[
\mathrm{uFDP}\leq q+o_P(1),\qquad \mathrm{uFDR}\leq q +o(1),
\]
and
\begin{equation*}
\mathbb{P}\Bigl(Z \big(\mu + C\sqrt{\log d/n} \big) \subseteq \hat{ Z}(\mu) \text{ for all }\mu\in(\mu_0,\mu_1) \Big) = 1- o(1).
\end{equation*}   
\end{restatable}






==> discussion.tex <==
% !TEX root = main.tex



\section{Discussion}\label{sec:discussion}





%%% Local Variables:
%%% TeX-master: "atlas"
%%% End:


==> homology.tex <==
% !TEX root =main.tex
% \subsection{Discovering various subgraphs with FDR control}
% Note that Algorithm \ref{alg:3} discovers subgraphs with the same structure. In practice, researchers may hope to discover subgraphs with different structure simultaneously. For example, in a protein network, biologist may be interested in discovering different protein groups of  different regulatory functions. This can also apply to testing the topological structure of a graph (e.g., estimating the order-$1,2$ betti number by selecting cycles, voids etc). In this section, we propose an algorithm  to select subgraph of different structure with bounded size and provide corresponding FDR control.% with FDR control. 

% Denote  the sequence of structure of interest to select by $\{F_j:j=1,2,\ldots,J\}$.  For example, $F_1$ could be the triangle structure while $F_2$ could be the $4$-clique structure, and we want to test whether the proteins in $F_1\subseteq G^*$ form a triangle structure and the proteins in $F_2\subseteq G^*$ form a $4$-loop structure. Formally speaking, we want to test whether $F_j\subseteq G^*$, $j=1,2,\ldots,J$. Note that it could be quite computationally expensive if we explore all the $J$ subgraphs while most of the structure could be insignificant due to the sparsity nature of the graph data. To  make the algorithm more achievable regarding various computational feasibility, we develop the algorithm such that it not only can select subgraphs with different structure but also can balance the trade off between computational  and statistical efficiency by exploiting the monotonicity of the graph structure.

% We transfer the estimated graph into $\tbinom{d}{m}$ large estimated subgraphs each with  distinct $m$ nodes where $m$ satisfies $d-m=O(1)$ ( e.g., $m$ could be $d-1$, $d-2, \ldots$). For $s=1,2,\ldots,\tbinom{d}{m}$, denote the $s$-th large subgraphs by $G^{(s)}=(V^{(s)},E^{(s)})$ where $V^{(s)}$ is the node set and $E^{(s)}= \{(u,v)\in V^{(s)}\times V^{(s)}:u\neq v\}$ is the edge set. At each large subgraph $G^{(s)}$, it is seen from Algorithm \ref{alg:5} that we can exploit the monotonicity to terminate the searching at an early time for a sparse subgraph. Therefore, we could select the subgraphs of interest with adaptive computation regrading the sparsity  in each of the large $O(\tbinom{d}{m})$ subgraphs instead of exhaustively searching all $J=\Omega(\tbinom{d}{m})$  small subgraphs. This could potentially reduce a tremendous of combinatorial computation  especially when the graph is extremely sparse.


% \begin{algorithm}[H]
%     \caption{Efficient algorithm for selecting  various structure with FDR control \label{alg:5}}
    
%     Input: $\widetilde{{\Theta}}$, FDR level $q$. 
    
%     Initialize tuning parameter $m$, $\alpha_j = 1$ for $j \in [J]$ and ${\cal V}:=\{V\subseteq V^*:|V|=m\}$\;
    
%     Calculate screened edge set $\widetilde{E}(q)= \Bigl\{(u,v): \sqrt{n}(|\widetilde{\Theta}_{uv}|) \geq \widehat{c}(q, \{(u,v)\}),u\neq v\in V^*\Bigr\}$ and screened subgraph set $\mathcal{I}=\big\{1 \leq j \leq J: F_j \subseteq (V^*,\widetilde{E}(q))\big\}$\; 
    
%     \For{ $s=1,2,\ldots,|{\cal V}|$}{
%     Initialize $V$ to be the $s$-th element of ${\cal V}$ \;
%     Calculate   $(\alpha^{(s)}_1,\alpha^{(s)}_2, \ldots, \alpha^{(s)}_J)=\texttt{PValueEstimation}(\widetilde\Theta, V,\mu,{\cal I})$\; 
%     }  
%     Update $p$ values $\alpha_j=\min_{1\leq s\leq |{\cal V}|}\{\alpha^{(s)}_j\}$, for $j\in {\cal I}$\;
%     Order $\alpha_{1},\alpha_{2},\ldots,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max}=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
%     Output: Reject hypotheses $\{H_{0j}(\mu):\alpha_{j} \leq \alpha_{(j_{\max})}\}$.
% \end{algorithm}
% %Jan 29
% % Denote  the sequence of structure of interest to select by $\{G_j=(V_j,E_j):j=1,2,\ldots,J\}$.  For example, $G_1$ could be the triangle structure while $G_2$ could be the $4$-clique structure, and we want to test whether the proteins in $G_1\subseteq G^*$ form a triangle structure and the proteins in $G_2\subseteq G$ form a $4$-loop structure. Formally speaking, we want to test whether $G_j\subseteq G^*$, $j=1,2,\ldots,J$. Note that it could be quite computationally expensive if we explore all the $J$ subgraphs while most of the structure could be insignificant due to the sparsity nature of the graph data. To  make the algorithm more achievable regarding various computational feasibility, we develop the algorithm such that it not only can select subgraphs with different structure but also can balance the trade off between computational  and statistical efficiency by exploiting the monotonicity of the graph structure.

% % We transfer the graph into $\tbinom{d}{m}$ large subgraphs each with  distinct $m$ nodes where $m$ satisfies $d-m\ll S$ ( e.g., $m$ could be $d-1$, $d-2, \ldots$). For $s=1,2,\ldots,\tbinom{d}{m}$, denote the $s$-th large subgraphs by $G^{(s)}=(V^{(s)},E^{(s)})$ where $V^{(s)}$ is the node set and $E^{(s)}= \{(x,y)\in E:x,y\in V^{(s)}\}$ is the edge set. At each large subgraph, it is seen from Algorithm \ref{alg:5} that we can exploit the monotonicity to terminate the searching at an early time for a sparse subgraph. Therefore, we could select the subgraphs of interest with adaptive computation regrading the sparsity  in each of the large $O(\tbinom{d}{m})$ subgraphs instead of exhaustively searching all $J=\Omega(\tbinom{d}{S})$  small subgraphs. Therefore, this may reduce a tremendous of combinatorial computation  especially when the graph is extremely sparse.



% %Let us first introduce the primal algorithm.

% % \begin{algorithm}[htbp]
% %     \caption{Discovering loops with FDR control\label{alg:4}}
    
% %     \SetKwInOut{Input}{Input}
% %     \SetKwInOut{Output}{Output}
% %     \Input{$\widetilde{{\Theta}}$,   significance level $\alpha$, subgraph size $m$. }
% %     \For{$s=1,2,\ldots,\tbinom{d}{m}$}{
% %     %%%%%%%   For loop   %%%%%%%%%%%%%%%%%%%%%%%%%
% %     Initialize  $t=0,\, E_{0,s}= \{(x, y)\in V^{(s)} \times V^{(s)}:x\neq y\}$, and $E_{0,s}^c=\emptyset$.
% %     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %     \Repeat{$ \mathcal{R}=\varnothing$}
% %     { 
% %     $t \leftarrow t+1$\;
% %     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %     Select the rejected edges $\mathcal{R} \leftarrow\Bigl\{(x, y) \in E_{t-1,s}:\,\sqrt{n}| \widetilde{{\Theta}}_{xy}\big|>\widehat{c}\Bigl(\alpha, E_{t-1,s}\Bigr)\Bigr\}$\;
% %     %%%%%%%%%%%%%%%%%%%%%%%%%%%
% %     $E_{t,s} \leftarrow E_{t-1,s} \backslash \mathcal{R}$ and  $E_{t,s}^c \leftarrow E_{t-1,s}^c \cup \mathcal{R}$\;
% %     }
% %     %%%%%%%%%%%%%%%%%%%%%%%%
% %     \For{$j=1,2,\ldots,J$}{Let $\psi^{(s)}_{j,\alpha}$ be $1$ if $G_j^*\subseteq G^{(s)}$ and $0$ otherwise.}
% %     }
% %  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
% %   	\Output{$\psi_{j, \alpha}=\max_{1\leq s \leq \tbinom{d}{m}}\{\psi^{(s)}_{j,\alpha}\}$, for $1\leq j\leq J$.}
% % \end{algorithm}


% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{algorithm}[htbp]
% %     \caption{Efficient algorithm for discovering subgraphs with FDR control \label{alg:5}}
% %     \SetKwInOut{Input}{Input}
% %     \SetKwInOut{Output}{Output}
% %     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% %     Denote $\widetilde{E}(q):= \Bigl\{(x,y)\in V\times V: \sqrt{n}|\widetilde{\Theta}_{xy}| \geq \widehat{c}\Bigl(q, \{(x,y)\}\Bigr),x\neq y\Bigr\}$\;
% %     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %     \For{$s = 1,2, \ldots, \tbinom{d}{m}$}{
% %     Let $ E^{(s)}= \{(x,y)\in \widetilde{E}(q):(x, y)\in V^{(s)} \times V^{(s)}\}$\;
% %     %%%%%%%%%%%% repeat loop  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %     Rearrange $E^{(s)}$ as $\{e_{(1)},e_{(2)},\ldots,e_{(|E^{(s)}|)}\}$ with 
% %     %Order the elements in the set $\Bigl\{|\widetilde{\Theta}_e|:e\in {E^{(s)}}\Bigr\}$ as 
% %     $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|E^{(s)}|)}}|$\; %where $\Bigl|\widetilde{\Theta}_{e_{(k)}}\Bigr|$
% %     %denotes the $k$-th largest entry and $e_{(k)}$ denotes the corresponding edge\;
% %       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %   For each $e\in E^{(s)}$ , define  $\widetilde{E}^{(s)}(e)=\{(x,y)\in E^{(s)}:|\widetilde{\Theta}_e|\geq \widetilde{\Theta}_{xy}|\}$ and 
% %   $K^{(s)}=\min\big\{1 \leq k \leq\left|E^{(s)}\right|:e_{(k+1)} \text{ forms at least  a loop with some edges in } \{e_{(1)},  ..., e_{(k)}\}$   and  there is at least an edge $e$ in some of these loops,  satisfying $\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e}|, \widetilde{E}^{(s)}({e})\Bigr)>q \big\}$ \;
% %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %   \For{$j=1,2,\ldots,J$}{
% %   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %   If $E^*_j\subseteq \{e_{(1)},e_{(2)},\ldots,e_{(K^{(s)})}\}$,  compute $\alpha_{j}^{(s)}=\max_{1\leq k\leq K}\{\widehat{c}^{-1}\Bigl(\sqrt{n}| \widetilde{\Theta}_{e_{(k)}}|, \widetilde{E}^{(s)}(e_{(k)})\Bigr)\}$, where $K=\argmax_k\{k: e_{(k)}\in E^*_j\}$; otherwise set $\alpha_j^{(s)}=1$\;}
% %     }
  
    
% %     Let $\alpha_{j}=\min_{1 \leq s \leq \tbinom{d}{m}}\{\alpha_j^{(s)}\}$, for $1\leq j\leq J$ \; 
    
% %     Order $\alpha_{1},\alpha_{2},\ldots,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
% %     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
% % \end{algorithm}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% % \begin{algorithm}[H]
% %     \caption{Efficient algorithm for discovering loops on $G$ with FDR control \label{alg:5}}
% %     \SetKwInOut{Input}{Input}
% %     \SetKwInOut{Output}{Output}
% %     \Input{$\widetilde{{\Theta}}$,  nominal FDR level $q$. }
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% %     Initialize $\alpha^{(s)}_j=1$, for $1\leq j\leq J, 1\leq s\leq \tbinom{d}{m}$; $\widetilde{E}(q)= \Bigl\{e\in E: \sqrt{n}(|\widetilde{\Theta}_e|) \geq \widehat{c}(q, \{e\})\Bigr\}$\;
% %     \For{$s = 1,2, \ldots, \tbinom{d}{m}$}{
% %   Let $ \widetilde{E}^{(s)}= \{e\in \widetilde{E}(q):e\in E^{(s)}\}$\;
% %     %%%%%%%%%%%% repeat loop  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %     Rearrange $\widetilde{E}^{(s)}$ as $\{e_{(1)},e_{(2)},\ldots,e_{(|\widetilde{E}^{(s)}|)}\}$ with 
% %     $|\widetilde{\Theta}_{e_{(1)}}| \geq|\widetilde{\Theta}_{e_{(2)}}| \geq \ldots \geq|\widetilde{\Theta}_{e_{(|\widetilde{E}^{(s)}|)}}|$\; 
% %      For each $e\in E^{(s)}$ , define  $E^{(s)}(e)=\{e'\in E^{(s)}:|\widetilde{\Theta}_e|\geq |\widetilde{\Theta}_{e'}|\}$\;
% %       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %      \For{$1\leq K\leq |\widetilde{E}^{(s)}|$ }{
% %      \For{$1\leq j\leq J$}{
% %      if $G^*_j\subseteq \Bigl(V^{(s)},\{e_{(1)},e_{(2)},\ldots,e_{(K)}\}\Bigr)$ but  $G^*_j\nsubseteq \Bigl(V^{(s)},\{e_{(1)},e_{(2)},\ldots,e_{(K-1)}\}\Bigr)$\; 
% %      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %      Update $\alpha_{j}^{(s)}=\max_{1\leq k\leq K}\Bigl\{\widehat{c}^{-1}\Bigl(\sqrt{n}(| \widetilde{\Theta}_{e_{(k)}}|), E^{(s)}(e_{(k)})\Bigr)\Bigr\}$\;
% %      if $\alpha_{j}^{(s)}>q$, go to $12$\;
% %      }
% %      } 
% %     }
% %     Order $\alpha_{1},\alpha_{2},\ldots,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \cdots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$. Let $j_{\max }=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$.
    
    
% %     \Output{Reject $\Bigl\{j: \alpha_{j} \leq \alpha_{(j_{\max })}\Bigr\}$ if $j_{\max }>0$; reject $\varnothing$ otherwise.}
    
    
% % \end{algorithm}
% At the same time, the flexible choice of $m$ enable us to preserve the statistical efficiency as much as possible. Note that  if we choose a small $m$, for example, we let $m=|V^*|$ and focus on one structure and, then Algorithm \ref{alg:5} will reduce to Algorithm \ref{alg:3}. 





% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \iffalse
% \begin{restatable}{proposition}{propequivhomo}\label{prop:4-5} 
% For $1\leq j\leq J$ and a specified significance level $\alpha$ with $\alpha\leq q$, let $\psi_{j,\alpha}$ be that defined in Algorithms \ref{alg:4}, and $\alpha_j$ be that defined in Algorithms \ref{alg:5}.  We have that
% \[
% \psi_{j,\alpha}=1\qquad \Longleftrightarrow \qquad \alpha_j\leq \alpha,\qquad \mbox{ for any $\alpha\leq q$. 
% }
% \]
% \end{restatable}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{restatable}[Single test lemma]{lemmma}{testhomology}\label{lem:testhomology}
%  {\jiajun conditions},  we have the following results on type I error and power.

% (i) Under the alternative hypothesis $H_{1,j}$, assuming $\min_{\{e \in V \times V: \Theta_{e}\neq 0\}}\{| \Theta_{e}|\} > 2C_{0} \sqrt{\frac{\log d}{n}}$ for some positive constant $C_0$, for $\red \alpha=\Omega(d^{-|V^*|})$
% \begin{equation*}
% \min_{ j \in [J]} 
% \mathbb{P}\Bigl(\psi_{j, \alpha}=1\Bigr) = 1+{\jiajun o(\frac{1}{J})}.    
% \end{equation*}

% (ii) Under the null hypothesis $H_{0,j}$, we have
% \begin{equation*}
% \lim _{(n, d) \rightarrow \infty} \P\Bigl(\psi_{j, \alpha}=1\Bigr) \leq \alpha.    
% \end{equation*}
% \end{restatable}
% \fi
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For Algorithm \ref{alg:5}, we have the following theorem which guarantee the FDR control of the selected structure of different shapes.
% \begin{restatable}[FDR control]{theorem}{thmFDRhomology}\label{thm:FDRhomology}
%  Under Assumption \ref{ass:signal}, we have that Algorithm \ref{alg:5} % with \eqref{eqn:alphahat} as input
%  satisfies: as $(n, d) \rightarrow \infty$,
% $$
% \mathrm{FDP} \leq q \frac{J_{0}}{J}+o_{\mathbb{P}}(1) \quad \text { and } \quad \lim _{(n, d) \rightarrow \infty} \mathrm{FDR} \leq q \frac{J_{0}}{J} 
% $$
% \end{restatable}




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \section{Ising Model}
% \begin{algorithm}[H]
%     \caption{Graph selection in Ising model}  \label{alg:Ising}
    
%     Input: $M$ (estimator for $\theta \omega$), $\theta$, $\cV$, FDR level $q$. 
    
%     Initialize $\alpha_j = 1$ for $j \in [J]$\;
    
%     \For{$V\in \cV$}{
%     Update the $p$-values by $(\alpha_1, \ldots, \alpha_J)=\texttt{PValueEstimation}(M, V)$ \; 
%     }  
       
%     Order $\alpha_{1},\ldots,\alpha_{J}$ as $\alpha_{(1)} \leq \alpha_{(2)} \leq \ldots \leq \alpha_{(J)}$ and set $\alpha_{(0)}=0$\;
%     Let $j_{\max}=\max \Bigl\{0 \leq j \leq J: \alpha_{(j)} \leq q j / J\Bigr\}$\;
    
%     Output: Reject $H_{0j}$ for those $j$ such that $\alpha_{j} \leq \alpha_{(j_{\max})}$.  Reject nothing if $j_{\max}= 0$.
    
%     \vspace{10pt}

% % \SetKwFunction{FMain}{PValueEstimation}
% % \SetKwRepeat{Do}{do}{while}
% % \SetKwProg{Fn}{Function}{:}{}
% % \Fn{\FMain{$M,V$}}{
% % Add edges with weights from high to low based on $M_{V\times V}$  until a subgraph of interest  $H_j$ emerges\;
% % Let $\alpha_j=\widehat{c}^{-1}\bigl(\min_{e\in E(H_j)}M_e - Q, \red V \times V\bigr)$\;
% %       %Let $ E= \{(j, k)\in V \times V: j\neq k\}$. %and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
% %     % Let $E = \{(u, v)\in V \times V: u\neq v\}$\;
% %     % Order the edge weight estimators $\{|\widetilde{\Theta}_{e} |: e \in E\}$ as $|\widetilde{\Theta}_{e_{(1)}}|  \leq \ldots  \leq |\widetilde{\Theta}_{e_{(|E|)}}| $, where $|\widetilde{\Theta}_{e_{(k)}}|$
% %     % denotes the $k$-th smallest estimator and $e_{(k)}$ denotes the corresponding edge\;
  
% %     % Initialize $k = |E|$; 
    
% %     % \Do{$p_{k+1}\le q$ or $k\ge 1$}{
% %     % Let $p_k= \widehat{c}^{-1}\bigl(\sqrt{n} | \widetilde{\Theta}_{e_{(k)}}|, \{e_{(1)}, \ldots, e_{(k)}\}\bigr)$;
    
% %     % Find $I_k=\big\{ j \in [J] : F_j \subseteq (V,\{e_{(k)}, e_{(k+1)},\ldots, e_{(|E|)}\}) \big\}$\;
    
% %     % Update $\alpha_{j}=\max\{p_{k}, p_{k+1},\ldots,p_{|E|}\}$ for all $j \in I_k \backslash I_{k+1}$, where $I_{|E|+1}=\emptyset$\;
    
% %     % $k=k-1$\;
% %     % }
% %     % Output: $\{\alpha_j:1\leq j\leq J\}$.
% % }  
% % \textbf{End Function} 

% \SetKwFunction{FMain}{PValueEstimation}
% \SetKwRepeat{Do}{do}{while}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{$M,V$}}{
%       %Let $ E= \{(j, k)\in V \times V: j\neq k\}$. %and denote the $|E_{jl}|$ edges in $E_{jl}$ as $e_{1},  e_{2},...,e_{|E_{jl}|}$, respectively.
%     Let $E = \{(u, v)\in V \times V: u\neq v\}$\;
%     Order the edge weight estimators $\{M_e: e \in E\}$ as $M_{e_{(1)}}  \leq \ldots  \leq M_{e_{(|E|)}} $, where $M_{e_{(k)}}$
%     denotes the $k$-th smallest estimated weight and $e_{(k)}$ denotes the corresponding edge\;
  
%     Initialize $k = |E|$; 
    
%     \Do{$p_{k+1}\le q$ or $k\ge 1$}{
%     Let $p_k= \widehat{c}^{-1}\bigl({\red M_{e_{(k)}}-\big(\text{tanh}(\theta)- 2\tau) }, \{e_{(1)}, \ldots, e_{(k)}\}\bigr)$;
    
%     Find $I_k=\big\{ j \in [J] : F_j \subseteq (V,\{e_{(k)}, e_{(k+1)},\ldots, e_{(|E|)}\}) \big\}$\;
    
%     Update $\alpha_{j}=\max\{p_{k}, p_{k+1},\ldots,p_{|E|}\}$ for all $j \in I_k \backslash I_{k+1}$, where $I_{|E|+1}=\emptyset$\;
    
%     $k=k-1$\;
%     }
%     Output: $\{\alpha_j:1\leq j\leq J\}$.
% }  
% \textbf{End Function} 

% \end{algorithm}
% Denote $\psi_{j,\alpha}=1$ if $\alpha_{j}\leq \alpha$ and $\psi_{j,\alpha}=0$ otherwise, for $1 \leq j \leq J$.  

% Let $M_{uv}:= \hat \EE X_u X_v = n^{-1} \sum_{i=1}^{n} X_{iu} X_{iv}$ and 
% $M^*_{uv}:= \EE X_u X_v, u, v \in [d]$. We have $$\sqrt{n}(M_{uv}-M^*_{uv}) \to N(0, \Var X_u X_v).$$


% Ising model is a collection of $d$ binary random variables $\bX=(X_{1}, X_{2}, \ldots X_{d})^{\top} \in \{1,-1\}^{d}$ with distribution
% \begin{equation}
% \mathbb{P}_{\theta, G_{\mathbf{w}}}(\boldsymbol{X}=\mathbf{x}) \propto \exp \Big(\theta \sum_{(u, v) \in E} w_{u v} x_{u} x_{v}\Big),    
% \end{equation}
% where $\theta \geq 0, G_{\wb}=(G, \wb)$ where $G=([d], E)$ is a  graph and $\mathbf{w} \in \mathbb{R}^{\binom{d}{2}}$ are weights on the edges. For $(u, v) \notin E(G)$, $w_{u v}=0$. 


% Let $\bX^{1}, \bX^{2}, \cdots, \bX^{n}\in \{1,-1\}^{d}$ be $n$ i.i.d. samples
% from the Ising model. 
% Let $$ M_{uv}:= \hat \EE X_u X_v = \frac{1}{n} \sum_{i=1}^{n} X_{u}^{i} X_{v}^{i} \ \text{ and }\ 
% M^*_{uv}:= \EE X_u X_v, u, v \in [d].$$ 
% We have $$\sqrt{n}(M_{uv}-M^*_{uv}) \to N(0, \Var (X_u X_v)).$$

% Let 
% \begin{equation}
% \begin{aligned}
% & T_E = \max_{(u,v) \in E} \sqrt{n}
% (M_{uv}-M^*_{uv}) = \max_{(u,v) \in E} \frac{1}{\sqrt{n} }\sum_{i=1}^{n} (X_{u}^{i} X_{v}^{i}-\EE X_u X_v),
% \\
% & T_E^\cB = \max_{(u,v) \in E} \frac{1}{\sqrt{n} }\sum_{i=1}^{n} (X_{u}^{i} X_{v}^{i} - M_{uv})\xi_i , \\
% & \tilde T_E = \max_{(u,v) \in E} \frac{1}{\sqrt{n} } \sum_{i=1}^{n} (X_{u}^{i} X_{v}^{i} - M_{uv}) \red = 0  , \\
% & \tilde T_E^\cB = \max_{(u,v) \in E} \frac{1}{\sqrt{n} }  \sum_{i=1}^{n} (X_{u}^{i} X_{v}^{i} - M^*_{uv})\xi_i,
% \end{aligned}    
% \end{equation}
% and define
% \begin{equation}
% \widehat{c}(\alpha, E)=\inf \left\{t \in \mathbb{R}: \mathbb{P}\Big(T_{E}^{\mathcal{B}} \leq t \mid \bX\Big) \geq 1-\alpha\right\}.
% \end{equation}  

% \begin{lemma}
% {\red Condition} For any edge set $E \subseteq V\times V$, we have  
% \begin{equation}
% \lim_{(n, d) \rightarrow \infty} 
% \sup_{\mathbf{w} \in \mathbb{R}^{\binom{d}{2}}} 
% \sup_{\alpha\in(0,1)}\bigg|\mathbb{P}\Big(\max _{(u,v) \in E} \sqrt{n}\big|M_{uv}-M^*_{uv}\big|>\widehat{c}(\alpha, E)\Big)-\alpha\bigg|=0    
% \end{equation} 

% \end{lemma}

% % Under the null, $\psi_{j, \alpha}=1$ implies that $\alpha_j \leq \alpha$, i.e., at least one edge in $N_{j}$ is selected to the edge set $E(H_j)$ at level $\alpha$.  So we have
% % \begin{equation}\label{eqn:imply}
% % \max _{e \in N_{j}} M_e 
% % \geq \min_{e\in E(H_j)} M_e
% % \overset{\text{(i)}}{\geq}
% % Q + \widehat{c}\bigl(\alpha_j, V_j \times V_j\bigr)
% % \overset{\text{(ii)}}{\geq}
% % Q + \widehat{c}\bigl(\alpha, V_j \times V_j\bigr)
% % \overset{\text{(iii)}}{\geq}   \widehat{c}\bigl(\alpha, V_j \times V_j\bigr)
% % \overset{\text{(iv)}}{\geq}   \widehat{c}\bigl(\alpha, N_j\bigr).
% % \end{equation}


% \textbf{Key steps in proving FDR control:}

% 1. It suffices to prove that
% \begin{equation}
% \sup_{\alpha \in [\alpha_{L}, 1]}\Biggl|\frac{\sum_{j \in \mathcal{H}_{0}} \mathbbm{1}\Bigl(\max_{e \in N_{j}} (M_e-M_e^*) \geq \widehat{c}\bigl(\alpha, N_{j}\bigr)\Bigr)}{J_{0} \alpha}-1\Biggr| \rightarrow 0 \quad \text { in probability. }
% \end{equation}

% 2. Denote $$I_{j}(\alpha):=\mathbbm{1}\Bigl(\max_{e \in N_{j}} (M_e-M_e^*) \geq \widehat{c}\bigl(\alpha, N_{j}\bigr)\Bigr),$$
% It suffices to prove that
% \begin{equation}\label{eqn:goto0inProb}
%   \max _{1 \leq m \leq \lambda_{d}}\Bigl|\frac{\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})}{J_{0} \alpha^{m}}-1\Bigr| \rightarrow 0  \text { in probability}.  
% \end{equation}


% By the union bound argument and Chebyshev's inequality, we have
% \begin{small}
% \begin{equation}\label{eqn:Chebyshev}
% \begin{aligned}
% \mathbb{P}\Bigl(\max _{1 \leq m \leq \lambda_{d}}\Bigl|\frac{\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})}{J_{0} \alpha^{m}}-1\Bigr| \geq \epsilon\Bigr) 
% \leq  \sum_{m=1}^{\lambda_{d}} \mathbb{P}\Bigl(\Bigl|\frac{\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})}{J_{0} \alpha^{m}}-1\Bigr| \geq \epsilon\Bigr) 
% \leq  \sum_{m=1}^{\lambda_{d}} \frac{\mathbb{E}\Bigl[\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})-J_{0} \alpha^{m}\Bigr]^{2}}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}}. 
% \end{aligned}
% \end{equation}
% \end{small}
% Then we decompose 
% \begin{small}
% \begin{equation}\label{eqn:decompose}
% \begin{aligned}
%  \sum_{m=1}^{\lambda_{d}} \frac{\mathbb{E}\Bigl[\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})-J_{0} \alpha^{m}\Bigr]^{2}}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}} 
% = & \sum_{m=1}^{\lambda_{d}} \frac{\sum_{j \in \mathcal{H}_{0}} \operatorname{Var}\Bigl(I_{j}(\alpha^{m})-J_{0} \alpha^{m}\Bigr)}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}}
% + \sum_{m=1}^{\lambda_{d}} \frac{\Bigl(\mathbb{E}\Bigl[\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})-J_{0} \alpha^{m}\Bigr]\Bigr)^{2}}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}} \\
% & +\sum_{m=1}^{\lambda_{d}} \frac{\sum_{j_{1}, j_{2} \in \mathcal{H}_{0}, j_{1} \neq j_{2}} \operatorname{Cov}\Bigl(I_{j_{1}}(\alpha^{m}), I_{j_{2}}(\alpha^{m})\Bigr)}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}} \\
% = & I_1 + I_2 + I_3.
% \end{aligned}
% \end{equation}
% \end{small}

% we immediately have
% $$
% \sum_{m=1}^{\lambda_{d}} \frac{\sum_{j \in \mathcal{H}_{0}} \operatorname{Var}\Bigl(I_{j}(\alpha^{m})-J_{0} \alpha^{m}\Bigr)}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}}  \leq \frac{C}{\epsilon^{2} J_{0} \alpha_{L}} \frac{\beta_{\lambda_{d}}}{h_{d}} 
% $$
% and
% $$
% \sum_{m=1}^{\lambda_{d}} \frac{\Bigl(\mathbb{E}\Bigl[\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})-J_{0} \alpha^{m}\Bigr]\Bigr)^{2}}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}} \leq \frac{\beta_{\lambda_{d}}}{\epsilon^{2} h_{d}} \eta^2(d, n, \zeta_{1}, \zeta_{2}, \alpha_{L})    
% $$
% since
% $$\Biggl|\frac{ \mathbbm{1}\Bigl(\max_{e \in N_{j}} (M_e-M_e^*) \geq \widehat{c}\bigl(\alpha, N_{j}\bigr)\Bigr)}{\alpha}-1\Biggr| = \eta (d, n, \zeta_{1}, \zeta_{2}, \alpha_{L}) $$
% where 
% \begin{equation}
% \eta (d, n, \zeta_{1}, \zeta_{2}, \alpha_{L}) 
% \red = xxxxx
% \end{equation}
% with $\red \zeta_{1} =  xxxxx ,  \zeta_{2}= xxxxx.$

% 3. 
% Let
% $$W_{j}(\alpha):=\mathbbm{1}\Bigl(\max_{e \in N_{j}} Z_e \geq {c}\bigl(\alpha, N_{j}\bigr)\Bigr), $$ 
% and
% $$I_3'=\sum_{m=1}^{\lambda_{d}} \frac{\sum_{j_{1}, j_{2} \in \mathcal{H}_{0}, j_{1} \neq j_{2}} \operatorname{Cov}\Bigl(W_{j_{1}}(\alpha^{m}), W_{j_{2}}(\alpha^{m})\Bigr)}{\epsilon^{2} J_{0}^{2} {\alpha^{m}}^{2}},$$
% where Gaussian vector $\{Z_e\}_{e \in N_j}$ shares the same asymptotic mean and asymptotic covariance matrix with $\{M_e-M_e^*\}_{e \in N_j}$. So $\E \{Z_e\}_{e \in N_j}=0 $ and $\Var (\{Z_e\}_{e \in N_j}) = \Var (\{X_u X_v\}_{(u,v) \in N_j}) $.

% We have
% \begin{equation}
% \bigl|I_3-I_3' \bigr| 
% \leq \frac{1}{\epsilon^{2}} \sum_{m=1}^{\lambda_{d}} \frac{\eta(d, n, \zeta_{1}, \zeta_{2}, \alpha_{L})}{\alpha^{m}} 
% \lesssim \frac{\beta_{\lambda_{d}}}{\alpha_{L} \epsilon^{2} h_{d}} \cdot \eta(d, n, \zeta_{1}, \zeta_{2}, \alpha_{L}).
% \end{equation}


% 5.   
% $$ \operatorname{Cov}\Bigl(W_{j_{1}}(\alpha), W_{j_{2}}(\alpha)\Bigr) = \Big|\mathbb{P}\Big(\max_{e \in N_{j_{1}} \cup N_{j_{2}}} Z_{e} \geq t\Big)-\mathbb{P}\Big(\max_{e \in N_{j_{1}} \cup N_{j_{2}}}Z_{e}^{\prime} \geq t\Big)\Big|$$
% where   $(Z_{e}^{\prime})_{e \in N_{j_{1}}} \indep(Z_{e}^{\prime})_{e \in N_{j_{2}}}$. 

% Next, we calculate the covariance matrix of $ \{Z_{e}\}_{e \in N_{j_{1}} \cup N_{j_{2}}}$, denoted by $\Sigma^{Z}$. We also let $\Sigma^{Z}_{11}=\Var (\{Z_{e}\}_{e \in N_{j_{1}}})$, $\Sigma^{Z}_{22}=\Var (\{Z_{e}\}_{e \in N_{j_{2}}})$ and $\Sigma^{Z}_{12}=\Cov (\{Z_{e}\}_{e \in N_{j_{1}}}, \{Z_{e}\}_{e \in N_{j_{1}}})$.  

% For $(k_1,\ell_1) \in N_{j_1} $ and $(k_2,\ell_2) \in N_{j_2}$, we have 
% $$\Cov(Z_{(k_1,\ell_1)}, Z_{(k_2,\ell_2)}) = \Cov(X_{k_1}X_{\ell_1}, X_{k_2}X_{\ell_2}) =  \E(X_{k_1}X_{\ell_1}X_{k_2}X_{\ell_2}) - \E(X_{k_1}X_{\ell_1} )\E( X_{k_2}X_{\ell_2}).$$ 

% Generally we define
% \begin{equation}\label{eqn:S-Ising}
% \begin{aligned}
% S =\sum_{j_{1}, j_{2} \in \mathcal{H}_{0}, j_{1} \neq j_{2}} \bigg|  \Big\{ 
% & \Big( (k_1,\ell_1), (k_2,\ell_2) \Big): (k_1,\ell_1) \in N_{j_{1}}, (k_2,\ell_2) \in N_{j_{2}}, (k_1,\ell_1) \neq (k_2,\ell_2), \\
% & \E(X_{k_1}X_{\ell_1}X_{k_2}X_{\ell_2}) - \E(X_{k_1}X_{\ell_1} )\E( X_{k_2}X_{\ell_2}) \neq 0 \Big\} \bigg|,  
% \end{aligned}   
% \end{equation}
% and we have
% \begin{equation}
%     \bigl| \Pi' \bigr|  
%     \lesssim \frac{\beta_{\lambda_{d}}}{h_d} \frac{1}{\epsilon^{2} J_{0}^{2} \alpha_L} S.
% \end{equation}

% 6. Combining all the above bounds together, we have
% \begin{equation}\label{eqn:4.13}
% \begin{aligned}
%     & \mathbb{P}\Bigl(\max _{1 \leq m \leq \lambda_{d}}\Bigl|\frac{\sum_{j \in \mathcal{H}_{0}} I_{j}(\alpha^{m})}{J_{0} \alpha^{m}}-1\Bigr| \geq \epsilon\Bigr) \\
%   \lesssim &  \frac{C}{\epsilon^{2} J_{0} \alpha_{L}} \frac{\beta_{\lambda_{d}}}{h_{d}} + \frac{\beta_{\lambda_{d}}}{\epsilon^{2} h_{d}} \eta^2(d, n, \zeta_{1}, \zeta_{2}, \alpha_{L}) + 
%     \frac{\beta_{\lambda_{d}}}{\epsilon^{2} \alpha_{L} \ h_{d}} \cdot \Big( \eta(d, n, \zeta_{1}, \zeta_{2}, \alpha_{L}) 
%     + \frac{1}{J_{0}^{2}} |S| \Big) \\
%     \lesssim &  \frac{\beta_{\lambda_{d}}}{\epsilon^{2} h_{d}} \eta^2(d, n, \zeta_{1}, \zeta_{2}, \alpha_{L}) + \frac{\beta_{\lambda_{d}}}{\epsilon^{2} h_{d}\alpha_{L}} \cdot \Big( \frac{1}{J_0} + \eta(d, n, \zeta_{1}, \zeta_{2}, \alpha_{L}) 
%     + \frac{1}{J_{0}^{2}} |S| \Big),
% \end{aligned}
% \end{equation}
% and our goal is to show that \eqref{eqn:4.13} is $o(1)$.



% \begin{remark}
% If assuming the true graph $G^* = (V^*, E^*)$ is a forest, we can further give a closed form of $S$.
% \end{remark}









% Depending on the true graph, there are only two cases for $\mathcal{CP}_{G^*}(k_{1}, k_{2}, \ell_1,\ell_2)$. $\mathcal{CP}_{G^*}(k_{1}, k_{2}, \ell_1,\ell_2) = \{(k_1,k_2), (\ell_1,\ell_2)\}$ if $(k_1,k_2), (\ell_1,\ell_2) \in E^*$ or $\mathcal{CP}_{G^*}(k_{1}, k_{2}, \ell_1,\ell_2) = \{(k_1,\ell_2), (k_2,\ell_1)\}$ if $(k_1,\ell_2), (k_2,\ell_1) \in E^*$. So $$\E(X_{k_1}X_{\ell_1}X_{k_2}X_{\ell_2})
%  = \E(X_{k_1} X_{k_2}) \E(X_{\ell_1} X_{\ell_2}) $$ or 
%  $$\E(X_{k_1}X_{\ell_1}X_{k_2}X_{\ell_2})
%  = \E(X_{k_1} X_{\ell_2}) \E(X_{\ell_1} X_{k_2}). $$
% follows immediately from the fact that on a tree
% $\mathbb{E}_{\theta, G^*} X_{u} X_{v}=\tanh (\theta w_{u v}) $.
% Page 52 of Neykov and Liu






==> method.tex <==


% !TEX root = main.tex


% For type I error, under the null, we assume in $E_j$, $\Theta_{E^*}=0$, so
% \begin{equation}
% \begin{aligned}  
% \P_0\Bigl(\psi_{j, \alpha}=1\Bigr) 
% & = \P_0\Bigl(\min_{e \in E_{j}} \sqrt{n}| \widetilde{{\Theta}}_{e}| >\widehat{c}(\alpha, E_{j})\Bigr) \\
% & \leq \P_0\Bigl(\sqrt{n}| \widetilde{{\Theta}}_{E^*}| >\widehat{c}(\alpha, E_{j})\Bigr) \\
% & = \P_0\Bigl(\sqrt{n}| \widetilde{{\Theta}}_{E^*}-\Theta_{E^*}| >\widehat{c}(\alpha, E_{j})\Bigr) \\
% & \leq \P_0\Bigl(\max_{e \in E_{j}} \sqrt{n}| \widetilde{{\Theta}}_{e}-\Theta_{e}| >\widehat{c}(\alpha, E_{j})\Bigr)
% \rightarrow \alpha,
% \end{aligned}    
% \end{equation}
% So the Type I error is controlled as desired.

% Next, we prove our testing procedure is powerful, i.e., the power goes to one asymptotically. Under alternative, we have 
% \begin{equation}
% \begin{aligned}
% \inf_{j \in [J]}\P\Bigl(\psi_{j, \alpha}=1\Bigr) 
% & = \inf_{j \in [J]}\P\Bigl(\min_{e \in E_{j}} \sqrt{n}| \widetilde{{\Theta}}_{e}| >\widehat{c}(\alpha, E_{j})\Bigr) \\
% & \geq \inf_{j \in [J]}\P\Bigl(\min_{e \in E_{j}} \sqrt{n}| \Theta_{e}| > \widehat{c}(\alpha, E_{j})+\delta, \max_{e \in E_{j}} \sqrt{n}| \widetilde{{\Theta}}_{e}-\Theta_{e}| < \delta \Bigr) \\
% & \geq \P\Bigl(\min_{e \in V \times V} \sqrt{n}| \Theta_{e}| > \widehat{c}(\alpha, V \times V)+\delta, \max_{e \in V \times V} \sqrt{n}| \widetilde{{\Theta}}_{e}-\Theta_{e}| < \delta \Bigr) 
% \end{aligned}    
% \end{equation}

% From xxxxxx, we have that
% \begin{equation}
% \widehat{c}\Bigl(\alpha, V \times V\Bigr) \leq C_{0} \sqrt{\frac{\log d}{n}} \cdot \sqrt{n}=C_{0} \sqrt{\log d}
% \end{equation}
% and
% \begin{equation}
% \mathbb{P}\Bigl(\max _{e \in V \times V}\Bigl|\widetilde{{\Theta}}_{e}-{\Theta}_{e}\Bigr| \leq C_{0} \sqrt{\frac{\log d}{n}}\Bigr)>1-2 / d
% \end{equation}

% So taking $\delta$ as $C_{0} \sqrt{\frac{\log d}{n}}$, under the assumption that $$\min_{e \in V \times V} \sqrt{n}| \Theta_{e}| > C_{0} \sqrt{\frac{\log d}{n}},$$ we immediately arrive at 
% \begin{equation}
% \inf_{j \in [J]}\P\Bigl(\psi_{j, \alpha}=1\Bigr) 
% >1-2 / d,
% \end{equation}
% which concludes the power analysis.



%%% Local Variables:
%%% TeX-master: "atlas"
%%% End:










==> others.tex <==
% !TEX root = ranking.tex


\section{Ignore this section} \label{sec:oth}


For $l_2$ norm in Lemma 15 in \cite{chen2019spectral},
they have
\begin{equation}
\begin{aligned}
\boldsymbol{\theta}^{t+1}-\boldsymbol{\theta}^{*} &=\boldsymbol{\theta}^{t}-\eta \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{t}\right)-\boldsymbol{\theta}^{*} \\
&=\boldsymbol{\theta}^{t}-\eta \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{t}\right)-\left[\boldsymbol{\theta}^{*}-\eta \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right]-\eta \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right) \\
&=\left\{\boldsymbol{I}_{n}-\eta \int_{0}^{1} \nabla^{2} \mathcal{L}_{\lambda}(\boldsymbol{\theta}(\tau)) \mathrm{d} \tau\right\}\left(\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right)-\eta \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right) \\
&:=\left\{\boldsymbol{I}_{n}-\eta\boldsymbol{A}\right\}\left(\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right)-\eta \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)
\end{aligned}
\end{equation}

Then 
\begin{equation}\begin{aligned}
\left\|\boldsymbol{\theta}^{t+1}-\boldsymbol{\theta}^{*}\right\|_{2} 
&\leq\left\|\left(\boldsymbol{I}_{n}-\eta \boldsymbol{A}\right)\left(\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right)\right\|_{2}+\eta\left\|\nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right\|_{2} \\
& \leq\left(1-\frac{1}{10 \kappa} \eta n p\right)\left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{2}+\eta\left\|\nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right\|_{2} \\
& \leq\left(1-\frac{1}{10 \kappa} \eta n p\right) C_{1} \kappa \sqrt{\frac{\log n}{p L}}+C \eta \sqrt{\frac{n^{2} p \log n}{L}} \\
& \leq C_{1} \kappa \sqrt{\frac{\log n}{p L}}
\end{aligned}\end{equation}


But for $l_\infty$ norm, we can achieve 
$\left\|\nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right\|_{\infty} \lesssim\sqrt{\frac{n p \log n}{L}}$, but
$\left\|\left(\boldsymbol{I}_{n}-\eta \boldsymbol{A}\right)\left(\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right)\right\|_{2} \leq\left(1-\frac{1}{10 \kappa} \eta n p\right)\left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{2}$
cannot be easily extended to $l_\infty$ norm.\\

$\Downarrow$

We then turn to bound every entry of $\boldsymbol{\theta}^{t+1}-\boldsymbol{\theta}^{*}$ instead, which gives us
\begin{equation}
\begin{aligned}
&{\theta}_m^{t+1}-{\theta}_m^{*} \\
&={\theta}_m^{t}-\eta \left[ \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{t}\right)\right]_m-{\theta}_m^{*} \\
&={\theta}_m^{t}-{\theta}_m^{*}-\eta \left\lbrace \left[ \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{t}\right)\right]_m -\left[ \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right]_m\right\rbrace -\eta \left[ \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right]_m \\
&= {\theta}_m^{t}-{\theta}_m^{*}-\eta \left[ \sum_{(i, j) \in \mathcal{E}, i>j}\left(\frac{e^{\theta^t_{i}}}{e^{\theta^t_{i}}+e^{\theta^t_{j}}}-\frac{e^{\theta^*_{i}}}{e^{\theta^*_{i}}+e^{\theta^*_{j}}}\right)\left(\boldsymbol{e}_{i}-\boldsymbol{e}_{j}\right) \right]_m 
-\eta \lambda \left( {\theta}_m^{t}-{\theta}_m^{*} \right) 
-\eta \left[ \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right]_m
\end{aligned}
\end{equation}

For the second term,  we have 
\begin{equation}
\begin{aligned}
&\left[ \sum_{(i, j) \in \mathcal{E}, i>j}\left(\frac{e^{\theta^t_{i}}}{e^{\theta^t_{i}}+e^{\theta^t_{j}}}-\frac{e^{\theta^*_{i}}}{e^{\theta^*_{i}}+e^{\theta^*_{j}}}\right)\left(\boldsymbol{e}_{i}-\boldsymbol{e}_{j}\right) \right]_m \\
=& \sum_{(i, m) \in \mathcal{E}, i > m}-\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{m}^{t}-\theta_{i}^{t}-\left(\theta_{m}^{*}-\theta_{i}^{*}\right)\right](-1)
+\sum_{(i, m) \in \mathcal{E}, i < m}-\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{m}^{t}-\left(\theta_{i}^{*}-\theta_{m}^{*}\right)\right] \\ 
=& \sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{m}^{t}-\theta_{i}^{t}-\left(\theta_{m}^{*}-\theta_{i}^{*}\right)\right] \\
=&\sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{m}^{t}-\theta_{m}^{*}\right]
-\sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{i}^{*}\right]
\end{aligned}
\end{equation}
where $c_i$ is some real value lying betwen $\theta_{m}^{t}-\theta_{i}^{t}$ and $\theta_{m}^{*}-\theta_{i}^{*}$ satisfying $\frac{e^{c}}{\left(1+e^{c}\right)^{2}} \leq \frac{1}{4}$ and $\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}=\frac{e^{-\left|c_{i}\right|}}{\left(1+e^{-\left|c_{i}\right|}\right)^{2}} \geq \frac{e^{-\left|c_{i}\right|}}{4} \geq \frac{1}{4 e^{\epsilon} \kappa} \geq \frac{1}{5 \kappa}$.

Taking the previous bounds together, we have 
\begin{small}
\begin{equation}
\begin{aligned}
&{\theta}_m^{t+1}-{\theta}_m^{*} \\
=& {\theta}_m^{t}-{\theta}_m^{*}-\eta \left[\sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{m}^{t}-\theta_{m}^{*}\right]
-\sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{i}^{*}\right] \right] 
-\eta \lambda \left( {\theta}_m^{t}-{\theta}_m^{*} \right) 
-\eta \left[ \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right]_m \\
=& \left( 1-\eta\lambda -\eta \sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\right) \left({\theta}_m^{t}-{\theta}_m^{*} \right) 
+ \eta \sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{i}^{*}\right] 
-\eta \left[ \nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right]_m \\
:=& I_1+I_2+I_3
\end{aligned}
\end{equation}
\end{small}

Thus 
\begin{equation}
\begin{aligned}
\left|\theta_{m}^{t+1}-\theta_{m}^{*}\right| 
&\leq\left(1-\eta \lambda-\frac{1}{10 \kappa} \eta np\right)\left|\theta_{m}^{t}-\theta_{m}^{*}\right|
+\frac{\eta np}{4}\left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{\infty}
+\eta \left\|\nabla \mathcal{L}_{\lambda}\left(\boldsymbol{\theta}^{*}\right)\right\|_{\infty}
\end{aligned}
\end{equation}

But since $-\left(\eta \lambda+\frac{1}{10 \kappa} \eta np\right)\left|\theta_{m}^{t}-\theta_{m}^{*}\right|
+\frac{\eta np}{4}\left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{\infty}$
or $-\left(\eta \lambda+\frac{1}{10 \kappa} \eta np\right)\left|\theta_{m}^{t}-\theta_{m}^{*}\right|
+\frac{\eta \sqrt{np}}{4}\left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{2}$ doesn't necessarily less than 0, it's not working out again......\\

$\Downarrow$

But if  $(i, m) \in \mathcal{E}$ and  $\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{i}^{*}\right] $ are independent, we can achieve a better rate for 

\begin{equation}
\begin{aligned}
&\sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{i}^{*}\right] \\
:=&  \sum_{ i\neq m}  \mathcal{E}_{i,m} z_i \\
=& \sum_{ i\neq m} ( \mathcal{E}_{i,m}-p) z_i +\sum_{ i\neq m}  p z_i \\
=&T_1+T_2
\end{aligned}
\end{equation} 

For $T_2$, we have
$\sum_{ i\neq m}  p z_i \leq \frac{1}{4}\sqrt{n}p \left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{2} $, which is great.

For $T_1$, by Bernstein's inequality (requiring independency),
we obatin $\sum_{ i\neq m} ( \mathcal{E}_{i,m}-p) z_i \leq \frac{1}{4}(\sqrt{2a np \log n} + \frac{2a}{3}\log n) \left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{\infty}$, which is smaller than $\frac{1}{10 \kappa}  np \left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{*}\right\|_{\infty}$ as long as $p>\frac{c_{0} \log n}{n}$ for some sufficiently large constant $c_{0}>0$. 


So 
\begin{equation}
\begin{aligned}
&\sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{i}^{*}\right] \\
=& \sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t}-\theta_{i}^{t,(m)}\right]
+\sum_{(i, m) \in \mathcal{E}, i\neq m}\frac{e^{c_{i}}}{\left(1+e^{c_{i}}\right)^{2}}\left[\theta_{i}^{t,(m)}-\theta_{i}^{*}\right] \\
\leq& \frac{1}{4} \sqrt{np} \left\|\boldsymbol{\theta}^{t}-\boldsymbol{\theta}^{t,(m)}\right\|_{2} + Bernstein\\
\lesssim & \sqrt{np} \sqrt{\frac{\log n}{npL}} + ......
\end{aligned}
\end{equation} 


	%Lemma 19 in \cite{chen2019spectral}  (Bernstein's inequality). Consider $n$ independent random variables $z_{l}(1 \leq l \leq n),$ each satisfying $\left|z_{l}\right| \leq B$. For any $a \geq 2,$ one has$$\left|\sum_{l=1}^{n} z_{l}-\mathbb{E}\left[\sum_{l=1}^{n} z_{l}\right]\right| \leq \sqrt{2 a \log n \sum_{l=1}^{n} \mathbb{E}\left[z_{l}^{2}\right]+\frac{2 a}{3} B \log n}$$ with probability at least $1-2 n^{-a}$.



%%% Local Variables:
%%% TeX-master: "atlas"
%%% End:


==> simulation.tex <==
% !TEX root = RankingFDR.tex

